PersonaChatBench: Evaluating Chat Assistants with Diverse Simulated Users

Conversational assistants are expected to help people with diverse backgrounds, preferences, and communication styles. Yet evaluations centered on a single cooperative user provide limited insight into how reliably an assistant serves users with different personas. We introduce PersonaChatBench, a framework for evaluating task competence and responsiveness to diverse user needs. PersonaChatBench pairs the same underlying task with multiple simulated users, each guided by a private persona card that specifies distinct needs, preferences, and interaction behaviors. By holding the task fixed while varying the user, the framework examines how assistant performance changes across user conditions. We evaluate 20 language models across six domains, separately assessing native task outcomes, fulfillment of expressed persona needs, and simulator fidelity. Our results show that task performance and need fulfillment vary across personas and domains. Strong task performance does not necessarily translate into satisfying individual needs, and models' relative strengths in meeting those needs are not consistent across domains. PersonaChatBench makes these differences measurable, revealing gaps obscured by aggregate scores and helping identify which users an assistant serves well and where adaptation is needed. It provides a basis for evaluating consistency across users and guiding the development of assistants that better accommodate diverse needs in everyday applications.

==> figures/persona_task_gaps_four_domains.tex <==
% Rebuilt from original Figure 4. Coding row removed; all other values unchanged.
\begin{tikzpicture}[x=0.064cm,y=1cm,font=\sffamily]
\path[use as bounding box] (-1,-0.55) rectangle (102,5.72);
\node[anchor=west,font=\sffamily\bfseries\small] at (0,5.45) {Health};
\node[anchor=east,font=\sffamily\bfseries\small,text=PCBlue] at (100,5.45) {Gap 13.13};
\node[anchor=west,font=\sffamily\scriptsize,text=black!65] at (0,5.22) {Claude Opus 5.5};
\draw[black!16,line width=.4pt] (0,4.98) -- (100,4.98);
\draw[PCBlue,line width=2.0pt] (52.75,4.98) -- (65.88,4.98);
\draw[PCBlue,fill=white,line width=1pt] (52.75,4.98) circle[radius=2.2pt];
\fill[PCBlue] (65.88,4.98) circle[radius=2.2pt];
\node[anchor=west,font=\sffamily\scriptsize] at (0,4.68) {\textbf{52.75}\quad Guarded, time-conscious novice};
\node[anchor=west,font=\sffamily\scriptsize] at (0,4.45) {\textbf{65.88}\quad Receptive, informed contributor};
\node[anchor=west,font=\sffamily\bfseries\small] at (0,4.13) {Math};
\node[anchor=east,font=\sffamily\bfseries\small,text=PCPurple] at (100,4.13) {Gap 8.04};
\node[anchor=west,font=\sffamily\scriptsize,text=black!65] at (0,3.90) {Grok 4.6};
\draw[black!16,line width=.4pt] (0,3.66) -- (100,3.66);
\draw[PCPurple,line width=2.0pt] (87.44,3.66) -- (95.48,3.66);
\draw[PCPurple,fill=white,line width=1pt] (87.44,3.66) circle[radius=2.2pt];
\fill[PCPurple] (95.48,3.66) circle[radius=2.2pt];
\node[anchor=west,font=\sffamily\scriptsize] at (0,3.36) {\textbf{87.44}\quad Anxious starter};
\node[anchor=west,font=\sffamily\scriptsize] at (0,3.13) {\textbf{95.48}\quad Concise independent learner};
\node[anchor=west,font=\sffamily\bfseries\small] at (0,2.81) {Finance};
\node[anchor=east,font=\sffamily\bfseries\small,text=PCOrange] at (100,2.81) {Gap 7.59};
\node[anchor=west,font=\sffamily\scriptsize,text=black!65] at (0,2.58) {Gemini 3.8 Flash};
\draw[black!16,line width=.4pt] (0,2.34) -- (100,2.34);
\draw[PCOrange,line width=2.0pt] (40.72,2.34) -- (48.3,2.34);
\draw[PCOrange,fill=white,line width=1pt] (40.72,2.34) circle[radius=2.2pt];
\fill[PCOrange] (48.3,2.34) circle[radius=2.2pt];
\node[anchor=west,font=\sffamily\scriptsize] at (0,2.04) {\textbf{40.72}\quad Careful learner};
\node[anchor=west,font=\sffamily\scriptsize] at (0,1.81) {\textbf{48.30}\quad Confident contrarian};
\node[anchor=west,font=\sffamily\bfseries\small] at (0,1.49) {Customer Service};
\node[anchor=east,font=\sffamily\bfseries\small,text=PCTeal] at (100,1.49) {Gap 22.73};
\node[anchor=west,font=\sffamily\scriptsize,text=black!65] at (0,1.26) {GPT-6 Astra};
\draw[black!16,line width=.4pt] (0,1.02) -- (100,1.02);
\draw[PCTeal,line width=2.0pt] (71.97,1.02) -- (94.7,1.02);
\draw[PCTeal,fill=white,line width=1pt] (71.97,1.02) circle[radius=2.2pt];
\fill[PCTeal] (94.7,1.02) circle[radius=2.2pt];
\node[anchor=west,font=\sffamily\scriptsize] at (0,0.72) {\textbf{71.97}\quad Wants the reason};
\node[anchor=west,font=\sffamily\scriptsize] at (0,0.49) {\textbf{94.70}\quad Self-doubt};
\draw[black!40,line width=.4pt] (0,0.12) -- (100,0.12);
\draw[black!40] (0,0.12) -- (0,0.06);
\node[anchor=north,font=\sffamily\scriptsize] at (0,0.02) {0};
\draw[black!40] (25,0.12) -- (25,0.06);
\node[anchor=north,font=\sffamily\scriptsize] at (25,0.02) {25};
\draw[black!40] (50,0.12) -- (50,0.06);
\node[anchor=north,font=\sffamily\scriptsize] at (50,0.02) {50};
\draw[black!40] (75,0.12) -- (75,0.06);
\node[anchor=north,font=\sffamily\scriptsize] at (75,0.02) {75};
\draw[black!40] (100,0.12) -- (100,0.06);
\node[anchor=north,font=\sffamily\scriptsize] at (100,0.02) {100};
\node[anchor=north,font=\sffamily\scriptsize] at (50,-0.20) {Task score};
\end{tikzpicture}


==> old_archive/sections/abstract.tex <==
Chat assistants are usually evaluated against one cooperative user, so a score does not show whether an assistant would solve the task and serve a different person. \benchmark{} fixes the task, the opening question and the assistant's first reply, and varies only who continues the conversation: a simulated user with a private persona card (Math generates the opening and first reply per persona). Each conversation receives a native task grade, a persona-needs score and a simulator audit, reported separately. We cover six domains, 20 tested assistants and 126,460 planned conversations.
% src: data/tables_key_numbers.json coverage.total.planned; data/models.csv (20 rows); math-benchmark/docs/METHODS.md (opening and first reply generated per persona)
Native task rankings agreed across five domains (Kendall's $W=0.68$, 13 models) but not with Health, where inquiry coverage tracked how much the assistant, acting as the doctor, asked and wrote in its first reply; this exception rests largely on two models.
% src: data/rank_consistency.csv kendall_w task coding..travel main_cohort_all_domains_in_set as_extracted (n=13); data/previews/mechanisms_stats.csv panel a and supp first_reply_words_median (main_cohort); recomputed from data/cells.csv without MiniMax M3 and Muse Glimmer 30B (see sections/results.tex)
Task and needs scores were negatively associated across models in Travel ($\rho=-0.63$) but not robustly elsewhere, and needs rankings showed no detectable agreement across domains.
% src: data/task_vs_needs.csv main_cohort (travel rho -0.626, p_perm 0.005; only Travel survives a Holm correction over six domains); data/rank_consistency.csv kendall_w needs (0.220, p_perm 0.194) and the Coding-free needs W in data/previews/rank_consistency_values.csv
Who asks matters most where the score depends on what the user leaves with: a skeptical comparer lowered the Travel reward by 24.1 points on average, with intervals below zero for all 19 models.
% src: data/previews/persona_effects_values.csv travel skeptical_comparer mean, n_models_ci_below
Many failures reflect the protocol rather than domain competence; one model made no tool call in 660 of 1,452 Customer Service conversations. We recommend reporting task outcomes, need outcomes, simulator validity and judge policies separately.
% src: data/muse_tool_diagnosis.md section 1 (660/1,452)


==> old_archive/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\benchmark{} treats the user as an experimental condition: it fixes the task, the question and the first reply (both generated per condition in Math) and judges the task, the persona's needs and the simulated user separately. Across six domains and 20 tested assistants, main-cohort task rankings agreed outside Health, and task success and need satisfaction diverged in domain-specific ways. The persona mattered most where the score depends on commitment, the ending or disclosure, and many failures concerned the protocol rather than domain competence.
% src: data/models.csv (20 models); data/domain_facts.json (6 domains)
Future work includes repeated trials, human selection of the remaining persona banks, independent judges and validation with real users.


==> old_archive/sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

A native task score shows whether the task was solved, not whether the person who asked was served, and our results suggest that the two can be in tension. The skeptical comparer, who asks the assistant to compare options before committing, lowered the Travel reward in a paired comparison, and assistants that left aspects uncommitted had lower rewards but higher needs scores. A persona effect on the native score thus admits two readings, a genuine loss or a metric that does not credit the requested conversation, and the persona-needs score helps to distinguish them.

We recommend four practices: reporting task and need outcomes separately and per domain, with cross-domain claims based on ranks; reporting needs coverage and simulator validity by persona; recording the supporting model and judge policy of every cell and comparing only like configurations; and checking formats, tool markers, budgets and harness interactions before reading a score as competence. Multi-turn uses of single-answer metrics also appear to reward particular conversational behaviors, such as asking early, committing early or writing long replies. Benchmarks should state such preferences, as \figref{fig:mechanisms} illustrates for three domains, because they shape which users appear well served.


==> old_archive/sections/experimental_setup.tex <==
\section{Experimental Setup}
\label{sec:setup}

We analyzed the recorded runs of the benchmark repository at a fixed commit and made no model calls for this paper. Every planned conversation, including failed and unscored ones, counts in the planned totals. Failures were kept as recorded, except under documented recovery amendments: five Qwen 3.8 27B and eight Muse Glimmer 30B Finance tasks were regenerated, three Claude Opus 5.5 Finance tasks were rerun with a larger output budget, and the Math runs of the two locally served models resent interrupted tutor calls once (Appendix~\ref{app:judge-policy}).
% src: data/build_manifest.json source_commit 4cbf5c4e; checkout output/results/finance/{qwen-3-8-27b,muse-glimmer-30b}/*/manifest.json recovery.native_resume.regenerated_task_ids (5, 8); data/cells.csv repaired_judges finance Claude Opus 5.5 (3 blocked tasks, 36 conditions, rerun at 65,536 tokens); output/results/math/{qwen-3-8-27b,muse-glimmer-30b}/*/manifest.json setup.notes (recovery r1 resent 32 interrupted teacher calls)

\subsection{Tested Models}
\label{sec:models}

\input{tables/models}

We evaluated the 20 tested assistants listed in \tabref{tab:models} \citep{openai2026gpt55,openai2026gpt56,openai2026gpt6,anthropic2026claude55,anthropic2026fable51,google2026gemini37flash,google2026gemini38flash,xai2026grok46,moonshot2026kimik3,minimax2026m3,deepseek2026v41flash,zhipu2026glm53flash,qwen2026qwen38flash,hf2026qwen38_27b,hf2026museglimmer30b}. Eighteen were called through hosted APIs or gateways; the open-weight Qwen 3.8 27B and Muse Glimmer 30B were served locally with vLLM 0.30.0 \citep{kwon2023vllm} in BF16 with a 65,536-token output cap, and their supporting roles used GPT-6 Luna at medium effort through a different provider route (Appendix~\ref{app:local-serving}).
% src: data/models.csv label (20 rows), served_locally, serving_route; data/cells.csv provider_route, thinking, output_budget_tokens (Qwen 3.8 27B, Muse Glimmer 30B); run manifests notes ("GPT-6 Luna medium ran through Azure, not Bedrock as for the Haiku/Sonnet cohort"; chat-template variable reasoning_effort / reasoning_strength)
The reasoning effort of the tested assistant was medium, except that MiniMax M3 ran without reasoning, DeepSeek V4.1 Flash at low effort, and Grok 4.6 in Health and Finance and Claude Opus 5.5 outside Math at high effort. Output budgets follow each package; they are not recorded for 54 of the 119 runs and otherwise range from 8,192 to 128,000 tokens, with a 10,000-token cap for Qwen 3.8 Flash and GLM 5.3 Flash in four domains.
% src: data/models.csv thinking_progress_table; data/cells.csv thinking, output_budget_tokens (NA in 54 of 119 runs; min 8192, max 128000; GLM 5.3 Flash and Qwen 3.8 Flash 10000 in math, finance, customer_service, travel)

\subsection{Supporting Roles and Cohorts}
\label{sec:cohorts}

The simulated user, any model-based task grader, the needs judge and the simulator audit are supporting roles. We call one tested model's run in one domain a \emph{cell}. The \emph{main cohort} of a domain contains the cells with the exact frozen task and persona panel, GPT-6 Luna at medium effort in every supporting role, a complete registry status and full dialogue evidence (transcripts and item-level judgments); the older Claude Haiku 5.5 and Claude Sonnet 5.5 packages, which predate the registry's final-data flag, qualify. It contains 12 models in Health, 14 in Coding, 15 in Math, 18 in Finance, 14 in Customer Service and 19 in Travel, or 92 of the 119 cells, and 12 models belong to it in all six domains. Supporting-role budgets still differ within it: GPT-6 Luna had 10,000 instead of 12,288 output tokens in the Finance cells of Qwen 3.8 Flash and GLM 5.3 Flash, and at least 8,192 instead of 500 to 1,200 in the Customer Service cells of the two locally served models (Appendix~\ref{app:local-serving}).
% src: data/tables_key_numbers.json domains.*.main_cohort_models, non_main_cells.main, domains.runs; data/build_manifest.json main_cohort_sizes, main_cohort_all6; scripts/build_dataset.py docstring (main-cohort rule incl. old-format Haiku/Sonnet packages without final_data); data/cells.csv notes (finance Qwen 3.8 Flash, GLM 5.3 Flash: GPT-6 Luna roles at 10,000, default 12,288); appendix/runs.tex local serving (Azure vs Bedrock; Luna calls at least 8,192 tokens, native Customer Service support budgets 500-1,200)
Rankings, rank correlations and persona effects use main-cohort cells only; the other 27 cells are reported with markers (\tabref{tab:exceptions} in Appendix~\ref{app:cohort}). Seven used GPT-5.6 Sol at high effort in some or all supporting roles: Grok 4.6 in Health and Finance, and Claude Opus 5.5 outside Math. Fifteen are score-only packages, delivered without transcripts, for GPT-5.5, GPT-5.6 Sol, GPT-5.6 Terra, GPT-6 Astra and GPT-6 Sol in Health, Math and Customer Service; in Health, these packages used a stricter native judge-acceptance rule than the \texttt{llm\_judgment\_v1} rule of the other Health runs. The five Coding cells of these models are registered as partial, and Fable 5.1 has no Health run.
% src: data/tables_key_numbers.json non_main_cells (support 7, scoreonly 15, partial 5, norun 1); data/cells.csv cohort_exclusion_reason, support_roles, task_metric_name (health: native_strict vs llm_judgment_v1), notes

\subsection{Metrics and Statistics}
\label{sec:metrics}
\label{sec:stats}

A domain's \emph{task headline} is its native task score over its native population (\tabref{tab:scorecard-full} in Appendix~\ref{app:coverage}) on a 0--100 scale: a percentage of episodes or criteria, the PRBench rubric percent in Finance, or reward$\times$100 in Travel. Its \emph{needs headline} is the persona-needs score, and \tabref{tab:coverage} gives the coverage of every cell.
% src: data/domain_facts.json <domain>.task_metric, task_population; data/cells.csv task_scale, task_population

The paired persona effect of a model is the mean, over tasks on which both conversations are scored, of the persona conversation's native score minus the neutral conversation's score, with a 95\% task-cluster bootstrap interval from 5,000 resamples. Summaries across models treat models as the units of replication. In Math the contrast includes the persona-specific opening and first reply. In Customer Service it uses graded completed conversations, whereas the headline scores incomplete ones as zero, and the neutral reference averages three trials, only the first of which shares the personas' first reply.
% src: data/verification.md (bootstrap: 5000 resamples, default_rng(0), 2.5/97.5 percentiles); data/persona_effects.csv task_population (customer_service: graded completed episodes, neutral = 3 trials per task, per-task mean); data/domain_facts.json customer_service.task_population; checkout customer-service-benchmark/eval/PROTOCOL.md section 3 item 7; math-benchmark/docs/METHODS.md

Because native metrics are not commensurable, cross-domain comparisons use ranks only: Spearman's $\rho$ for a pair of domains over models in the main cohort of both, and tie-corrected Kendall's $W$ over models in the main cohort of all included domains. Within a domain, Spearman's $\rho$ between the task and needs headlines across models is an association, not a causal estimate. All $p$-values come from 10,000 permutations, two-sided for $\rho$ and one-sided for $W$; we report them uncorrected and note where a result does not survive a Holm correction within its family. About 5\% of per-model intervals are expected to exclude zero by chance.
% src: data/build_manifest.json statistics (permutations=10000, seed 0); scripts/build_dataset.py docstring (two-sided |r_perm|>=|r_obs|; one-sided W_perm>=W_obs; tie-corrected W); data/rank_consistency.csv populations main_cohort_both (Spearman pairs) and main_cohort_all_domains_in_set (Kendall W); data/task_vs_needs.csv population main_cohort
We do not interpret Coding needs rankings, because needs-scored Coding conversations range from 19 to 591 per cell, depending mainly on how packages handled judge outputs that failed validation (\secref{sec:validity}).
% src: data/cells.csv coding needs_den (min 19: MiniMax M3, GPT-6 Astra; Gemini 3.7/3.8 Flash 54/64 under validated original outputs; max 591: Claude Opus 5.5), repaired_judges
Because each task, model and condition was run once, apart from the three Customer Service neutral trials, each paired difference rests on one draw: the intervals cannot separate generation noise from task heterogeneity, and headline scores carry no run-to-run uncertainty.
% src: data/tables_key_numbers.json domains.*.neutral_trials (customer_service 3, others 1)


==> old_archive/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

People who bring the same request to a chat assistant may expect different conversations. A patient who does not know a medical term needs plain explanations, whereas an informed patient may want the reasoning behind each question; one traveler wants every option compared, whereas another wants a single clear recommendation. Chat assistants are nevertheless evaluated mostly against a fixed user: rubric and preference evaluations score answers to a scripted question \citep{zheng2023mtbench,chiang2024chatbotarena,arora2025healthbench,akyurek2025prbench}, and interactive benchmarks place one cooperative simulated user in each environment \citep{yao2024taubench,barres2025tau2bench,dou2025simulatorarena,wu2025collabllm}. Studies that vary the simulated user typically do so within one domain \citep{shim2025noncollaborative,chopra2026ppol}, and persona work mostly conditions the assistant rather than the user \citep{zhang2018personachat,gupta2023biasrunsdeep}. What is missing is a benchmark that treats the user as an experimental condition while the task is held fixed, keeps each domain's native grader, measures separately whether the particular user was served and does so for many assistants and domains.

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures/overview.pdf}
\caption{\textbf{Overview of \benchmark.}
\textbf{a,} A task has a persona-free question $q$ and a public context $c$, which the tested assistant sees; user-side facts $K$, which only the simulated user sees; and a private native evaluator $e$. The shared first reply $r$ is generated once per task, model and trial and reused in every condition (Math: $q$ and $r$ per condition).
\textbf{b,} After $(q,r)$, simulated users with private persona cards and a neutral user without a card respond or stop; purple dots mark expressed needs, the turn cap $T$ is a limit, and the lower block shows which inputs each role sees.
\textbf{c,} Every conversation receives a native task grade and a simulator audit, and every persona conversation a persona-needs score; the three are never merged.
Bottom: planned conversations per model by domain, 6,383 for a model with runs in all six domains.}
% src: data/tables_key_numbers.json domains.*.episodes_per_model (sum 6,383); math-benchmark/docs/METHODS.md (Math opening per persona)
\label{fig:overview}
\end{figure}

We introduce \benchmark{} (\figref{fig:overview}), which brings six domains (health consultation, coding, mathematics tutoring, financial advice, customer service and travel planning) under one shared protocol while keeping each domain's source tasks and native grading. The \emph{tested assistant} answers a persona-free question once per task, assistant setup and trial, and this \emph{shared first reply} opens every condition, so that differences between conditions do not originate in the opening. Math is the documented exception: the student's opening and the tutor's first reply are generated per condition, so Math contrasts include the opening. In each \emph{persona condition}, a \emph{simulated user} continues under a private persona card with one or more needs frozen in advance and may stop at any time; the persona reaches the assistant only through the user's messages. A \emph{neutral condition} without a card is the paired reference. Conversations receive three judgments that are never pooled: the \emph{native task grade} of the source benchmark, a \emph{persona-needs score} over needs that the user expressed and the assistant could answer (persona conditions only) and a \emph{simulator audit} of the simulated user; as in PARADISE \citep{walker1997paradise}, task success and user satisfaction remain distinct. We report per-domain results and cross-domain rank agreement rather than one leaderboard over heterogeneous metrics.

We evaluated 20 tested assistants over 126,460 planned conversations and report four patterns for the \emph{main cohort}, the runs that share one frozen panel and the same supporting model and effort (\secref{sec:cohorts}).
% src: data/tables_key_numbers.json coverage.total.planned; data/models.csv (20 models)
First, native task rankings agreed across the five domains other than Health (Kendall's $W=0.68$, $n=13$, $p<0.001$); Health inquiry coverage tracked the number of questions and the length of the first reply of the tested assistant, which plays the doctor, and the Health disagreement rests largely on two models (\secref{sec:consistency}).
% src: data/rank_consistency.csv kendall_w task coding..travel main_cohort_all_domains_in_set n=13 (W 0.678, p_perm 0.0001); data/previews/mechanisms_stats.csv panel a and supp first_reply_words_median (main_cohort); MiniMax M3 / Muse Glimmer 30B sensitivity in sections/results.tex
Second, task and persona-needs scores were robustly associated across models only in Travel ($\rho=-0.63$, $n=19$, $p=0.005$), where assistants that left more requested aspects without a committed choice earned lower rewards but higher needs scores (\secref{sec:tradeoff}).
% src: data/task_vs_needs.csv population=main_cohort travel (rho -0.626, p_perm 0.005); data/previews/mechanisms_stats.csv panel b and supp x_noncommit vs needs_value (travel, main_cohort); Math and Customer Service sensitivity in sections/results.tex
Third, in paired comparisons with the neutral user, a skeptical comparer lowered the Travel reward by 24.1 points on average over 19 models, whereas no persona changed Math correctness by more than 1.7 percentage points on average over 15 models (\secref{sec:persona-effects}).
% src: data/previews/persona_effects_values.csv travel skeptical_comparer (mean -24.1, n_models 19); math rows (max |mean| 1.65, n_models 15)
Fourth, many failures were protocol failures: Muse Glimmer 30B, for example, made no tool call in 660 of 1,452 Customer Service conversations (\secref{sec:failures}).
% src: data/muse_tool_diagnosis.md section 1 (660/1,452)
Our contributions are:
\begin{itemize}[leftmargin=1.4em,itemsep=1pt,topsep=1pt]
  \item \textbf{A shared protocol} for persona-conditioned evaluation: a shared first reply, private cards with frozen needs, natural stopping, role-separated inputs and three separate judgments (\secref{sec:benchmark}).
  \item \textbf{A six-domain benchmark} over natively graded sources, run on 20 tested assistants, with a declared main cohort and every run's judge policy (\secref{sec:setup}).
  \item \textbf{An analysis} of cross-domain rank agreement, the divergence of task and need outcomes, paired persona effects, protocol failures and measurement validity (\secref{sec:results}).
\end{itemize}


==> old_archive/sections/limitations.tex <==
\section{Limitations and Responsible Use}
\label{sec:limitations}

\emph{Single trial and selected panels.} Because each task was run once per model and condition, apart from the three Customer Service neutral trials (\secref{sec:metrics}), generation noise and task heterogeneity cannot be separated, headline scores and rankings carry no run-to-run uncertainty, and the intervals treat partly outcome-selected panels as samples of tasks; the estimates of these panels, including persona-effect sizes, may not generalize to the source benchmarks. Recovery amendments regenerated some failed generations and reran the voided first Health runs of both locally served models.
% src: data/tables_key_numbers.json domains.*.neutral_trials (persona conditions 1; customer_service neutral 3); data/cells.csv notes (recovery, resume; examples with counts in sections/experimental_setup.tex); output/results/health/qwen-3-8-27b/*-r2/manifest.json setup.amendments health_r1_voided; checkout output/panels/README.md (outcome-selected case-study panels)

\emph{Simulated users and model judges.} Personas are synthetic conditions, and the results do not show how real users with similar preferences would be served. Only the Customer Service persona bank has human selection decisions (\status{retain}); the other five await human selection.
% src: output/panels/*/persona.json personas[].selection.status (retain: customer_service; pending: other five)
In most banks, personas differ in several attributes at once, so differences between personas cannot generally be traced to a single attribute. GPT-6 Luna simulates the user and judges every main-cohort conversation, including its own, which exposes the scores of OpenAI models to self-preference \citep{panickssery2024selfpreference} and all scores to correlated judge errors.

\emph{Heterogeneous runs.} Providers, serving, reasoning settings, tested and supporting-role budgets, routes and judge-output acceptance and repair rules differ between packages, and budgets are not always recorded.
% src: data/models.csv served_locally (Qwen 3.8 27B, Muse Glimmer 30B); data/cells.csv output_budget_tokens (NA in 54 of 119 cells), repaired_judges, notes (supporting-role budgets)
The behavioral mechanisms are associations across models with partly collinear predictors, several cross-domain associations depend on two low-scoring models, and the Finance persona effects and needs ranking are confounded with conversation length. Legal consultation and privacy and security advice, two further protocol domains, are left to future work.
% src: standard/README.md (eight domains); domain table (Law, HelpBench)

\emph{Responsible use.} Personas are communication and behavior conditions, not stand-ins for demographic groups, and no attribute should be read as a trait of a population or used to justify treating users differently. Persona differences are meant to locate failures in how assistants serve people, not to rank people.


==> old_archive/sections/personachatbench.tex <==
\section{PersonaChatBench}
\label{sec:benchmark}

\subsection{Problem Formulation}
\label{sec:formulation}

A \emph{task} $t$ consists of a persona-free initial question $q_t$, a public context $c_t$ (tools, policy, catalogs), user-side facts $K_t$ that the simulated user may know, and a private native evaluator $e_t$ with the source benchmark's tests, rubric or reward. An \emph{assistant setup} $A$ fixes the tested model, prompt, reasoning setting and tools; a \emph{trial} $\tau$ indexes an independent repeat. A \emph{persona} $p=(a_p,N_p)$ is a card with attribute values $a_p$ and observable needs $N_p$; before the assistant answers, a need policy $\pi_{t,p}(n)=(\alpha,\kappa,\beta)$ freezes whether need $n$ applies to $t$ ($\alpha$), whether it is critical ($\kappa$) and which behavior satisfies it ($\beta$). The neutral user $\varnothing$ has no card. For $(t,A,\tau)$ the assistant produces one reply $r=A(c_t,q_t)$, and every condition $p\in\mathcal{P}_t\cup\{\varnothing\}$ continues from $(q_t,r)$:
\[
h_p=(q_t,\,r,\,u_1,\,a_1,\,\dots,\,u_k,\,a_k),\qquad u_i\sim U(K_t,p,h_{<i}),\quad a_i\sim A(c_t,h_{<i},u_i),
\]
where the simulated user $U$ may stop instead of writing $u_i$. A turn is one user message and its reply, the opening pair included, and the cap $T$ is checked after each reply. A conversation $h_p$ together with its stop reason and judgments is an \emph{episode}, the unit of the run records. Three judgments are computed from $h_p$ and never combined: a native task grade $y(h_p)=e_t(h_p)$, a status $\sigma_n(h_p)$ for every need, and an audit $v(h_p)$ of the simulated user. Because conditions share $(t,A,\tau)$ and $r$, the contrast $\Delta_t(p)=y(h_p)-y(h_\varnothing)$ is paired and, up to sampling variation, estimates the total effect of the user condition on the continuation: the user's messages and stopping and the assistant's responses to them. In Math, the simulated student writes the opening $q_{t,p}$ in character and the tutor's first reply $r_p=A(c_t,q_{t,p})$ is generated per condition, so a Math contrast is paired by task only and includes the opening.
% src: checkout math-benchmark/docs/METHODS.md (opening and first tutor reply generated independently per persona; first reply not shared)

\subsection{Domains and Tasks}
\label{sec:domains}

\input{tables/domains}

The six domains (\tabref{tab:domains}) keep their source tasks and native metrics and yield 6,383 planned conversations for a model with runs in all six domains, or 126,460 over the 119 runs.
% src: data/tables_key_numbers.json domains.*.episodes_per_model (1,200+700+1,435+1,164+1,452+432 = 6,383), domains.total_planned_episodes = 126,460, domains.runs = 119 (Fable 5.1 has no Health run)
The Coding, Finance and Customer Service panels were selected using outcomes of earlier runs, partly on persona-induced score changes (Coding and Finance tasks; Customer Service cards and policy variant), and are therefore case-study panels, not random samples. The Math tasks were curated during development for simulation stability, observable traits and gradability, not drawn as a held-out test set.
% src: checkout output/panels/README.md ("Outcome-selected Coding/Finance/Customer Service panels are case-study panels"); appendix/coding.tex, appendix/finance.tex, appendix/service.tex Task panel paragraphs (selection criteria; customer-service-benchmark/HANDOVER.md: cards chosen on completion against the neutral customer and unmet critical needs); math-benchmark/docs/METHODS.md (task selection basis; development curated set, not an independent test set)

\subsection{Personas and Needs}
\label{sec:personas}

Each domain stores its persona bank as auditable cards (Appendices~\ref{app:health}--\ref{app:travel}). Health uses five hand-written profiles with two needs each, Coding six cards derived from MatrAIx records \citep{li2026matraix} with six needs each, and Math six authored profiles with four to six needs each. Finance uses six shared presets with three needs each, two of them critical in the strict needs mode used by every Finance run, and five task-specific personas (D1--D5) designed for each task. Customer Service uses eight cards that each vary one behavior, such as giving up early, and Travel five profiles with three needs each.
% src: checkout output/panels/<domain>/persona.json (cards, dimensions, needs per card; Health 5x2, Coding 6x6, Math 4-6, CS 8 cards, Travel 5x3); finance-benchmark/data/presets_strict.json (6 presets x 3 needs, 2 critical; groups communication/pressure) and finance-benchmark/README.md (strict needs mode); data/persona_labels.csv; data/domain_facts.json finance.condition_note
A persona keeps its needs together rather than being split into one-need personas, and the needs are a grading plan, not a script of mandatory questions. Every card was automatically screened as eligible, but only the Customer Service bank has human selection decisions (\status{retain}), made after reviewers read conversations; the other five banks are therefore not yet conversation-validated (Appendix~\ref{app:cards}).
% src: checkout output/panels/*/persona.json selection.status (customer_service: retain; others: pending)

\subsection{Shared Protocol}
\label{sec:protocol}

\begin{algorithm}[t]
  \caption{One task, one assistant setup and one trial across all conditions.}
  \label{alg:episode}
  \footnotesize
  \setstretch{1.0}
  \begin{algorithmic}[1]
    \REQUIRE Task $t=(q,c,K,e)$; assistant setup $A$; conditions $\mathcal{P}\cup\{\varnothing\}$; turn cap $T$
    \STATE Freeze persona cards, need policies $\pi_{t,p}$, prompts, models and $T$ in the run manifest.
    \STATE $r\gets A(c,q)$ \COMMENT{one shared first reply, saved and reused; Math generates $q$ and $r$ per condition}
    \FOR{each condition $p$ (persona card, or none for $\varnothing$)}
      \STATE $h\gets[q,r]$
      \WHILE{turns$(h)<T$}
        \STATE $(u,\mathit{stop})\gets U(K,p,h)$ \COMMENT{$U$ sees $K$ and the card, never $e$}
        \STATE \textbf{if} $\mathit{stop}$ \textbf{then break}
        \STATE $a\gets A(c,h+[u])$;\quad $h\gets h+[u,a]$ \COMMENT{$A$ sees $c$ and the public dialogue}
      \ENDWHILE
      \STATE $y\gets e(h)$;\ \ $\sigma\gets \mathrm{NeedsJudge}(\pi_{t,p},h)$;\ \ $v\gets\mathrm{Audit}(K,p,h)$
      \STATE record $(h,\text{stop reason},y,\sigma,v)$, including failed and unscored episodes
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

\begin{table}[t]
\centering
\tablestyle{4pt}{1.1}
\begin{tabular}{@{}p{2.3cm}p{6.4cm}p{6.4cm}@{}}
\toprule
\textbf{Role} & \textbf{May use} & \textbf{Must not receive} \\
\midrule
Tested assistant & Task context, permitted tools, public dialogue & Persona card, hidden answers or tests, judge prompts \\
Simulated user & Card (if any), authorized facts, public dialogue & Hidden answers or tests, task rubric, judge feedback \\
Task grader & Artifact or dialogue; source tests, rubric or reward & A replacement rubric devised after seeing results \\
Needs judge & Frozen need policies $\pi_{t,p}$; public dialogue & Permission to infer requests or change criticality \\
Simulator auditor & Persona card, authorized facts, dialogue & Authority to change any assistant score \\
\bottomrule
\end{tabular}
\caption{\textbf{Information visibility by role.} The roles are logical and need not be different models. Shared prompt cores for four roles are combined with domain additions, and the assembled prompts are saved with every run (Appendix~\ref{app:prompts}).}
\label{tab:roles}
\end{table}

Algorithm~\ref{alg:episode} and \tabref{tab:roles} summarize how a conversation starts and continues and what each role sees. Generating the shared first reply once per task, setup and trial keeps persona differences out of the opening without making one model inherit another's answer. Besides the Math exception, Customer Service runs the neutral user in three trials, each with its own first reply; the persona conditions share the first reply of the first trial. The persona card reaches only the simulated user, which may disclose authorized facts but may not invent facts or completed actions. The turn cap is a maximum; there is no forced one-turn condition, minimum length or disclosure quota. Natural endings, cap stops and errors are recorded separately. Outside Math, a conversation that ends after the shared first reply has not tested the persona's needs.
% src: checkout standard/README.md sections 2-3; math-benchmark/docs/METHODS.md (Math opening); customer-service-benchmark/eval/PROTOCOL.md section 3 items 5 and 7 (each trial has its own shared first reply); output/panels/customer_service/grid.json (neutral 3 trials, cards 1)

\subsection{Three Judgments}
\label{sec:judgments}

\paragraph{Native task grade.}
Each domain applies its source evaluator: hidden tests in Coding, a rule-based policy check in Customer Service, the native choice reward in Travel, and model judges applying the source rubric or reference solution in Health, Math and Finance. Whether a grade reads the final artifact or the whole conversation is declared in advance; apart from Finance's local advice threshold, no pass threshold is added where a source has none, and whole-conversation uses of single-answer rubrics are local adaptations, not official scores.

\paragraph{Persona-needs score.}
The needs judge assigns each frozen need one of seven statuses (Appendix~\ref{app:statuses}). A need that was inapplicable, never expressed or expressed without a later reply is unscored, as is one whose answer cannot be judged (\status{not_observable}); otherwise it is \status{satisfied}, \status{partially_satisfied} or \status{not_satisfied}, with credit $c(\sigma_n)$ of $1$, $\tfrac12$ or $0$. With $N^{\mathrm{sc}}(h)$ the scored needs of conversation $h$,
\[
S(h)=\frac{1}{|N^{\mathrm{sc}}(h)|}\sum_{n\in N^{\mathrm{sc}}(h)}c(\sigma_n),
\]
and a cell's persona-needs score is the mean of $S(h)$ over persona conversations with $|N^{\mathrm{sc}}(h)|\geq1$. Unscored statuses are reported as coverage and never imputed. Outside Math, the shared first reply precedes any disclosure and cannot earn credit; in Math, a need stated in the student's opening can be met by the first reply. Coding scores only persona-specific needs, and Finance's strict needs mode judges a need on every later reply to which it applies.
% src: checkout standard/README.md section 4 (statuses, credit 1/0.5/0); standard/prompts/persona_needs_judge.md; math run records grades.persona_needs (disclosures cited at u01, teacher passages at a01); finance-benchmark/data/presets_strict.json note; data/domain_facts.json needs_scope

\paragraph{Persona pass.}
Finance, Customer Service and Travel also report a binary \emph{persona pass}: with $C$ the applicable critical needs, a conversation passes if every need in $C$ was expressed, answered and satisfied, fails if an answered need in $C$ was partially or not satisfied, and is otherwise unknown, or not applicable if $C=\emptyset$. Only Finance reports a joint pass, which also requires a rubric percent of at least 50, a local advice threshold. In every domain, safety and task constraints outrank a conflicting preference.
% src: checkout finance-benchmark/README.md (advice pass = 50% or more; joint = advice pass and persona pass); customer-service-benchmark/eval/METRICS.md section 4 and travel-benchmark/README.md (persona pass rule; no separate joint pass); data/<domain>_cells.csv persona_pass_* (finance, customer_service, travel only)

\paragraph{Evidence validation and simulator audit.}
Judges return structured output with quoted evidence. Outside Health, code validates it before acceptance: the status must belong to the fixed vocabulary, the cited evidence must be locatable in the transcript, and outside Math the opening question and shared reply cannot count as disclosure or response. The Health runs with dialogue evidence instead accept any interpretable judge label. Rejected outputs are retried and otherwise stay missing unless a documented repair applies (\secref{sec:validity}). The simulator audit checks whether the simulated user kept its facts and persona, responded to the assistant and did not leak answers. It returns \textsf{valid}, \textsf{invalid} or \textsf{uncertain} with quoted evidence and never changes an assistant score; Math uses only the first two verdicts, and Health records evidence without a verdict. Coding computes both the task and the needs scores only on simulator-valid conversations, and Customer Service restricts only its needs score to them.
% src: data/domain_facts.json <domain>.audit; data/cells.csv task_population, needs_population (coding: completed and simulator-valid episodes for task and needs; customer_service: needs only); appendix/protocol.tex Evidence validation (healthbench llm_judgment_v1 acceptance; data/health_episodes.csv.gz score_policy); checkout math-benchmark/docs/METHODS.md (QC valid/invalid); healthbench-benchmark/RUNNING_V5.md (advisory audit)


==> old_archive/sections/related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Personas and simulated users.}
Persona-conditioned language models can approximate varied human responses \citep{argyle2022outofone,ge2024personahub}, and recent resources generate personas for coverage \citep{paglieri2026personagenerators}, evaluate interactive systems with them \citep{liu2026personaeval} or provide population-scale profiles \citep{li2026matraix}, one of our attribute sources. Persona experiments are, however, fragile: they depend on undocumented design choices and analytic flexibility \citep{batzner2025whosepersonae,cummins2025analyticflexibility}, their output diversity must be measured \citep{kambhatla2025lexicaldiversity}, and a simulator's fitness for purpose must be argued for each use \citep{liu2026fitnessforpurpose,bao2026eval4sim}. We therefore store persona cards as auditable records with screening and selection status and audit the simulated user in every conversation.

\paragraph{User simulation for interactive evaluation.}
User simulators have long served dialogue evaluation \citep{eckert1997usermodeling,schatzmann2007agenda,wang2023userbehavior}. $\tau$-bench, $\tau^2$-bench and AppWorld-UL test tool-using agents against a simulated user \citep{yao2024taubench,barres2025tau2bench,chen2026appworldul}; SimulatorArena reports that profile-conditioned simulators align with human judgments in math tutoring and document creation \citep{dou2025simulatorarena}; and other benchmarks probe clarification, collaboration, social goals and underspecification \citep{trinh2026hilbench,ta2026regretbench,somasekharan2026sciconvbench,wu2025collabllm,zhou2023sotopia,laban2025lost}. Studies that vary the simulated user through non-collaborative behavior, generated personas or diversity-guided sampling report that agent outcomes change with the user \citep{shim2025noncollaborative,chopra2026ppol,nakash2026diversity}, while others document the limits of simulators as proxies for people \citep{jeong2026assistantbias,balog2026bounding,seshadri2026lostinsimulation,zhou2026sim2real}. These benchmarks and studies typically fix the user population within one environment or domain. \benchmark{} instead makes the user a replicated experimental factor, pairs conditions through a shared first reply in every domain except Math, and applies one protocol to 20 assistants with source-native graders.
% src: data/models.csv (20 models); data/domain_facts.json (6 domains); checkout math-benchmark/docs/METHODS.md (Math opening and first reply per persona)

\paragraph{Personalization and user-dependent behavior.}
Persona-grounded dialogue first conditioned the \emph{agent} on a profile \citep{zhang2018personachat}, and studies of persona-assigned assistants report no reliable accuracy gain, implicit reasoning biases and uneven persona adherence \citep{zheng2023helpfulassistant,gupta2023biasrunsdeep,samuel2024personagym}. On the user side, personalization benchmarks give the model a stored profile \citep{salemi2023lamp}, pluralistic alignment targets diverse users \citep{kirk2024prism,sorensen2024pluralistic}, and other studies test whether identity cues, background or stated views change responses \citep{eloundou2024firstperson,wu2025personalizedsafety,sharma2023sycophancy}. These studies change what the model is told about the user; in \benchmark{} the assistant receives no profile, and needs appear only in the user's words.

\paragraph{Domain benchmarks and judges.}
We build on natively graded sources: MedDialogRubrics for medical consultation \citep{gong2026meddialogrubrics}, related to rubric-based health evaluation and diagnostic dialogue \citep{arora2025healthbench,tu2024amie}; LiveCodeBench for coding \citep{jain2024livecodebench}; for mathematics, the SimulatorArena tutoring tasks built on MATH problems \citep{dou2025simulatorarena,hendrycks2021math}, HARP \citep{yue2024harp} and IMO-ProofBench \citep{luong2025imoproofbench}, alongside tutoring work \citep{macina2023mathdial,jurenka2024learnlm}; PRBench for financial advice \citep{akyurek2025prbench}; ABCD for customer service \citep{chen2021abcd}; and UserBench for travel \citep{qian2025userbench}, related to travel-planning benchmarks \citep{xie2024travelplanner}. Many of these sources use model judges, which agree imperfectly with humans and can favor their own generations \citep{zheng2023mtbench,panickssery2024selfpreference}; we keep the source graders, record the judge configuration of every run and treat self-judging as an explicit caveat.
% src: checkout math-benchmark/THIRD_PARTY_NOTICES.md (SimulatorArena task selection; MATH problems; HARP; IMO-ProofBench); data/domain_facts.json <domain>.source_benchmark


==> old_archive/sections/results.tex <==
\section{Results}
\label{sec:results}

\subsection{Scorecard}
\label{sec:scorecard}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{figures/scorecard_heatmap.pdf}
\caption{\textbf{Scorecard of 20 tested models in six domains.}
\textbf{a,} Native task score and \textbf{b,} persona-needs score, on a 0--100 scale (Finance: rubric percent; Travel: reward$\times$100). Color: percentile among the domain's main-cohort models. The upper block holds the 12 models in the main cohort of all six domains; within each block, rows are ordered alphabetically by model family. Hatched cells are outside the main cohort: $\dagger$ simulated user and judges on GPT-5.6 Sol (high) for some or all roles; $\ddagger$ score-only package; $\S$ run registered as partial; -- no run. Exact values: \tabref{tab:scorecard} (Appendix~\ref{app:coverage}).}
% src: data/previews/scorecard_heatmap_values.csv; scripts/fig_scorecard.py docstring
\label{fig:scorecard}
\end{figure}

\figref{fig:scorecard} and \tabref{tab:scorecard} give both headlines for every cell. Of 126,460 planned conversations, 122,569 (96.9\%) were generated and 122,469 received a native task grade; 78,846 persona conversations had at least one scoreable need (\tabref{tab:coverage}).
% src: data/tables_key_numbers.json coverage.total (planned, generated, task_graded, needs_scoreable)
No model led every domain. The highest main-cohort task scores were those of MiniMax M3 in Health (46.8), Fable 5.1 in Coding (95.5) and Finance (57.1), Qwen 3.8 Flash in Math (97.7), Gemini 3.8 Flash in Customer Service (94.1) and Gemini 3.7 Flash in Travel (86.6); MiniMax M3 and Qwen 3.8 Flash generated only 932 of 1,200 and 985 of 1,435 conversations, respectively.
% src: data/tables_key_numbers.json scorecard.best_main, low_generation_main_cells
The highest needs scores were those of GPT-6 Luna in Health (96.5) and Finance (90.1), Claude Opus 5.5 in Math (90.5), Fable 5.1 in Customer Service (80.2) and GPT-6 Astra in Travel (94.0). Headline scores carry no interval (\secref{sec:metrics}), and in seven of these 11 comparisons the runner-up was within one point.
% src: data/tables_key_numbers.json scorecard.best_main; data/cells.csv task_value, needs_value (main cohort; gaps to runner-up: health task 0.5, coding task 0.8, math task 0.3, math needs 0.7, finance needs 0.1, customer_service needs 0.9, travel needs 0.3; Coding needs not interpreted)
Customer Service completion ranged from 22.7\% to 94.1\%, although 12 of 14 main-cohort models reached the policy-correct decision in more than 90\% of planned conversations.
% src: data/cells.csv task_value, outcome_correct_value (main cohort, customer_service; outcome_correct over planned)

\subsection{Task Rankings Agree across Domains, Except Health}
\label{sec:consistency}

\begin{figure}[t]
\centering
\includegraphics[width=0.86\linewidth]{figures/rank_consistency.pdf}
\caption{\textbf{Agreement of model rankings across domains.}
\textbf{a,} Spearman's $\rho$ between the rankings of two domains (task headline below the diagonal, persona-needs headline above), over the models in the main cohort of both ($n$); outlined: two-sided permutation $p<0.05$ after a Holm correction over the 15 pairs of each headline; gray: Coding needs, not interpreted.
\textbf{b,} Kendall's $W$ over all six domains (dark bars; 12 models in the main cohort of all six) and over five domains (light bars): task without Health, for the same 12 models and for the 13 models in the main cohort of all five; needs without Coding. One-sided permutation $p$; dashed line: mean of $W$ under the permutation null.}
% src: data/rank_consistency.csv (as_extracted); data/previews/rank_consistency_values.csv (Holm-adjusted pair p-values; needs W without Coding); scripts/fig_consistency.py docstring
\label{fig:consistency}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.86\linewidth]{figures/mechanisms.pdf}
\caption{\textbf{Conversational behaviors associated with the headline scores.}
One point per model with dialogue evidence; filled markers are the domain's main cohort, which defines Pearson's $r$, the two-sided permutation $p$, $n$ and the dashed least-squares fit; the gray header gives $r$ over all models. Labels as in \figref{fig:tradeoff}.
\textbf{a,} Health: mean number of question marks in the shared first reply against inquiry coverage.
\textbf{b,} Travel: share of requested aspects without a committed choice against the choice reward; dotted line ($100-x$): the reward if every committed choice were correct.
\textbf{c,} Finance: median length of the shared first reply against the rubric percent and \textbf{d,} against the persona pass rate. Associations are across models, not causal estimates.}
% src: data/previews/mechanisms_stats.csv, data/previews/mechanisms_values.csv; scripts/fig_mechanisms.py docstring
\label{fig:mechanisms}
\end{figure}

Native task rankings agreed across the five domains other than Health (\figref{fig:consistency}). Kendall's $W$ over these five domains was 0.64 for the 12 models in the main cohort of all six domains and 0.68 for the 13 models in the main cohort of all five ($p<0.001$ for both). The strongest pairs were Coding and Finance ($\rho=0.91$, $n=13$), Coding and Math ($\rho=0.84$, $n=14$) and Customer Service and Travel ($\rho=0.82$, $n=14$; all $p<0.001$), whereas Math and Customer Service correlated only weakly ($\rho=0.17$, $n=14$, $p=0.56$).
% src: data/rank_consistency.csv kendall_w task coding..travel (0.641 n=12, 0.678 n=13, p_perm 0.0001); spearman_pair task main_cohort_both (incl. math-customer_service 0.174, p_perm 0.559)
Adding Health lowered $W$ to 0.42 ($n=12$, $p=0.001$), and the correlations of Health with the other domains ranged from $\rho=-0.60$ with Customer Service ($n=12$, $p=0.043$, not significant after the Holm correction) to $\rho=0.11$ with Finance ($n=12$, $p=0.73$).
% src: data/rank_consistency.csv kendall_w task six domains (0.421, p_perm 0.0013); spearman_pair task health-customer_service (p_perm 0.0426; Holm-adjusted 0.43 in data/previews/rank_consistency_values.csv), health-finance
Both the agreement and the Health exception depend partly on two models: MiniMax M3 and Muse Glimmer 30B ranked first and second on Health coverage but 13th or lower in every other domain. Without them, $W$ was 0.44 over the five domains and 0.42 over all six ($n=10$), and the mean correlation of Health with the other domains rose from $-0.19$ to 0.32 (\tabref{tab:rank-sensitivity}).
% src: data/cells.csv task_rank_main_cohort (MiniMax M3: health 1, others 14-19; Muse Glimmer 30B: health 2, others 13-18); recomputed from data/cells.csv task_value for the 12 all-six models minus these two with the build_dataset.py statistics (tie-corrected W 0.437, p_perm 0.010; six domains 0.420, p_perm 0.003; mean Spearman of Health with the five others -0.189 with all 12, 0.321 without the two)

The Health disagreement is consistent with inquiry coverage rewarding broad questioning. Across the 12 main-cohort models, the mean number of questions in the shared first reply, counted as question marks, was strongly associated with coverage ($r=0.86$, $n=12$, $p<0.001$; \figref{fig:mechanisms}a): GPT-6 Luna asked 2.3 questions and reached 27.0\% coverage, whereas MiniMax M3 asked 8.0 and reached 46.8\%.
% src: data/previews/mechanisms_stats.csv panel a main_cohort; data/previews/mechanisms_values.csv health (GPT-6 Luna, MiniMax M3)
The question count was strongly correlated with reply length ($r=0.83$, $n=12$, $p<0.001$), and the partial correlation controlling for median reply length was 0.52 ($n=12$, $p=0.08$), so the two cannot be separated with 12 models.
% src: data/previews/mechanisms_stats.csv supp health (x_questions vs first_reply_words_median 0.828, p_perm 0.0009; partial r 0.521, p 0.081)
Inquiry coverage thus appears to credit early and broad history-taking, which no Health persona's needs request, and we read the Health ranking separately.
% src: output/panels/health/persona.json (needs per persona concern explanation, privacy, focus and the form of questions; none requests broad history-taking)

\subsection{Solving the Task versus Serving the User}
\label{sec:tradeoff}

\begin{figure}[t]
\centering
\includegraphics[width=0.86\linewidth]{figures/task_vs_needs.pdf}
\caption{\textbf{Native task score against persona-needs score within each domain.}
One point per tested model: filled, labeled circles are main-cohort models colored by family; hollow gray circles are cells outside the main cohort, excluded from Spearman's $\rho$ (header, with a two-sided permutation $p$ and $n$). $^\ast$: needs score over fewer than 50 conversations; bold: GPT-6 Luna, which also runs the simulated user and judges. Labels: QwenF and Qwen27B, Qwen 3.8 Flash and 27B; Gem3.7 and Gem3.8, Gemini 3.7 and 3.8 Flash; 5.5, 5.6Sol, 5.6Terra, Astra, 6Sol and Luna, GPT models; Haiku, Sonnet and Opus, Claude 5.5 models.}
% src: data/task_vs_needs.csv (main_cohort rows); scripts/fig_tradeoff.py docstring and SHORT
\label{fig:tradeoff}
\end{figure}

Within domains, rankings by task and by needs agreed only partly (\figref{fig:tradeoff}). The association was negative in Travel ($\rho=-0.63$, $n=19$, $p=0.005$), the only domain in which it survives a Holm correction over the six domains. It was positive in Math ($\rho=0.56$, $n=15$, $p=0.032$) and Customer Service ($\rho=0.54$, $n=14$, $p=0.048$), but both associations depend on MiniMax M3 and Muse Glimmer 30B, which scored low on both headlines; without them, $\rho$ was 0.33 ($n=13$, $p=0.27$) and 0.28 ($n=12$, $p=0.37$), respectively. It was weak in Finance and Health ($\rho=0.13$ and $-0.25$, both $p>0.4$).
% src: data/task_vs_needs.csv population=main_cohort (spearman_rho, spearman_p_perm; Holm: travel 0.0051 x 6 = 0.031, math 0.0319 x 5 = 0.16; finance 0.13 n=18 p=0.61, health -0.25 n=12 p=0.45; coding 0.22 n=14 p=0.46 in the fig:tradeoff header, not interpreted); recomputed from data/cells.csv without MiniMax M3 and Muse Glimmer 30B with the build_dataset.py statistics (math 0.330 p_perm 0.271; customer_service 0.280 p_perm 0.371)
The largest divergences involved particular models. GPT-6 Luna had the highest needs score in Health and Finance but ranked last of 12 on the Health task and 17th of 18 on the Finance task, and GPT-6 Astra had the highest Travel needs score but ranked 16th of 19 on the Travel task. Conversely, Claude Sonnet 5.5 and Gemini 3.7 Flash ranked third and first on the Travel task but 19th and 17th on needs, respectively, and Fable 5.1 had the highest Finance task score but ranked tenth on needs.
% src: data/cells.csv needs_value, task_rank_main_cohort, needs_rank_main_cohort (health, finance, travel)

The behaviors associated with these divergences differ by domain (\figref{fig:mechanisms}). In Travel, the reward was nearly a linear function of the share of requested aspects left without a committed choice ($r=-0.99$, $n=19$), largely by construction: an uncommitted aspect earns no credit, and the share of credit earned by committed choices, 83.8\% to 95.5\%, was not significantly associated with the reward ($r=-0.18$, $n=19$, $p=0.49$). The uncommitted share was positively associated with the needs score ($r=0.61$, $n=19$, $p=0.006$), so assistants that keep comparing or confirming before committing appear to serve the user's needs but forfeit reward when the user ends first (Appendix~\ref{app:travel-results}).
% src: data/previews/mechanisms_stats.csv panel b, supp committed_credit_pct vs y_reward and supp x_noncommit vs needs_value (main_cohort); data/previews/mechanisms_values.csv travel (uncommitted share 7.5% Gemini 3.7 Flash to 59.5% MiniMax M3, as in appendix/travel.tex); travel-benchmark/README.md (a naturally terminated missing choice contributes 0)
In Finance, longer shared first replies were associated with a higher rubric percent ($r=0.62$, $n=18$, $p=0.006$) and, not significantly, a lower persona pass rate ($r=-0.40$, $n=18$, $p=0.10$), consistent with exhaustive replies covering more rubric criteria. The Finance needs score tracked conversation length more closely: the mean number of assistant turns per persona conversation was strongly associated with it ($r=-0.93$, $n=18$, $p<0.001$), and the six OpenAI models had the shortest conversations and the highest needs scores. Because the strict needs mode judges every later reply and the simulated user decides when to stop, the Finance needs ranking cannot be separated from conversation length.
% src: data/previews/mechanisms_values.csv finance x_words (268 words GPT-6 Sol to 749 MiniMax M3, as in appendix/finance.tex); data/previews/mechanisms_stats.csv panels c, d and supp finance persona_turns_mean vs needs_value (main_cohort; from data/finance_episodes.csv.gz assistant_turns, generated persona episodes); data/cells.csv finance needs_rank_main_cohort (GPT-6 Luna 1, GPT-6 Astra 2, GPT-6 Sol 3, GPT-5.6 Sol 4, GPT-5.6 Terra 5, GPT-5.5 6; mean turns 2.04-2.73 against 2.88-4.80 for the others); finance-benchmark/data/presets_strict.json (answer_first, focused_response)

Needs rankings showed no detectable agreement across domains. Kendall's $W$ for the needs headline was 0.22 over six domains ($n=12$, $p=0.19$) and 0.23 without Coding, whose needs rankings we do not interpret ($n=12$, $p=0.31$), both close to their null means (\figref{fig:consistency}b); only Health and Finance agreed significantly after the Holm correction ($\rho=0.94$, $n=12$, $p<0.001$). The persona-needs score should therefore be read per domain.
% src: data/rank_consistency.csv kendall_w needs six domains (0.220 p 0.194); data/previews/rank_consistency_values.csv needs W health,math,finance,customer_service,travel (n=12, p 0.314) and Holm-adjusted pair p-values; spearman_pair needs health-finance

\subsection{Persona Effects Depend on What the Score Measures}
\label{sec:persona-effects}

\begin{figure}[t]
\centering
\includegraphics[width=0.88\linewidth]{figures/persona_effects.pdf}
\caption{\textbf{Paired change in the native task score under each persona, relative to the neutral user.}
Rows are persona conditions, coded as in the appendix persona tables, which give exact values; D1--D5 are the task-specific Finance personas. Gray dots are main-cohort models (number in the header), filled when the model's 95\% task-cluster bootstrap interval excludes zero; the colored marker is the unweighted mean across models with a 95\% $t$-interval (orange: below zero; purple: above; dark gray: spans zero). Bottom rows: each model's mean over personas. Units: percentage points; reward$\times$100 in Travel. Customer Service uses graded completed conversations and averages three neutral trials; Math differences include the per-persona opening and first reply (\secref{sec:metrics}).}
% src: data/previews/persona_effects_values.csv; scripts/fig_persona_effects.py docstring; data/persona_effects.csv task_population (customer_service: graded completed episodes); data/persona_effects_summary.csv mean_delta_unweighted; math-benchmark/docs/METHODS.md (opening and first reply generated per persona); customer-service-benchmark/eval/PROTOCOL.md section 3 items 7 and 12 (each trial has its own shared first reply; personas trial 1, neutral trials 1-3)
\label{fig:persona}
\end{figure}

The persona effect on the native score depended on what the metric measures (\figref{fig:persona}). Because the Coding and Finance tasks and the Customer Service cards were selected partly on persona effects in earlier runs (\secref{sec:domains}), effects there may overstate those on the source benchmarks, unlike the unselected Health, Math and Travel panels.
% src: appendix/coding.tex, appendix/finance.tex, appendix/service.tex Task panel paragraphs (outcome-based selection); appendix/travel.tex (complete official split)

\emph{Travel: commitment.} Four of the five Travel personas lowered the reward on average: the skeptical comparer by 24.1 points, with intervals below zero for all 19 models, and the concise decider, efficient comparer and careful planner by 16.7, 13.3 and 10.4 points, respectively (Appendix~\ref{app:travel-effects}). The concise planner, the only persona without a clear effect ($-1.4$), expressed a need in 14.1\% of its needs-judged conversations, against 99.8\% for the skeptical comparer; this contrast suggests that requests to compare options, to proceed one aspect at a time or to explain before committing defer the commitment that the reward credits.
% src: data/previews/persona_effects_values.csv travel rows (mean, n_models_ci_below; 16, 13 and 13 models below zero, as in appendix/travel.tex); data/travel_needs.csv episode_expressed_rate, mean over 19 main-cohort models (concise_planner 0.1406, skeptical_comparer 0.9984), as in appendix/travel.tex; output/panels/travel/persona.json (comparison, paced_questions, explain_before_commit)

\emph{Customer Service: the ending.} Customers who wanted the reason for a decision and those who gave up early lowered completion most, by 7.5 and 7.2 percentage points, respectively, each with intervals below zero for seven models. Of planned conversations, the share with a correct decision and process but a wrong ending rose from 1.3\% under the neutral user to 9.0\% and 7.7\% for these customers, whereas the share of wrong decisions changed less (Appendix~\ref{app:service-effects}).
% src: data/previews/persona_effects_values.csv customer_service A09, C3; data/customer_service_episodes.csv.gz failure_bucket by condition, main cohort (wrong_ending 71/5,544, 166/1,848, 143/1,848; wrong_decision 460/5,544, 147/1,848, 212/1,848, i.e. 8.3% to 8.0% and 11.5%, as in appendix/service.tex)

\emph{Health: disclosure.} The three novice personas (P1, P3 and P4) lowered inquiry coverage by 2.9, 3.8 and 3.2 percentage points on average, respectively, with intervals below zero for 8, 12 and 11 of the 12 models; the two informed personas (P2 and P5) raised it by 2.2 and 2.1 percentage points. Averaged over the 12 models, the simulated patient disclosed 54.2\% to 55.1\% of the authorized case facts to the novices, 69.5\% to 70.0\% to the informed personas and 65.4\% to the neutral user, whereas the share elicited by the assistant's own questions varied only from 26.4\% to 28.9\% (Appendix~\ref{app:health-effects}).
% src: data/previews/persona_effects_values.csv health rows (p1 -2.94/8, p3 -3.84/12, p4 -3.23/11, p2 +2.16, p5 +2.10); data/health_episodes.csv.gz fact_acquisition, active_fact_acquisition by condition, per-model means then mean over the 12 main-cohort models (p3 0.5424, p4 0.5512, p5 0.6945, p2 0.6996, neutral 0.6541; active p3 0.2639, neutral 0.2891), as in appendix/health.tex

\emph{Math and Coding: content correctness.} Mean Math effects, which include the persona-specific opening and first reply, lay between $-0.6$ and $+1.7$ percentage points, and only the cross-model interval of the detail-oriented checker (P2, $+1.7$) excluded zero. The mean effects of five of the six Coding personas lay between $-2.5$ and $+1.6$ percentage points. The detailed typed professional lowered the pass rate by 10.3 percentage points, with intervals below zero for seven models, through submissions that the LiveCodeBench harness failed before any test ran: only the two personas that request type annotations elicited code containing \texttt{from \_\_future\_\_ import annotations}, and all 191 such main-cohort submissions, like all 242 across packages, failed, as the harness places its own imports first (Appendix~\ref{app:coding-effects}).
% src: data/previews/persona_effects_values.csv math rows (math-p02 ci_lo 0.59, ci_hi 2.71; other math cross-model intervals include 0), coding rows; math-benchmark/docs/METHODS.md (opening per persona); output/panels/coding/persona.json (type_annotations need: matraix_r495132, matraix_r518717); benchmark checkout output/results/coding/*/{data,evidence}.jsonl.gz final_code joined to data/coding_episodes.csv.gz task_outcome (all future-import submissions in these two conditions, all 'fail'; 242 = 213 outside Opus + 29 Opus; 191 main cohort; recomputed from benchmark checkout, not in data/; counting the 179 eligible main-cohort submissions as passes gives +1.8 pp for both personas, dropping them +0.7 and +1.3, as in appendix/coding.tex)

\emph{Finance: length.} Pooled over the five task-specific personas, the rubric percent rose by 3.0 percentage points, with intervals above zero for 13 of 18 models, and pooled over the six shared presets by 1.2 percentage points. The neutral user, however, ended 60.0\% of its generated main-cohort conversations after the shared first reply (1,030 of 1,716), against 0.1\% to 12.7\% for the personas; averaged over the 18 models, its conversations had 1.8 assistant messages, against 2.5 to 4.2 for the persona conditions (\tabref{tab:finance-personas}). Because the rubric evaluates the whole conversation, longer conversations offer more chances to cover criteria, so the gain is not evidence of better advice.
% src: data/persona_effects.csv finance pooled rows, main cohort (pooled:designed mean 2.98, ci_low>0 for 13/18; pooled:shared_presets mean 1.16); data/finance_episodes.csv.gz generated==True, main cohort: stop_reason=user_ended_after_first_reply pooled by condition (neutral 1,030/1,716; careful_learner 2/1,713; p01 216/1,707) and assistant_turns as per-model condition means averaged over 18 models (neutral 1.81; reassurance_seeker 2.46; confident_contrarian 4.21, as in tab:finance-personas); finance-benchmark/README.md (rubric over the whole conversation)

\subsection{Where Conversations Fail}
\label{sec:failures}

\begin{figure}[t]
\centering
\includegraphics[width=0.86\linewidth]{figures/failures.pdf}
\caption{\textbf{Generation failures by tested model and domain.} All 20 tested models; 126,460 planned conversations.
\textbf{a,} Share of planned conversations not generated ($1-$generated$/$planned, \%), pooled over a model's domains in \emph{All}; -- no run; \emph{(local)} served locally with vLLM in BF16.
\textbf{b,} Conversations not generated per model, by failure kind (Math: generation stage only). Completed conversations scored zero, for example for a missing marker, are not counted.}
% src: data/failures.csv, data/previews/failures_plotted.csv; scripts/fig_failures.py docstring
\label{fig:failures}
\end{figure}

Generation failures were rare and concentrated in a few models (\figref{fig:failures}): 3,891 of 126,460 planned conversations (3.1\%) were not generated, 2,358 of them through truncation, protocol or format errors or empty answers. Qwen 3.8 Flash failed to generate 1,204 of its planned conversations (18.9\%) and GLM 5.3 Flash 664 (10.4\%), about half of them through truncation, often after exhausting a 10,000-token cap while reasoning, whereas both Gemini models generated all of theirs. Claude Haiku 5.5 produced 415 invalid JSON objects as the Health doctor.
% src: data/tables_key_numbers.json coverage.total; data/previews/failures_plotted.csv domain=all (not_generated, rate; truncated 1,051, protocol_format 1,027, empty_answer 280; Qwen 3.8 Flash truncated 659 of 1,204, GLM 5.3 Flash 320 of 664); data/cells.csv notes (math Qwen 3.8 Flash and GLM 5.3 Flash: teacher exhausted the 10,000 cap in reasoning, 443 and 284 conversations); data/health_episodes.csv.gz failure_code, failed_role=doctor (Claude Haiku 5.5)

Other protocol failures occurred in completed conversations and lowered the native score directly. In Customer Service, where tools are invoked with a bracketed text marker, Muse Glimmer 30B made no tool call in 660 of 1,452 conversations, against zero to nine for every other model with rule-level records. In 31.6\% of its assistant turns it announced a look-up in prose without writing the marker, against 1.2\% for Qwen 3.8 27B on the same local serving setup; token accounting against the serving logs indicates model behavior rather than a serving artifact (Appendix~\ref{app:service-caveats}). Process gaps, that is, correct decisions without the required look-ups or a matching action, accounted for 57.6\% of the conversations of MiniMax M3, which ran without reasoning. In Coding, 74 completed conversations of Muse Glimmer 30B and 99 of Claude Haiku 5.5 scored zero because of a missing or malformed submission marker. Native scores therefore partly measure compliance with formats, markers and budgets.
% src: data/muse_tool_diagnosis.md sections 1, 3 and 4 (5,186 of 16,427 turns; Qwen 3.8 27B 142 of 11,608; at most about 1.6% of calls discarded), as in appendix/service.tex; data/customer_service_episodes.csv.gz failure_bucket=process_gap (MiniMax M3); data/cells.csv notes coding (Muse Glimmer 30B 74, Claude Haiku 5.5 99)

\subsection{Measurement Validity}
\label{sec:validity}

\emph{Needs are expressed in only part of the conversations.} Among main-cohort persona conversations with a needs judgment, the share with at least one scoreable need was 60.6\% in Health, 71.3\% in Customer Service, 78.6\% in Travel, 91.2\% in Finance, 98.3\% in Coding and more than 99.9\% in Math. The Health simulated users expressed 45.0\% of applicable needs and only 27.2\% to 35.8\% under the novice personas, whose needs are thus tested least, and the P3 and P4 patients demonstrated their persona attributes in only 30.7\% and 16.1\% of audited opportunities (\tabref{tab:health-personas}).
% src: data/tables_key_numbers.json coverage.<domain>.Main cohort needs_scoreable/needs_judged (coding 2,957/3,009; math 17,590/17,593); data/health_needs.csv main cohort, needs_expressed_rate, mean over models (level=pooled all_personas 0.450; level=condition p3 0.272, p1 0.358), as in appendix/health.tex; data/health_episodes.csv.gz attribute_demonstration, main cohort, per-model condition means averaged over 12 models (p3 30.7, p4 16.1)

\emph{Simulator failures concentrate in particular personas.} Between 87.3\% and 99.9\% of audited main-cohort conversations per cell were valid (Health has no verdict). Pooled over these conversations, 21.9\% of the Finance careful-learner and 10.1\% of the concise-pragmatist conversations were invalid, against at most 4.4\% for every other Finance condition, and 14.4\% of those of the Customer Service customer who bundles questions, against 0.5\% for the neutral customer.
% src: data/cells.csv sim_valid_rate (main cohort min 0.873 travel GPT-6 Astra, max 0.999 math DeepSeek V4.1 Flash); data/finance_episodes.csv.gz sim_audit_status and data/customer_service_episodes.csv.gz audit_status by condition, pooled over main-cohort audited episodes (finance careful_learner 376/1,718, concise_pragmatist 173/1,720, other conditions 0.7% to 4.4%, neutral 26/1,721; customer_service A10_uncertainty_low 264/1,838, neutral 30/5,542), as in appendix/finance.tex and appendix/service.tex

\emph{Cells with a different supporting model are not comparable by design.} The Grok 4.6 Health cell differs from the main cohort in the tested model, its high reasoning effort, GPT-5.6 Sol (high) as simulated user and judges and a third judged need for three personas. Its share of persona conversations with a scoreable need, 90.0\% against 35.3\% to 74.2\% in the main cohort, is partly mechanical, and its pooled persona effect ($-4.6$ percentage points) lay outside the main-cohort range ($-3.1$ to $+0.1$). The Claude Opus 5.5 Health cell used GPT-5.6 Sol as simulated user for the neutral condition and three personas but GPT-6 Luna for the other two, so its paired effects are confounded by the simulated user.
% src: data/cells.csv health Grok 4.6 thinking high, support_roles gpt-5.6-sol/high, needs_scoreable/needs_judged (Grok 4.6 899/999; GPT-6 Luna 353/1,000; MiniMax M3 705/950), notes (extra judged needs for P1, P2 and P5, as in tab:exceptions); data/persona_effects_summary.csv health pooled_delta (Grok 4.6 -0.046; main-cohort min/max -0.031/+0.0007); data/cells.csv health Claude Opus 5.5 support_roles, notes (neutral, p1, p2, p5: gpt-5.6-sol high; p3, p4: gpt-6-luna medium)

\emph{Judge policies differ across packages.} The Gemini packages publish a score update that bypasses judge-output validation; our headline uses the validated judgments, as for every other model, and the alternative changes no Kendall's $W$ by more than 0.01. The policy matters most for Coding needs: validation left the Gemini models with 54 and 64 scored conversations, against 585 to 590 for the three packages with repaired judge outputs (\tabref{tab:judge-policy} in Appendix~\ref{app:judge-policy}).
% src: data/rank_consistency.csv as_extracted vs gemini_alt_policy (max |diff| 0.0084); data/cells.csv coding Gemini notes, needs_den, needs_den_alt_policy (540 and 525 rejected judgments, reported in appendix/runs.tex); coding needs_den (main cohort: Fable 5.1 585, Claude Sonnet 5.5 586, Claude Haiku 5.5 590; others 19 to 190), repaired_judges

\emph{Same-vendor judging.} GPT-6 Luna, an OpenAI model, simulates the user and runs every judge in the main cohort, and it had the highest needs score in Health and Finance. In Finance, the six OpenAI models held needs ranks 1 to 6 of 18, with GPT-6 Astra and GPT-6 Sol at 90.0 and 88.8 against GPT-6 Luna's 90.1. A shared family style and a same-vendor preference of the judge or simulated user cannot be separated without an independent judge.
% src: data/cells.csv finance needs_value, needs_rank_main_cohort (GPT-5.5, GPT-5.6 Sol, GPT-5.6 Terra, GPT-6 Astra, GPT-6 Sol, GPT-6 Luna: ranks 1-6)


==> old_archive/tables/coverage.tex <==
% Generated by scripts/make_tables.py from data/cells.csv (coverage columns).
\begin{table*}[p]
\tablestyle{2.6pt}{1.04}\scriptsize
\begin{tabular}{@{}l@{\hspace{7pt}}rrrrr@{\hspace{7pt}}rrrrr@{\hspace{7pt}}rrrrr@{}}
\toprule
 & \multicolumn{5}{c}{\textbf{Health} (1,200 planned)} & \multicolumn{5}{c}{\textbf{Coding} (700 planned)} & \multicolumn{5}{c}{\textbf{Math} (1,435 planned)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
\textbf{Model} & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. \\
\midrule
Qwen 3.8 27B & 1,031 & 1,120 & 930 & 614 & 1,122 & 581 & 581 & 199 & 196 & 582 & 1,334 & 1,333 & 1,144 & 1,144 & 1,331 \\
Muse Glimmer 30B & 1,164 & 1,198 & 1,000 & 693 & 1,200 & 681 & 681 & 129 & 120 & 682 & 1,431 & 1,429 & 1,228 & 1,228 & 1,428 \\
GPT-6 Luna & 1,188 & 1,198 & 1,000 & 353 & 1,200 & 699 & 699 & 143 & 143 & 640 & 1,434 & 1,434 & 1,229 & 1,229 & 1,433 \\
Gemini 3.7 Flash & 1,200 & 1,200 & 1,000 & 596 & 1,200 & 700 & 700 & 60 & 60 & 614 & 1,435 & 1,427 & 1,224 & 1,224 & 1,428 \\
Gemini 3.8 Flash & 1,200 & 1,200 & 1,000 & 590 & 1,200 & 700 & 700 & 75 & 75 & 609 & 1,435 & 1,429 & 1,226 & 1,226 & 1,426 \\
Kimi K3 & 1,184 & 1,196 & 1,000 & 627 & 1,200 & 685 & 685 & 106 & 95 & 641 & 1,406 & 1,406 & 1,208 & 1,208 & 1,403 \\
MiniMax M3 & 932\rlap{$^{\circ}$} & 1,140 & 950 & 705 & 1,140 & 676 & 676 & 42 & 39 & 527 & 1,409 & 1,403 & 1,207 & 1,206 & 1,400 \\
DeepSeek V4.1 Flash & 1,141 & 1,176 & 980 & 593 & 1,176 & 697 & 697 & 75 & 73 & 634 & 1,411 & 1,409 & 1,206 & 1,206 & 1,409 \\
GLM 5.3 Flash & 1,120 & 1,188 & 990 & 660 & 1,188 & 443\rlap{$^{\circ}$} & 443 & 131 & 124 & 446 & 1,150 & 1,150 & 984 & 984 & 1,149 \\
Qwen 3.8 Flash & 1,009 & 1,128 & 940 & 585 & 1,128 & 364\rlap{$^{\circ}$} & 364 & 120 & 117 & 370 & 985\rlap{$^{\circ}$} & 985 & 825 & 825 & 985 \\
Claude Haiku 5.5 & 657\rlap{$^{\circ}$} & 1,080 & 900 & 450 & 1,080 & 700 & 700 & 600 & 598 & 700 & 1,435 & 1,435 & 1,230 & 1,229 & 1,435 \\
Claude Sonnet 5.5 & 1,130 & 1,194 & 995 & 620 & 1,194 & 699 & 699 & 599 & 591 & 699 & 1,434 & 1,434 & 1,230 & 1,230 & 1,434 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}1,173\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}999} & {\color{black!45}899} & {\color{black!45}1,200} & 700 & 700 & 136 & 134 & 656 & 1,402 & 1,399 & 1,204 & 1,204 & 1,400 \\
Fable 5.1 & -- &  &  &  &  & 693 & 693 & 594 & 592 & 693 & 1,428 & 1,428 & 1,223 & 1,223 & 1,428 \\
Claude Opus 5.5 & {\color{black!45}1,194\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}1,000} & {\color{black!45}787} & {\color{black!45}1,200} & {\color{black!45}700\rlap{$^{\dagger}$}} & {\color{black!45}700} & {\color{black!45}600} & {\color{black!45}591} & {\color{black!45}700} & 1,432 & 1,432 & 1,225 & 1,224 & 1,430 \\
GPT-5.5 & {\color{black!45}1,199\rlap{$^{\ddagger}$}} & {\color{black!45}1,076} & {\color{black!45}998} & {\color{black!45}636} & {\color{black!45}1,092} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}112} & {\color{black!45}112} & {\color{black!45}653} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}1,435} & {\color{black!45}1,230} & {\color{black!45}1,230} & {\color{black!45}1,432} \\
GPT-5.6 Sol & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}1,128} & {\color{black!45}997} & {\color{black!45}521} & {\color{black!45}1,089} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}143} & {\color{black!45}143} & {\color{black!45}662} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}1,431} & {\color{black!45}1,229} & {\color{black!45}1,229} & {\color{black!45}1,431} \\
GPT-5.6 Terra & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}1,112} & {\color{black!45}1,000} & {\color{black!45}485} & {\color{black!45}1,075} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}103} & {\color{black!45}103} & {\color{black!45}662} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}1,433} & {\color{black!45}1,228} & {\color{black!45}1,228} & {\color{black!45}1,430} \\
GPT-6 Astra & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}1,107} & {\color{black!45}1,000} & {\color{black!45}476} & {\color{black!45}1,097} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}24} & {\color{black!45}24} & {\color{black!45}69} & {\color{black!45}1,434\rlap{$^{\ddagger}$}} & {\color{black!45}1,434} & {\color{black!45}1,229} & {\color{black!45}1,228} & {\color{black!45}1,430} \\
GPT-6 Sol & {\color{black!45}1,187\rlap{$^{\ddagger}$}} & {\color{black!45}1,115} & {\color{black!45}989} & {\color{black!45}395} & {\color{black!45}1,087} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}129} & {\color{black!45}129} & {\color{black!45}660} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}1,435} & {\color{black!45}1,230} & {\color{black!45}1,230} & {\color{black!45}1,434} \\
\midrule
\textit{All runs} & 21,309 & 21,954 & 18,668 & 11,285 & 21,868 & 13,218 & 13,218 & 4,120 & 4,059 & 11,899 & 27,731 & 27,701 & 23,739 & 23,735 & 27,676 \\
\textit{Main cohort} & 12,956 & 14,018 & 11,685 & 7,086 & 14,028 & 9,018 & 9,018 & 3,009 & 2,957 & 8,493 & 20,561 & 20,533 & 17,593 & 17,590 & 20,519 \\
\midrule[\heavyrulewidth]
 & \multicolumn{5}{c}{\textbf{Finance} (1,164 planned)} & \multicolumn{5}{c}{\textbf{Customer Service} (1,452 planned)} & \multicolumn{5}{c}{\textbf{Travel} (432 planned)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
\textbf{Model} & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. \\
\midrule
Qwen 3.8 27B & 1,123 & 1,060 & 1,045 & 1,000 & 1,140 & 1,452 & 1,452 & 1,056 & 751 & 1,452 & 432 & 432 & 349 & 270 & 432 \\
Muse Glimmer 30B & 994 & 1,118 & 1,067 & 1,007 & 1,164 & 1,452 & 1,452 & 1,056 & 754 & 1,452 & 394 & 394 & 336 & 277 & 405 \\
GPT-6 Luna & 1,163 & 1,102 & 1,052 & 867 & 1,162 & 1,452 & 1,452 & 1,025 & 722 & 1,435 & 431 & 431 & 340 & 261 & 430 \\
Gemini 3.7 Flash & 1,164 & 1,065 & 1,064 & 1,033 & 1,159 & 1,452 & 1,452 & 1,056 & 728 & 1,452 & 432 & 432 & 322 & 251 & 432 \\
Gemini 3.8 Flash & 1,164 & 1,090 & 1,060 & 1,009 & 1,158 & 1,452 & 1,452 & 1,056 & 744 & 1,452 & 432 & 432 & 327 & 254 & 432 \\
Kimi K3 & 1,159 & 1,107 & 1,062 & 994 & 1,159 & 1,445 & 1,445 & 1,025 & 719 & 1,445 & 430 & 430 & 308 & 243 & 430 \\
MiniMax M3 & 1,159 & 965 & 1,066 & 1,038 & 1,163 & 1,452 & 1,452 & 1,056 & 768 & 1,452 & 366 & 366 & 266 & 186 & 373 \\
DeepSeek V4.1 Flash & 1,164 & 1,108 & 1,067 & 981 & 1,164 & 1,448 & 1,448 & 1,053 & 748 & 1,452 & 431 & 431 & 333 & 267 & 431 \\
GLM 5.3 Flash & 1,122 & 1,081 & 1,034 & 978 & 1,128 & 1,452 & 1,452 & 1,056 & 756 & 1,452 & 432 & 432 & 341 & 274 & 432 \\
Qwen 3.8 Flash & 937 & 890 & 869 & 822 & 948 & 1,452 & 1,452 & 1,056 & 761 & 1,452 & 432 & 432 & 343 & 268 & 432 \\
Claude Haiku 5.5 & 1,164 & 1,164 & 1,067 & 996 & 1,164 & 1,452 & 1,452 & 1,056 & 774 & 1,452 & 430 & 430 & 360 & 292 & 432 \\
Claude Sonnet 5.5 & 1,164 & 1,164 & 1,067 & 990 & 1,164 & 1,452 & 1,452 & 1,056 & 753 & 1,452 & 432 & 432 & 360 & 294 & 432 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}1,163\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}1,066} & {\color{black!45}1,028} & {\color{black!45}1,163} & 1,446 & 1,446 & 1,052 & 758 & 1,452 & 429 & 429 & 342 & 275 & 430 \\
Fable 5.1 & 1,164 & 1,164 & 1,067 & 1,005 & 1,164 & 1,452 & 1,452 & 1,056 & 754 & 1,452 & 432 & 432 & 360 & 288 & 432 \\
Claude Opus 5.5 & {\color{black!45}1,164\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}1,067} & {\color{black!45}1,035} & {\color{black!45}1,164} & {\color{black!45}1,452\rlap{$^{\dagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}764} & {\color{black!45}1,452} & {\color{black!45}431\rlap{$^{\dagger}$}} & {\color{black!45}431} & {\color{black!45}360} & {\color{black!45}360} & {\color{black!45}432} \\
GPT-5.5 & 1,164 & 1,122 & 1,067 & 982 & 1,164 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}743} & {\color{black!45}1,452} & 431 & 431 & 359 & 291 & 432 \\
GPT-5.6 Sol & 1,164 & 1,146 & 1,067 & 909 & 1,164 & {\color{black!45}1,448\rlap{$^{\ddagger}$}} & {\color{black!45}1,448} & {\color{black!45}1,053} & {\color{black!45}739} & {\color{black!45}1,452} & 426 & 426 & 357 & 270 & 432 \\
GPT-5.6 Terra & 1,164 & 1,130 & 1,067 & 928 & 1,164 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}752} & {\color{black!45}1,452} & 432 & 432 & 359 & 282 & 432 \\
GPT-6 Astra & 1,154 & 1,108 & 1,051 & 846 & 1,134 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}776} & {\color{black!45}1,452} & 428 & 428 & 357 & 264 & 432 \\
GPT-6 Sol & 1,164 & 1,153 & 1,067 & 860 & 1,164 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}746} & {\color{black!45}1,452} & 431 & 431 & 357 & 282 & 432 \\
\midrule
\textit{All runs} & 22,778 & 22,063 & 21,039 & 19,308 & 22,954 & 29,019 & 29,019 & 21,048 & 15,010 & 29,016 & 8,514 & 8,514 & 6,836 & 5,449 & 8,547 \\
\textit{Main cohort} & 20,451 & 19,737 & 18,906 & 17,245 & 20,627 & 20,311 & 20,311 & 14,715 & 10,490 & 20,304 & 8,083 & 8,083 & 6,476 & 5,089 & 8,115 \\
\bottomrule
\end{tabular}
\caption{\textbf{Episode coverage per model and domain.} \emph{Gen.}: episodes whose conversation was generated; a conversation stopped at the turn cap counts as generated, except in Travel, where a capped episode has no primary task score, and in Health, whose single capped conversation is recorded as a failure; \emph{Task}: episodes with a native task grade; \emph{Needs}: persona episodes with a needs judgment (the neutral user has no needs); \emph{Scor.}: persona episodes with at least one need that the user expressed and the assistant had a chance to answer; \emph{Aud.}: episodes with a simulator audit. In Health the task is also graded on the recorded part of dialogues whose generation failed, so Task can exceed Gen. Over all 119 runs, 126,460 episodes were planned, 122,569 generated, 122,469 task-graded, 95,450 needs-judged, 78,846 needs-scoreable and 121,960 audited. Failed and unscored episodes stay in the planned denominators. Gray values mark cells outside the main cohort, with the markers of \tabref{tab:scorecard}; $^{\circ}$ fewer than 80\% of planned episodes generated; -- no run.}
\label{tab:coverage}
\end{table*}


==> old_archive/tables/domain_coding.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/coding_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Pass rate}} & \multicolumn{2}{c}{\textbf{Simulator audit}} & \multicolumn{2}{c}{\textbf{Needs}} & \multicolumn{2}{c}{\textbf{Stops}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & Gen. & Value & $n$ & Planned & Valid & $n$ & Value & $n$ & Cap & Format \\
\midrule
Qwen 3.8 27B & 581 & 87.1 & 565 & 72.3 & 97.8 & 582 & \textbf{95.2} & 190 & 28 & 12 \\
Muse Glimmer 30B & 681 & 69.6 & 618 & 65.4 & 91.8 & 682 & 86.8 & 106 & 314 & 74 \\
GPT-6 Luna & 699 & 84.0 & 630 & 84.3 & 98.4 & 640 & 94.1 & 124 & 36 & 0 \\
Gemini 3.7 Flash & 700 & 87.7 & 593 & 87.1 & 96.6 & 614 & 92.2 & 54 & 139 & 1 \\
Gemini 3.8 Flash & 700 & 88.1 & 595 & 88.6 & 97.7 & 609 & 92.0 & 64 & 100 & 2 \\
Kimi K3 & 685 & 90.1 & 608 & 87.4 & 96.3 & 641 & 94.7 & 85 & 61 & 0 \\
MiniMax M3 & 676 & 67.6 & 479 & 60.3 & 91.7 & 527 & 85.7\rlap{$^{\ast}$} & 19 & 378 & 7 \\
DeepSeek V4.1 Flash & 697 & 88.8 & 618 & 88.1 & 97.6 & 634 & 93.8 & 67 & 58 & 4 \\
GLM 5.3 Flash & 443\rlap{$^{\circ}$} & 92.0 & 426 & 58.1 & 97.3 & 446 & 91.7 & 120 & 32 & 2 \\
Qwen 3.8 Flash & 364\rlap{$^{\circ}$} & 91.2 & 362 & 47.4 & 98.9 & 370 & 94.0 & 116 & 19 & 4 \\
Claude Haiku 5.5 & 700 & 79.0 & 692 & 79.0 & 98.9 & 700 & 86.1 & 590 & 88 & 99 \\
Claude Sonnet 5.5 & 699 & 94.7 & 693 & 94.4 & 99.1 & 699 & 88.2 & 586 & 38 & 4 \\
\addlinespace[2pt]
Grok 4.6 & 700 & 86.8 & 644 & 86.6 & 98.2 & 656 & 92.5 & 123 & 29 & 0 \\
Fable 5.1 & 693 & \textbf{95.5} & 684 & 94.6 & 98.7 & 693 & 90.9 & 585 & 27 & 0 \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}700\rlap{$^{\dagger}$}} & {\color{black!45}94.7\rlap{$^{\dagger}$}} & {\color{black!45}695} & {\color{black!45}94.7} & {\color{black!45}99.3} & {\color{black!45}700} & {\color{black!45}95.4\rlap{$^{\dagger}$}} & {\color{black!45}591} & {\color{black!45}11} & {\color{black!45}0} \\
{\color{black!45}GPT-5.5} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}88.6\rlap{$^{\S}$}} & {\color{black!45}643} & {\color{black!45}88.6} & {\color{black!45}98.5} & {\color{black!45}653} & {\color{black!45}94.8\rlap{$^{\S}$}} & {\color{black!45}102} & {\color{black!45}38} & {\color{black!45}22} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}92.2\rlap{$^{\S}$}} & {\color{black!45}656} & {\color{black!45}92.3} & {\color{black!45}99.1} & {\color{black!45}662} & {\color{black!45}94.9\rlap{$^{\S}$}} & {\color{black!45}129} & {\color{black!45}11} & {\color{black!45}0} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}87.3\rlap{$^{\S}$}} & {\color{black!45}651} & {\color{black!45}87.7} & {\color{black!45}98.3} & {\color{black!45}662} & {\color{black!45}91.3\rlap{$^{\S}$}} & {\color{black!45}89} & {\color{black!45}42} & {\color{black!45}1} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}100.0\rlap{$^{\S}$}} & {\color{black!45}68} & {\color{black!45}97.3} & {\color{black!45}98.6} & {\color{black!45}69} & {\color{black!45}97.3\rlap{$^{\S\ast}$}} & {\color{black!45}19} & {\color{black!45}0} & {\color{black!45}0} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}93.6\rlap{$^{\S}$}} & {\color{black!45}645} & {\color{black!45}93.3} & {\color{black!45}97.7} & {\color{black!45}660} & {\color{black!45}93.9\rlap{$^{\S}$}} & {\color{black!45}117} & {\color{black!45}24} & {\color{black!45}0} \\
\bottomrule
\end{tabular}
\caption{\textbf{Coding: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 700 planned. \emph{Pass rate}: headline (confirmed hidden-test passes of the final submission over completed, simulator-valid episodes) and its $n$; \emph{Planned}: passes over all 700 planned episodes, non-generated ones counted as failures. \emph{Simulator audit}: valid share of audited episodes and the number audited. \emph{Needs}: score over expressed and answered persona-specific needs, with $n$ scoreable eligible persona episodes. \emph{Cap}: conversations stopped at the turn cap; \emph{Format}: final submissions that failed the required format. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. $^{\ast}$ fewer than 50 scoreable episodes. n.r.\ not recorded. Gemini 3.7 / 3.8 Flash follow the original validated judge outputs, as all models do; under the raw-judge score update that their packages also publish they would read Gemini 3.7: task 87.7 ($n$\,=\,674), needs 87.9 ($n$\,=\,578); Gemini 3.8: task 88.3 ($n$\,=\,682), needs 87.5 ($n$\,=\,584).}
\label{tab:domain-coding}
\end{table*}


==> old_archive/tables/domain_customer_service.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/customer_service_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{2}{c}{\textbf{Task}} & \multicolumn{3}{c}{\textbf{Needs}} &  & \multicolumn{3}{c}{\textbf{Failed tasks}} &  \\
\cmidrule(lr){3-4} \cmidrule(lr){5-7} \cmidrule(lr){9-11}
\textbf{Model} & Gen. & Complete & Decision & Value & $n$ & Pass & Sim.\ valid & Decision & Process & Ending & Cap \\
\midrule
Qwen 3.8 27B & 1,452 & 71.3 & 95.8 & 74.0 & 706 & 57.1 & 94.5 & 61 & 294 & 62 & 0 \\
Muse Glimmer 30B & 1,452 & 35.5 & 52.9 & 47.5 & 683 & 32.8 & 92.6 & 684 & 220 & 32 & 23 \\
GPT-6 Luna & 1,452 & 75.2 & 95.2 & 69.2 & 665 & 52.3 & 94.8 & 70 & 222 & 68 & 0 \\
Gemini 3.7 Flash & 1,452 & 92.6 & 96.2 & 75.9 & 677 & 60.8 & 94.1 & 55 & 29 & 23 & 0 \\
Gemini 3.8 Flash & 1,452 & \textbf{94.1} & 97.3 & 78.4 & 695 & 66.3 & 94.7 & 39 & 20 & 26 & 0 \\
Kimi K3 & 1,445 & 74.5 & 90.8 & 79.3 & 682 & 66.1 & 95.1 & 127 & 188 & 48 & 0 \\
MiniMax M3 & 1,452 & 22.7 & 82.2 & 65.2 & 697 & 46.1 & 93.1 & 259 & 836 & 28 & 0 \\
DeepSeek V4.1 Flash & 1,448 & 72.0 & 95.0 & 69.4 & 698 & 51.5 & 94.8 & 69 & 265 & 69 & 0 \\
GLM 5.3 Flash & 1,452 & 56.3 & 92.4 & 74.9 & 719 & 59.1 & 95.0 & 111 & 492 & 32 & 0 \\
Qwen 3.8 Flash & 1,452 & 60.5 & 93.5 & 73.3 & 717 & 56.2 & 95.6 & 94 & 433 & 46 & 0 \\
Claude Haiku 5.5 & 1,452 & 69.6 & 95.7 & 70.2 & 710 & 51.1 & 93.5 & 63 & 282 & 96 & 0 \\
Claude Sonnet 5.5 & 1,452 & 86.8 & 97.2 & 71.0 & 693 & 50.5 & 94.8 & 41 & 58 & 92 & 0 \\
\addlinespace[2pt]
Grok 4.6 & 1,446 & 83.6 & 97.4 & 65.6 & 705 & 52.1 & 94.3 & 32 & 150 & 50 & 0 \\
Fable 5.1 & 1,452 & 87.7 & 96.3 & \textbf{80.2} & 716 & 65.9 & 94.5 & 54 & 74 & 50 & 0 \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}1,452\rlap{$^{\dagger}$}} & {\color{black!45}85.8\rlap{$^{\dagger}$}} & {\color{black!45}97.4} & {\color{black!45}72.4\rlap{$^{\dagger}$}} & {\color{black!45}740} & {\color{black!45}54.3} & {\color{black!45}96.6} & {\color{black!45}38} & {\color{black!45}82} & {\color{black!45}86} & {\color{black!45}0} \\
{\color{black!45}GPT-5.5} & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}89.9\rlap{$^{\ddagger}$}} & {\color{black!45}95.5} & {\color{black!45}78.1\rlap{$^{\ddagger}$}} & {\color{black!45}715} & {\color{black!45}63.9} & {\color{black!45}96.2} & {\color{black!45}66} & {\color{black!45}43} & {\color{black!45}38} & {\color{black!45}0} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}1,448\rlap{$^{\ddagger}$}} & {\color{black!45}88.9\rlap{$^{\ddagger}$}} & {\color{black!45}95.7} & {\color{black!45}78.5\rlap{$^{\ddagger}$}} & {\color{black!45}702} & {\color{black!45}67.7} & {\color{black!45}95.0} & {\color{black!45}58} & {\color{black!45}49} & {\color{black!45}50} & {\color{black!45}0} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}89.3\rlap{$^{\ddagger}$}} & {\color{black!45}97.7} & {\color{black!45}72.9\rlap{$^{\ddagger}$}} & {\color{black!45}696} & {\color{black!45}57.2} & {\color{black!45}94.3} & {\color{black!45}33} & {\color{black!45}80} & {\color{black!45}43} & {\color{black!45}0} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}97.2} & {\color{black!45}76.3\rlap{$^{\ddagger}$}} & {\color{black!45}744} & {\color{black!45}61.9} & {\color{black!45}96.3} & {\color{black!45}41} & {\color{black!45}99} & {\color{black!45}111} & {\color{black!45}0} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}82.2\rlap{$^{\ddagger}$}} & {\color{black!45}97.5} & {\color{black!45}74.3\rlap{$^{\ddagger}$}} & {\color{black!45}719} & {\color{black!45}58.8} & {\color{black!45}95.9} & {\color{black!45}37} & {\color{black!45}141} & {\color{black!45}80} & {\color{black!45}0} \\
\bottomrule
\end{tabular}
\caption{\textbf{Customer Service: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 1,452 planned. \emph{Task}: headline rule-based completion over all 1{,}452 planned episodes (policy-correct decision, required look-ups, matching execution and ending; incomplete episodes count 0) and the policy decision alone. \emph{Needs}: score over simulator-valid completed persona episodes, its $n$, and persona pass (every critical need met). \emph{Sim.\ valid}: valid share of audited completed episodes. \emph{Failed tasks}: graded episodes that were not completed, by first failure: wrong decision, process gap (right decision without the required look-ups or execution), or wrong ending. \emph{Cap}: conversations stopped at the 24-message cap. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. For Gemini 3.7 / 3.8 Flash the raw-judge score update published by their packages gives the same headline values.}
\label{tab:domain-customer-service}
\end{table*}


==> old_archive/tables/domain_finance.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/finance_cells.csv.
\begin{table*}[tb]
\tablestyle{3.6pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{4}{c}{\textbf{Rubric percent}} & \multicolumn{3}{c}{\textbf{Pass rates}} & \multicolumn{2}{c}{\textbf{Needs}} &  &  &  \\
\cmidrule(lr){3-6} \cmidrule(lr){7-9} \cmidrule(lr){10-11}
\textbf{Model} & Gen. & All & $n$ & Persona & Neutral & Advice & Persona & Joint & Value & $n$ & Sim.\ valid & Cap & Turns \\
\midrule
Qwen 3.8 27B & 1,123 & 45.4 & 1,060 & 45.4 & 45.2 & 40.0 & 11.5 & 4.4 & 56.7 & 1,000 & 92.5 & 140 & 4.1 \\
Muse Glimmer 30B & 994 & 35.4 & 1,118 & 35.3 & 36.0 & 24.0 & 21.0 & 5.8 & 62.7 & 1,007 & 92.1 & 73 & 3.3 \\
GPT-6 Luna & 1,163 & 35.7 & 1,102 & 35.8 & 33.9 & 21.6 & 63.0 & 13.4 & \textbf{90.1} & 867 & 96.6 & 4 & 2.1 \\
Gemini 3.7 Flash & 1,164 & 43.5 & 1,065 & 43.9 & 39.2 & 39.3 & 12.9 & 3.9 & 61.4 & 1,033 & 92.5 & 291 & 4.6 \\
Gemini 3.8 Flash & 1,164 & 45.1 & 1,090 & 45.2 & 43.4 & 41.4 & 13.9 & 6.2 & 63.1 & 1,009 & 92.6 & 256 & 4.5 \\
Kimi K3 & 1,159 & 47.2 & 1,107 & 47.2 & 46.6 & 44.5 & 24.7 & 9.5 & 68.5 & 994 & 94.1 & 103 & 3.4 \\
MiniMax M3 & 1,159 & 43.1 & 965 & 43.2 & 42.5 & 40.1 & 11.2 & 4.3 & 55.4 & 1,038 & 93.3 & 237 & 4.6 \\
DeepSeek V4.1 Flash & 1,164 & 44.0 & 1,108 & 44.2 & 42.2 & 36.3 & 35.5 & 11.3 & 77.8 & 981 & 96.6 & 22 & 2.8 \\
GLM 5.3 Flash & 1,122 & 46.9 & 1,081 & 47.0 & 45.5 & 45.2 & 19.6 & 8.8 & 66.3 & 978 & 94.3 & 98 & 3.5 \\
Qwen 3.8 Flash & 937 & 48.7 & 890 & 49.0 & 45.2 & 49.1 & 12.4 & 6.0 & 57.2 & 822 & 93.6 & 104 & 3.8 \\
Claude Haiku 5.5 & 1,164 & 37.6 & 1,164 & 37.8 & 35.4 & 22.6 & 29.0 & 6.6 & 74.1 & 996 & 94.4 & 64 & 3.1 \\
Claude Sonnet 5.5 & 1,164 & 52.3 & 1,164 & 52.3 & 52.2 & 55.3 & 26.9 & 16.2 & 72.7 & 990 & 95.3 & 23 & 2.8 \\
\addlinespace[2pt]
{\color{black!45}Grok 4.6} & {\color{black!45}1,163\rlap{$^{\dagger}$}} & {\color{black!45}51.5\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}51.5} & {\color{black!45}51.1} & {\color{black!45}55.1} & {\color{black!45}44.6} & {\color{black!45}24.6} & {\color{black!45}80.4\rlap{$^{\dagger}$}} & {\color{black!45}1,028} & {\color{black!45}96.0} & {\color{black!45}25} & {\color{black!45}2.9} \\
Fable 5.1 & 1,164 & \textbf{57.1} & 1,164 & 57.2 & 56.0 & 67.9 & 25.2 & 16.8 & 70.1 & 1,005 & 94.2 & 58 & 3.1 \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}1,164\rlap{$^{\dagger}$}} & {\color{black!45}64.6\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}64.7} & {\color{black!45}63.6} & {\color{black!45}77.4} & {\color{black!45}39.0} & {\color{black!45}29.8} & {\color{black!45}77.9\rlap{$^{\dagger}$}} & {\color{black!45}1,035} & {\color{black!45}98.0} & {\color{black!45}25} & {\color{black!45}2.8} \\
GPT-5.5 & 1,164 & 48.8 & 1,122 & 49.2 & 44.8 & 53.1 & 33.9 & 17.2 & 78.7 & 982 & 93.9 & 29 & 2.6 \\
GPT-5.6 Sol & 1,164 & 50.6 & 1,146 & 50.8 & 48.7 & 53.5 & 46.7 & 23.6 & 85.3 & 909 & 95.6 & 2 & 2.1 \\
GPT-5.6 Terra & 1,164 & 47.3 & 1,130 & 47.5 & 45.3 & 43.5 & 43.9 & 19.6 & 82.6 & 928 & 94.2 & 3 & 2.2 \\
GPT-6 Astra & 1,154 & 50.6 & 1,108 & 50.8 & 48.1 & 53.9 & 62.9 & 32.9 & 90.0 & 846 & 96.4 & 2 & 2.0 \\
GPT-6 Sol & 1,164 & 36.0 & 1,153 & 36.2 & 34.2 & 21.6 & 58.7 & 12.8 & 88.8 & 860 & 94.8 & 7 & 2.1 \\
\bottomrule
\end{tabular}
\caption{\textbf{Finance: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 1,164 planned. \emph{Rubric percent}: headline PRBench expert-rubric percent over the whole conversation for all 12 conditions, its $n$, and separately for the 11 persona conditions and the neutral user. \emph{Pass rates} (persona conditions only): advice pass (rubric percent $\geq 50$), persona pass (every critical need expressed, answered and met) and both together. \emph{Needs}: score over expressed and answered needs (strict needs mode) and $n$ scoreable persona episodes. \emph{Sim.\ valid}: valid share of audited episodes. \emph{Cap}: conversations stopped at the 8-turn cap; \emph{Turns}: mean assistant turns per generated conversation. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. Gemini 3.7 / 3.8 Flash follow the original validated judge outputs, as all models do; under the raw-judge score update that their packages also publish they would read Gemini 3.7: task 44.1 ($n$\,=\,1,164), needs 61.7 ($n$\,=\,1,036); Gemini 3.8: task 45.5 ($n$\,=\,1,164), needs 63.5 ($n$\,=\,1,016).}
\label{tab:domain-finance}
\end{table*}


==> old_archive/tables/domain_health.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/health_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{4}{c}{\textbf{Inquiry coverage}} &  & \multicolumn{4}{c}{\textbf{Needs}} &  \\
\cmidrule(lr){3-6} \cmidrule(lr){8-11}
\textbf{Model} & Gen. & Value & $n$ & Fail${=}0$ & Partial & Facts & Value & $n$ & Expr. & Opp. & Attr. \\
\midrule
Qwen 3.8 27B & 1,031 & 40.0 & 1,120 & 37.4 & 54.2 & 65.1 & 78.8 & 614 & 51.4 & 96.7 & 49.1 \\
Muse Glimmer 30B & 1,164 & 46.3 & 1,198 & 46.3 & 60.4 & 71.7 & 82.6 & 693 & 47.7 & 99.2 & 46.9 \\
GPT-6 Luna & 1,188 & 27.0 & 1,198 & 27.0 & 39.7 & 45.5 & \textbf{96.5} & 353 & 24.6 & 100.0 & 44.0 \\
Gemini 3.7 Flash & 1,200 & 32.9 & 1,200 & 32.9 & 47.1 & 52.9 & 83.9 & 596 & 44.7 & 100.0 & 54.0 \\
Gemini 3.8 Flash & 1,200 & 32.1 & 1,200 & 32.1 & 45.7 & 51.8 & 83.1 & 590 & 45.2 & 100.0 & 53.9 \\
Kimi K3 & 1,184 & 40.6 & 1,196 & 40.5 & 56.5 & 66.3 & 91.5 & 627 & 45.2 & 100.0 & 47.9 \\
MiniMax M3 & 932\rlap{$^{\circ}$} & \textbf{46.8} & 1,140 & 44.5 & 62.3 & 70.6 & 80.1 & 705 & 57.2 & 94.2 & 50.8 \\
DeepSeek V4.1 Flash & 1,141 & 39.9 & 1,176 & 39.1 & 55.3 & 63.9 & 93.9 & 593 & 42.1 & 98.8 & 46.5 \\
GLM 5.3 Flash & 1,120 & 40.4 & 1,188 & 40.0 & 55.3 & 62.6 & 88.0 & 660 & 49.7 & 98.2 & 49.2 \\
Qwen 3.8 Flash & 1,009 & 39.7 & 1,128 & 37.3 & 54.4 & 63.0 & 77.4 & 585 & 49.0 & 96.0 & 48.7 \\
Claude Haiku 5.5 & 657\rlap{$^{\circ}$} & 39.8 & 1,080 & 35.9 & 54.5 & 61.4 & 91.7 & 450 & 39.7 & 86.4 & 41.0 \\
Claude Sonnet 5.5 & 1,130 & 41.5 & 1,194 & 41.3 & 56.8 & 63.5 & 90.1 & 620 & 43.6 & 97.1 & 43.8 \\
\addlinespace[2pt]
{\color{black!45}Grok 4.6} & {\color{black!45}1,173\rlap{$^{\dagger}$}} & {\color{black!45}45.1\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}45.0} & {\color{black!45}59.0} & {\color{black!45}63.7} & {\color{black!45}97.0\rlap{$^{\dagger}$}} & {\color{black!45}899} & {\color{black!45}57.8} & {\color{black!45}99.9} & {\color{black!45}72.2} \\
{\color{black!45}Fable 5.1} & \multicolumn{11}{l}{\textit{no run}} \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}1,194\rlap{$^{\dagger}$}} & {\color{black!45}45.7\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}45.7} & {\color{black!45}59.9} & {\color{black!45}65.6} & {\color{black!45}91.6\rlap{$^{\dagger}$}} & {\color{black!45}787} & {\color{black!45}55.6} & {\color{black!45}100.0} & {\color{black!45}63.2} \\
{\color{black!45}GPT-5.5} & {\color{black!45}1,199\rlap{$^{\ddagger}$}} & {\color{black!45}40.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,076} & {\color{black!45}36.5} & n.r. & {\color{black!45}65.3} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}636} & {\color{black!45}44.6} & {\color{black!45}100.0} & {\color{black!45}47.7} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}35.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,128} & {\color{black!45}33.7} & n.r. & {\color{black!45}58.2} & {\color{black!45}97.2\rlap{$^{\ddagger}$}} & {\color{black!45}521} & {\color{black!45}36.2} & {\color{black!45}100.0} & {\color{black!45}45.9} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}34.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,112} & {\color{black!45}31.8} & n.r. & {\color{black!45}56.8} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}485} & {\color{black!45}33.2} & {\color{black!45}100.0} & {\color{black!45}43.7} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}34.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,107} & {\color{black!45}31.7} & n.r. & {\color{black!45}55.7} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}476} & {\color{black!45}33.1} & {\color{black!45}100.0} & {\color{black!45}44.0} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}1,187\rlap{$^{\ddagger}$}} & {\color{black!45}26.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,115} & {\color{black!45}24.8} & n.r. & {\color{black!45}44.5} & {\color{black!45}98.0\rlap{$^{\ddagger}$}} & {\color{black!45}395} & {\color{black!45}27.8} & {\color{black!45}100.0} & {\color{black!45}45.7} \\
\bottomrule
\end{tabular}
\caption{\textbf{Health: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 1,200 planned. \emph{Inquiry coverage}: headline (share of applicable source inquiry criteria fully met, over all planned episodes with a task score) and its $n$; \emph{Fail${=}0$}: the same over all 1{,}200 planned episodes with generation failures scored 0; \emph{Partial}: coverage with partial credit for partly met criteria (n.r.\ in score-only packages). \emph{Facts}: share of the patient's source facts the doctor acquired. \emph{Needs}: persona-needs score and $n$ scoreable persona episodes; \emph{Expr.}: share of applicable need items the patient expressed; \emph{Opp.}: share of expressed items the doctor had a chance to answer. \emph{Attr.}: share of persona attributes the simulated patient demonstrated (simulator audit evidence; the Health audit is advisory and has no valid/invalid label). Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. For Gemini 3.7 / 3.8 Flash the raw-judge score update published by their packages gives the same headline values.}
\label{tab:domain-health}
\end{table*}


==> old_archive/tables/domain_math.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/math_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{6}{c}{\textbf{Tutor correctness}} &  &  & \multicolumn{2}{c}{\textbf{Needs}} &  \\
\cmidrule(lr){3-8} \cmidrule(lr){11-12}
\textbf{Model} & Gen. & Value & $n$ & Arena & HARP & IMO & Neutral & Student & Strict & Value & $n$ & Sim.\ valid \\
\midrule
Qwen 3.8 27B & 1,334 & 91.1 & 1,143 & 98.6 & 90.5 & 79.2 & 87.9 & 98.5 & 58.7 & 81.8 & 1,144 & 99.4 \\
Muse Glimmer 30B & 1,431 & 81.6 & 1,226 & 99.1 & 86.3 & 36.8 & 82.3 & 93.9 & 40.4 & 58.0 & 1,228 & 99.4 \\
GPT-6 Luna & 1,434 & 91.5 & 1,229 & 99.5 & 94.4 & 67.6 & 91.2 & 95.9 & 84.4 & 85.8 & 1,229 & 99.8 \\
Gemini 3.7 Flash & 1,435 & 89.0 & 1,223 & 99.5 & 92.3 & 59.9 & 88.2 & 97.1 & 76.2 & 84.4 & 1,224 & 99.4 \\
Gemini 3.8 Flash & 1,435 & 89.5 & 1,225 & 99.1 & 93.4 & 58.6 & 88.7 & 96.9 & 75.0 & 86.2 & 1,226 & 98.9 \\
Kimi K3 & 1,406 & 92.4 & 1,208 & 98.2 & 94.8 & 72.4 & 90.9 & 97.8 & 68.1 & 84.1 & 1,208 & 99.4 \\
MiniMax M3 & 1,409 & 80.8 & 1,201 & 98.2 & 83.1 & 43.6 & 80.2 & 91.2 & 22.6 & 64.5 & 1,206 & 97.0 \\
DeepSeek V4.1 Flash & 1,411 & 94.5 & 1,206 & 99.5 & 95.2 & 83.3 & 93.6 & 99.3 & 85.7 & 81.5 & 1,206 & 99.9 \\
GLM 5.3 Flash & 1,150 & 94.0 & 984 & 97.7 & 92.7 & 97.1 & 95.2 & 97.6 & 53.3 & 83.8 & 984 & 99.5 \\
Qwen 3.8 Flash & 985\rlap{$^{\circ}$} & \textbf{97.7} & 825 & 98.6 & 97.3 & 100.0 & 98.1 & 99.4 & 87.3 & 85.7 & 825 & 99.7 \\
Claude Haiku 5.5 & 1,435 & 90.7 & 1,230 & 99.1 & 95.6 & 56.9 & 88.3 & 96.5 & 70.3 & 85.3 & 1,229 & 99.2 \\
Claude Sonnet 5.5 & 1,434 & 95.3 & 1,230 & 100.0 & 97.2 & 79.9 & 95.6 & 98.4 & 74.5 & 86.6 & 1,230 & 99.7 \\
\addlinespace[2pt]
Grok 4.6 & 1,402 & 91.9 & 1,203 & 98.6 & 93.2 & 74.5 & 92.3 & 98.5 & 76.2 & 79.9 & 1,204 & 99.5 \\
Fable 5.1 & 1,428 & 96.4 & 1,223 & 100.0 & 96.8 & 89.8 & 96.6 & 99.0 & 77.1 & 89.8 & 1,223 & 99.8 \\
Claude Opus 5.5 & 1,432 & 97.4 & 1,227 & 100.0 & 97.5 & 93.6 & 99.0 & 99.5 & 84.4 & \textbf{90.5} & 1,224 & 99.5 \\
{\color{black!45}GPT-5.5} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}92.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}98.6} & {\color{black!45}93.3} & {\color{black!45}79.9} & {\color{black!45}93.2} & {\color{black!45}99.0} & {\color{black!45}85.4} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}99.7} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}95.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}100.0} & {\color{black!45}95.8} & {\color{black!45}86.1} & {\color{black!45}95.1} & {\color{black!45}98.2} & {\color{black!45}87.9} & {\color{black!45}85.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & {\color{black!45}99.9} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}88.8\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}99.1} & {\color{black!45}91.5} & {\color{black!45}62.6} & {\color{black!45}88.3} & {\color{black!45}95.8} & {\color{black!45}78.3} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}99.6} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}1,434\rlap{$^{\ddagger}$}} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & {\color{black!45}99.5} & {\color{black!45}98.8} & {\color{black!45}97.1} & {\color{black!45}99.0} & {\color{black!45}98.7} & {\color{black!45}96.1} & {\color{black!45}91.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}99.7} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}95.0\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}98.6} & {\color{black!45}96.3} & {\color{black!45}84.5} & {\color{black!45}97.6} & {\color{black!45}97.6} & {\color{black!45}89.7} & {\color{black!45}89.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}99.5} \\
\bottomrule
\end{tabular}
\caption{\textbf{Math: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 1,435 planned. \emph{Tutor correctness}: headline (the tutor's final or endorsed solution is correct with valid support) over persona episodes with a tutor grade, its $n$, the same by task bank (SimulatorArena-MATH, HARP, IMO-ProofBench) and for the neutral student. \emph{Student}: the student's final answer is correct; \emph{Strict}: tutor solution correct and free of errors. \emph{Needs}: score over expressed and answered needs and $n$ scoreable persona episodes. \emph{Sim.\ valid}: share of audited episodes whose simulated student passed the persona check. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. Gemini 3.7 / 3.8 Flash follow the original validated judge outputs, as all models do; under the raw-judge score update that their packages also publish they would read Gemini 3.7: task 88.8 ($n$\,=\,1,230), needs 84.4 ($n$\,=\,1,230); Gemini 3.8: task 89.5 ($n$\,=\,1,230), needs 86.1 ($n$\,=\,1,230).}
\label{tab:domain-math}
\end{table*}


==> old_archive/tables/domain_travel.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/travel_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{4}{c}{\textbf{Choice reward}} &  & \multicolumn{3}{c}{\textbf{Needs}} &  \\
\cmidrule(lr){3-6} \cmidrule(lr){8-10}
\textbf{Model} & Gen. & Value & $n$ & Valid only & $n$ & Revision & Value & $n$ & Pass & Sim.\ valid \\
\midrule
Qwen 3.8 27B & 432 & 63.9 & 402 & 64.5 & 371 & 100.0 & 91.1 & 270 & 82.4 & 92.8 \\
Muse Glimmer 30B & 394 & 54.7 & 364 & 56.2 & 325 & 73.3 & 93.7 & 277 & 69.5 & 89.9 \\
GPT-6 Luna & 431 & 47.7 & 401 & 50.1 & 354 & 100.0 & 87.1 & 261 & 88.9 & 89.3 \\
Gemini 3.7 Flash & 432 & \textbf{86.6} & 402 & 87.0 & 386 & 100.0 & 85.2 & 251 & 71.4 & 96.3 \\
Gemini 3.8 Flash & 432 & 76.3 & 402 & 76.8 & 380 & 100.0 & 88.1 & 254 & 82.6 & 94.9 \\
Kimi K3 & 430 & 71.1 & 400 & 71.9 & 364 & 100.0 & 88.2 & 243 & 75.9 & 91.9 \\
MiniMax M3 & 366 & 38.4 & 336 & 39.5 & 306 & 63.3 & 88.8 & 186 & 64.7 & 91.7 \\
DeepSeek V4.1 Flash & 431 & 73.6 & 401 & 74.3 & 368 & 100.0 & 85.5 & 267 & 80.2 & 92.3 \\
GLM 5.3 Flash & 432 & 64.2 & 402 & 64.1 & 380 & 93.3 & 86.3 & 274 & 69.4 & 94.4 \\
Qwen 3.8 Flash & 432 & 66.6 & 402 & 67.1 & 377 & 100.0 & 87.6 & 268 & 78.2 & 94.2 \\
Claude Haiku 5.5 & 430 & 40.3 & 400 & 41.3 & 365 & 100.0 & 93.0 & 292 & 79.7 & 91.9 \\
Claude Sonnet 5.5 & 432 & 79.3 & 402 & 79.6 & 380 & 100.0 & 84.2 & 294 & 86.2 & 94.9 \\
\addlinespace[2pt]
Grok 4.6 & 429 & 75.6 & 399 & 77.9 & 355 & 100.0 & 85.2 & 275 & 80.6 & 89.8 \\
Fable 5.1 & 432 & 79.7 & 402 & 80.2 & 377 & 100.0 & 87.8 & 288 & 80.9 & 94.2 \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}431\rlap{$^{\dagger}$}} & {\color{black!45}63.7\rlap{$^{\dagger}$}} & {\color{black!45}401} & {\color{black!45}64.7} & {\color{black!45}367} & {\color{black!45}100.0} & {\color{black!45}93.1\rlap{$^{\dagger}$}} & {\color{black!45}360} & {\color{black!45}70.9} & {\color{black!45}92.1} \\
GPT-5.5 & 431 & 64.2 & 401 & 63.9 & 377 & 100.0 & 91.0 & 291 & 95.8 & 94.4 \\
GPT-5.6 Sol & 426 & 52.6 & 396 & 54.2 & 348 & 80.0 & 87.6 & 270 & 87.5 & 88.9 \\
GPT-5.6 Terra & 432 & 66.8 & 402 & 67.9 & 374 & 80.0 & 88.3 & 282 & 95.3 & 93.3 \\
GPT-6 Astra & 428 & 44.0 & 398 & 44.4 & 345 & 100.0 & \textbf{94.0} & 264 & 95.9 & 87.3 \\
GPT-6 Sol & 431 & 41.2 & 401 & 42.1 & 360 & 100.0 & 90.1 & 282 & 89.4 & 90.3 \\
\bottomrule
\end{tabular}
\caption{\textbf{Travel: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 432 planned. \emph{Choice reward}: headline UserBench reward (1 / 0.8 / 0 per requested aspect, averaged over the two aspects) over recorded official-task episodes with a score, its $n$, and the same over simulator-valid completed episodes only (\emph{Valid only}). \emph{Revision}: final-state success on the five authored revision tasks (30 episodes per model), never pooled with the reward. \emph{Needs}: score over expressed and answered needs, its $n$, and persona pass (critical needs met, among episodes with a decided pass). \emph{Sim.\ valid}: valid share of audited episodes. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. Gemini 3.7 / 3.8 Flash follow the original validated judge outputs, as all models do; under the raw-judge score update that their packages also publish they would read Gemini 3.7: task 86.6 ($n$\,=\,402), needs 85.7 ($n$\,=\,289); Gemini 3.8: task 76.3 ($n$\,=\,402), needs 88.6 ($n$\,=\,287).}
\label{tab:domain-travel}
\end{table*}


==> old_archive/tables/domains.tex <==
% Generated by scripts/make_tables.py from data/domain_facts.json, data/cells.csv and data/*_episodes.csv.gz.
\begin{table*}[t]
\tablestyle{3pt}{1.1}\scriptsize
\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}p{1.55cm} *{6}{>{\raggedright\arraybackslash}X}@{}}
\toprule
 & \textbf{Health} & \textbf{Coding} & \textbf{Math} & \textbf{Finance} & \textbf{Customer Service} & \textbf{Travel} \\
\midrule
\textbf{Source benchmark} & MedDialogRubrics\newline\citep{gong2026meddialogrubrics} & LiveCodeBench\newline\citep{jain2024livecodebench} & SimulatorArena-MATH, HARP, IMO-ProofBench\newline\citep{dou2025simulatorarena,yue2024harp,luong2025imoproofbench} & PRBench-Finance\newline\citep{akyurek2025prbench} & ABCD\newline\citep{chen2021abcd} & UserBench (Travel-44)\newline\citep{qian2025userbench} \\
\addlinespace[1.5pt]
\textbf{Tasks} & 200 cases with inquiry rubrics & 100 selected questions & 205: 37 SimulatorArena, 139 HARP, 29 IMO & 97 questions (finance hard split) & 132 policy items & 72: 67 official + 5 authored revision \\
\addlinespace[1.5pt]
\textbf{Assistant / user} & doctor / patient & coding assistant / developer & tutor / student & financial advisor / client & service agent with policy and tools / customer & travel agent with tools / traveler \\
\addlinespace[1.5pt]
\textbf{Conditions} & 5 personas + neutral & 6 personas + neutral & 6 personas + neutral & 11 personas + neutral (6 shared presets and 5 personas written for each task) & 8 personas + neutral (neutral run 3 times per task) & 5 personas + neutral \\
\addlinespace[1.5pt]
\textbf{Episodes / model} & 1,200 & 700 & 1,435 & 1,164 & 1,452 & 432 \\
\addlinespace[1.5pt]
\textbf{Turn cap} & 20 doctor replies (incl. shared first reply) & 5 assistant turns, then a final submission & 25 tutor turns & 8 assistant turns & 24 agent messages incl. tool follow-ups & 10 assistant replies \\
\addlinespace[1.5pt]
\textbf{Native task metric} & Inquiry coverage: share of applicable source inquiry criteria fully met & Hidden tests passed by the final submission & Tutor's final or endorsed solution correct with valid support (0/1) & Expert rubric percent over the whole conversation (0--100) & Rule-based completion: correct decision, required look-ups, matching action and ending & Choice reward (1 / 0.8 / 0 per aspect) on official tasks; authored tasks scored separately \\
\addlinespace[1.5pt]
\textbf{Needs scored} & Needs expressed, answered and observable & Expressed and answered persona-specific needs & Expressed and answered needs & Expressed and answered needs (strict needs mode) & Expressed and answered needs, simulator-valid episodes & Expressed and answered needs \\
\addlinespace[1.5pt]
\textbf{Simulator audit} & Advisory; no valid/invalid label & Valid / invalid / uncertain; both scores use valid episodes & Valid / invalid & Valid / invalid / uncertain & Valid / invalid / uncertain; needs score uses valid episodes & Valid / invalid / uncertain \\
\addlinespace[1.5pt]
\textbf{Models} & 12 / 19 & 14 / 20 & 15 / 20 & 18 / 20 & 14 / 20 & 19 / 20 \\
\bottomrule
\end{tabularx}
\caption{\textbf{The six domains.} Each column gives a domain's source benchmark and native task metric, its roles (tested assistant / simulated user), the persona conditions beside the neutral user, the planned episodes per model, that is, tasks $\times$ (persona conditions + neutral trials), with 126,460 planned episodes over the 119 runs, the turn cap (a limit, not a target), the needs that enter the persona-needs score and the simulator audit. \emph{Models}: models in the main cohort / models with a run (\tabref{tab:models}). The shared first reply and its exceptions are described in \secref{sec:protocol}, the three judgments in \secref{sec:judgments} and the task populations in \tabref{tab:scorecard-full}.}
\label{tab:domains}
\end{table*}


==> old_archive/tables/models.tex <==
% Generated by scripts/make_tables.py from data/models.csv and data/cells.csv.
\begin{table*}[t]
\tablestyle{2.5pt}{1.08}\scriptsize
\begin{tabular}{@{}llll>{\raggedright\arraybackslash}p{2.55cm}@{\hspace{5pt}} *{6}{r@{\hspace{6.5pt}}} l@{}}
\toprule
 & & & & & \multicolumn{6}{c}{\textbf{Output budget ($10^3$ tokens)}} & \\
\cmidrule(lr){6-11}
\textbf{Model} & \textbf{Developer} & \textbf{Serving} & \textbf{Thinking} & \textbf{Simulator \& judges} & \textbf{H} & \textbf{C} & \textbf{M} & \textbf{F} & \textbf{S} & \textbf{T} & \textbf{Main cohort} \\
\midrule
Qwen 3.8 27B & Qwen Team, Alibaba & Local vLLM & medium & Luna-m & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 6 \\
Muse Glimmer 30B & n.r. & Local vLLM & medium & Luna-m & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 6 \\
GPT-6 Luna & OpenAI & Hosted API & medium & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
Gemini 3.7 Flash & Google DeepMind & GCP-routed API & medium & Luna-m & n.r. & 32.8\rlap{$^{r}$} & 20 & n.r. & n.r. & 8.2 & 6 \\
Gemini 3.8 Flash & Google DeepMind & GCP-routed API & medium & Luna-m & n.r. & 32.8\rlap{$^{r}$} & 20 & n.r. & n.r. & 8.2 & 6 \\
Kimi K3 & Moonshot AI & Hosted API & medium & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
MiniMax M3 & MiniMax & Hosted API & off & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
DeepSeek V4.1 Flash & DeepSeek & Hosted API & low & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
GLM 5.3 Flash & Zhipu AI & Hosted gateway & medium & Luna-m & 12 & 32.8 & 10 & 10 & 10 & 10 & 6 \\
Qwen 3.8 Flash & Qwen Team, Alibaba & Hosted gateway & medium & Luna-m & 12 & 32.8 & 10 & 10 & 10 & 10 & 6 \\
Claude Haiku 5.5 & Anthropic & AWS Bedrock & medium & Luna-m & 12 & 32.8\rlap{$^{r}$} & 12.3\rlap{$^{r}$} & 12.3\rlap{$^{r}$} & n.r.\rlap{$^{r}$} & 8.2 & 6 \\
Claude Sonnet 5.5 & Anthropic & AWS Bedrock & medium & Luna-m & 12 & 32.8\rlap{$^{r}$} & 12.3\rlap{$^{r}$} & 12.3 & n.r.\rlap{$^{r}$} & 8.2 & 6 \\
\midrule
Grok 4.6 & xAI & Hosted API & medium; high (H,F) & Luna-m; Sol-h (H,F) & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 4 (C,M,S,T) \\
Fable 5.1 & Anthropic & AWS Bedrock & medium & Luna-m & -- & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 5 (C,M,F,S,T) \\
Claude Opus 5.5 & Anthropic & AWS Bedrock & high; medium (M) & Sol-h; Luna-m (M); Sol-h/Luna-m (H,S) & n.r. & 128 & n.r. & 12.3\rlap{$^{r}$} & n.r. & 8.2 & 1 (M) \\
GPT-5.5 & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-5.6 Sol & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-5.6 Terra & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-6 Astra & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-6 Sol & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
\bottomrule
\end{tabular}
\caption{\textbf{Tested models.} The first 12 models are in the main cohort of all six domains (H Health, C Coding, M Math, F Finance, S Customer Service, T Travel). \emph{Developer}: attributed from the model family, as the run records give only model identifiers. \emph{Thinking}: the tested assistant's reasoning setting. \emph{Simulator \& judges}: the model behind the simulated user, the task and needs judges and the simulator audit; Luna-m = GPT-6 Luna at medium effort, Sol-h = GPT-5.6 Sol at high effort, Sol-h/Luna-m = differs by condition (H) or by episode (S), Luna-h/n.r.\ = GPT-6 Luna at high or unrecorded effort by role. \emph{Output budget}: the tested assistant's maximum output tokens; $^{r}$ = failed generations rerun under a documented recovery amendment with a budget of 65,536 tokens and kept in the headline (for Claude Haiku 5.5 and Claude Sonnet 5.5 in Customer Service, the only recorded budget); separately reported recoveries are not marked. n.r.\ = not recorded; -- = no run. \emph{Main cohort}: number of domains in whose main cohort (\secref{sec:cohorts}) the run lies.}
\label{tab:models}
\end{table*}


==> old_archive/tables/persona_effects.tex <==
% Generated by scripts/make_tables.py from data/persona_effects.csv (main-cohort rows only).
\begin{table*}[p]
\tablestyle{4pt}{1.04}\scriptsize
\begin{tabular}{@{}l r rrrr rr@{}}
\toprule
 & & \multicolumn{4}{c}{\textbf{Persona $-$ neutral (points)}} & \multicolumn{2}{c}{\textbf{95\% CI excludes 0}} \\
\cmidrule(lr){3-6} \cmidrule(l){7-8}
\textbf{Condition} & \textbf{Models} & \textbf{Mean} & \textbf{Median} & \textbf{Min} & \textbf{Max} & \textbf{Below} & \textbf{Above} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Health} \textit{(inquiry coverage; neutral mean 39.9 over 12 main-cohort models)}} \\
\hspace{0.6em}P1: Receptive novice & 12 & $-$2.9 & $-$2.9 & $-$5.9 & $-$0.6 & 8 & 0 \\
\hspace{0.6em}P2: Informed questioner & 12 & $+$2.2 & $+$1.8 & $-$0.1 & $+$5.7 & 0 & 6 \\
\hspace{0.6em}P3: Private, time-conscious novice & 12 & $-$3.8 & $-$3.6 & $-$5.7 & $-$2.2 & 12 & 0 \\
\hspace{0.6em}P4: Guarded, time-conscious novice & 12 & $-$3.2 & $-$3.0 & $-$5.2 & $-$1.4 & 11 & 0 \\
\hspace{0.6em}P5: Receptive, informed contributor & 12 & $+$2.1 & $+$2.3 & $-$1.4 & $+$5.2 & 0 & 8 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{All personas pooled} & 12 & $-$1.1 & $-$1.1 & $-$3.1 & $+$0.1 & 5 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Coding} \textit{(pass rate; neutral mean 87.1 over 14 main-cohort models)}} \\
\hspace{0.6em}495132: Detailed typed professional & 14 & $-$10.3 & $-$7.7 & $-$30.0 & $+$4.0 & 7 & 0 \\
\hspace{0.6em}518717: Performance-focused student & 14 & $-$2.5 & $-$1.5 & $-$10.1 & $+$5.6 & 3 & 0 \\
\hspace{0.6em}690429: Deadline-driven technologist & 14 & $-$0.2 & $-$0.5 & $-$10.3 & $+$8.2 & 0 & 0 \\
\hspace{0.6em}809272: Examples-first minimalist & 14 & $+$1.6 & $+$2.0 & $-$3.3 & $+$7.7 & 0 & 0 \\
\hspace{0.6em}835253: Plain-language technologist & 14 & $-$0.1 & $-$0.5 & $-$9.2 & $+$4.9 & 0 & 0 \\
\hspace{0.6em}992645: Examples-first learner & 14 & $+$0.5 & 0.0 & $-$3.8 & $+$6.8 & 0 & 0 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{All personas pooled} & 14 & $-$1.9 & $-$1.6 & $-$6.8 & $+$4.0 & 2 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Math} \textit{(tutor correctness; neutral mean 91.2 over 15 main-cohort models)}} \\
\hspace{0.6em}P1: Concise independent learner & 15 & $+$0.6 & $+$1.0 & $-$2.8 & $+$3.7 & 1 & 0 \\
\hspace{0.6em}P2: Detail-oriented checker & 15 & $+$1.7 & $+$1.0 & $-$0.5 & $+$7.5 & 0 & 1 \\
\hspace{0.6em}P3: Example-led explorer & 15 & $+$0.3 & 0.0 & $-$2.8 & $+$4.4 & 0 & 1 \\
\hspace{0.6em}P4: Intuitive demonstration seeker & 15 & $+$0.1 & $+$0.5 & $-$3.0 & $+$2.5 & 1 & 0 \\
\hspace{0.6em}P5: Anxious starter & 15 & $-$0.6 & $-$0.5 & $-$4.1 & $+$2.2 & 0 & 0 \\
\hspace{0.6em}P6: Frustrated learner & 15 & $+$0.7 & $+$1.0 & $-$2.5 & $+$3.5 & 0 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Finance} \textit{(rubric percent; neutral mean 43.6 over 18 main-cohort models)}} \\
\hspace{0.6em}CL: Careful learner & 18 & $+$0.4 & $+$0.5 & $-$3.0 & $+$2.6 & 0 & 3 \\
\hspace{0.6em}SQ: Skeptical questioner & 18 & $+$1.6 & $+$1.1 & $-$1.2 & $+$6.4 & 0 & 4 \\
\hspace{0.6em}CP: Concise pragmatist & 18 & $-$0.3 & $-$0.5 & $-$4.0 & $+$2.6 & 1 & 0 \\
\hspace{0.6em}DP: Decisive pusher & 18 & $+$2.4 & $+$2.5 & $-$0.9 & $+$4.9 & 0 & 9 \\
\hspace{0.6em}CC: Confident contrarian & 18 & $+$2.6 & $+$2.1 & $-$1.1 & $+$6.8 & 0 & 8 \\
\hspace{0.6em}RS: Reassurance seeker & 18 & $+$0.4 & $+$0.4 & $-$2.9 & $+$3.1 & 1 & 2 \\
\hspace{0.6em}D1: Designed persona 1 (task-specific) & 18 & $+$0.7 & $+$0.5 & $-$1.7 & $+$3.1 & 0 & 2 \\
\hspace{0.6em}D2: Designed persona 2 (task-specific) & 18 & $+$4.3 & $+$4.8 & $+$0.4 & $+$8.7 & 0 & 13 \\
\hspace{0.6em}D3: Designed persona 3 (task-specific) & 18 & $+$3.6 & $+$3.0 & $+$1.0 & $+$7.5 & 0 & 12 \\
\hspace{0.6em}D4: Designed persona 4 (task-specific) & 18 & $+$3.4 & $+$3.3 & $+$0.5 & $+$6.3 & 0 & 12 \\
\hspace{0.6em}D5: Designed persona 5 (task-specific) & 18 & $+$3.2 & $+$3.3 & $-$1.2 & $+$6.1 & 0 & 11 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{Six shared presets pooled} & 18 & $+$1.2 & $+$1.1 & $-$1.7 & $+$3.5 & 0 & 5 \\
\hspace{0.6em}\textit{Five designed personas pooled} & 18 & $+$3.0 & $+$2.9 & $+$0.3 & $+$5.8 & 0 & 13 \\
\hspace{0.6em}\textit{All personas pooled} & 18 & $+$2.0 & $+$2.1 & $-$0.8 & $+$4.5 & 0 & 11 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Customer Service} \textit{(task completion; neutral mean 72.5 over 14 main-cohort models)}} \\
\hspace{0.6em}P2: Frustrated on refusal & 14 & $-$0.5 & $-$0.6 & $-$8.8 & $+$6.4 & 1 & 0 \\
\hspace{0.6em}C2: Self-doubt & 14 & $+$0.7 & $+$0.3 & $-$4.0 & $+$5.8 & 0 & 0 \\
\hspace{0.6em}C3: Gives up early & 14 & $-$7.2 & $-$6.8 & $-$14.1 & $-$0.3 & 7 & 0 \\
\hspace{0.6em}A03: Money matters & 14 & $-$0.7 & $-$1.6 & $-$12.6 & $+$7.1 & 2 & 1 \\
\hspace{0.6em}A09: Wants the reason & 14 & $-$7.5 & $-$9.3 & $-$13.4 & $+$0.9 & 7 & 0 \\
\hspace{0.6em}A10: Bundles questions & 14 & $-$4.6 & $-$4.7 & $-$13.9 & $+$5.1 & 4 & 0 \\
\hspace{0.6em}A11: Risk-sensitive & 14 & $-$3.8 & $-$2.5 & $-$12.4 & $+$0.8 & 2 & 0 \\
\hspace{0.6em}A12: Wants options & 14 & $-$1.8 & $-$1.8 & $-$9.6 & $+$5.1 & 1 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Travel} \textit{(choice reward; neutral mean 73.4 over 19 main-cohort models)}} \\
\hspace{0.6em}CP: Careful planner & 19 & $-$10.4 & $-$10.9 & $-$25.2 & $+$6.2 & 13 & 0 \\
\hspace{0.6em}SC: Skeptical comparer & 19 & $-$24.1 & $-$21.6 & $-$40.8 & $-$10.0 & 19 & 0 \\
\hspace{0.6em}CD: Concise decider & 19 & $-$16.7 & $-$16.7 & $-$29.6 & $-$8.8 & 16 & 0 \\
\hspace{0.6em}EC: Efficient comparer & 19 & $-$13.3 & $-$12.7 & $-$26.1 & $-$1.6 & 13 & 0 \\
\hspace{0.6em}CN: Concise planner & 19 & $-$1.4 & $-$0.4 & $-$13.9 & $+$11.5 & 3 & 2 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{All personas pooled} & 19 & $-$13.1 & $-$13.8 & $-$24.2 & $-$2.2 & 16 & 0 \\
\bottomrule
\end{tabular}
\caption{\textbf{Change in the native task score under each persona, relative to the neutral user.} For each main-cohort model, the paired change is the mean over tasks of the persona episode's task score minus the neutral episode's score on the same task (same initial question and same first assistant reply; in Math the opening and first reply are generated per persona, so the Math contrast also includes the opening), in percentage points (Finance: rubric points; Travel: reward$\times$100); tasks enter only when both episodes have a task score. \emph{Mean}, \emph{Median}, \emph{Min} and \emph{Max} summarize the per-model changes over the main-cohort models with a paired estimate (\emph{Models}); \emph{Below} / \emph{Above} count models whose 95\% task-cluster bootstrap interval (5{,}000 resamples) lies entirely below / above zero. Pooled rows treat the persona conditions together (Finance: also the six shared presets and the five designed personas as groups), paired by task with the neutral user. Finance designed personas D1--D5 are written separately for each task; Math and Customer Service have no pooled estimate in the data. In Customer Service the contrast uses graded completed episodes (the task headline uses all planned episodes, incomplete ones scored 0), and the neutral score averages the task's graded neutral trials (up to three), of which only the first shares the persona conditions' first reply.}
\label{tab:persona-effects}
\end{table*}


==> old_archive/tables/scorecard.tex <==
% Generated by scripts/make_tables.py from data/cells.csv (headline columns task_value, needs_value).
\begin{table*}[t]
\tablestyle{4pt}{1.06}
\begin{tabular}{@{}l@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{5pt}}}
\toprule
 & \multicolumn{2}{c}{\textbf{Health}} & \multicolumn{2}{c}{\textbf{Coding}} & \multicolumn{2}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Finance}} & \multicolumn{2}{c}{\textbf{Cust.\ Service}} & \multicolumn{2}{c}{\textbf{Travel}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
\textbf{Model} & Task & Needs & Task & Needs & Task & Needs & Task & Needs & Task & Needs & Task & Needs \\
\midrule
\multicolumn{13}{@{}l}{\textit{Main cohort in all six domains}} \\
Qwen 3.8 27B & 40.0 & 78.8 & 87.1 & \textbf{95.2} & 91.1 & 81.8 & 45.4 & 56.7 & 71.3 & 74.0 & 63.9 & 91.1 \\
Muse Glimmer 30B & 46.3 & 82.6 & 69.6 & 86.8 & 81.6 & 58.0 & 35.4 & 62.7 & 35.5 & 47.5 & 54.7 & 93.7 \\
GPT-6 Luna & 27.0 & \textbf{96.5} & 84.0 & 94.1 & 91.5 & 85.8 & 35.7 & \textbf{90.1} & 75.2 & 69.2 & 47.7 & 87.1 \\
Gemini 3.7 Flash & 32.9 & 83.9 & 87.7 & 92.2 & 89.0 & 84.4 & 43.5 & 61.4 & 92.6 & 75.9 & \textbf{86.6} & 85.2 \\
Gemini 3.8 Flash & 32.1 & 83.1 & 88.1 & 92.0 & 89.5 & 86.2 & 45.1 & 63.1 & \textbf{94.1} & 78.4 & 76.3 & 88.1 \\
Kimi K3 & 40.6 & 91.5 & 90.1 & 94.7 & 92.4 & 84.1 & 47.2 & 68.5 & 74.5 & 79.3 & 71.1 & 88.2 \\
MiniMax M3 & \textbf{46.8}\rlap{$^{\circ}$} & 80.1\rlap{$^{\circ}$} & 67.6 & 85.7\rlap{$^{\ast}$} & 80.8 & 64.5 & 43.1 & 55.4 & 22.7 & 65.2 & 38.4 & 88.8 \\
DeepSeek V4.1 Flash & 39.9 & 93.9 & 88.8 & 93.8 & 94.5 & 81.5 & 44.0 & 77.8 & 72.0 & 69.4 & 73.6 & 85.5 \\
GLM 5.3 Flash & 40.4 & 88.0 & 92.0\rlap{$^{\circ}$} & 91.7\rlap{$^{\circ}$} & 94.0 & 83.8 & 46.9 & 66.3 & 56.3 & 74.9 & 64.2 & 86.3 \\
Qwen 3.8 Flash & 39.7 & 77.4 & 91.2\rlap{$^{\circ}$} & 94.0\rlap{$^{\circ}$} & \textbf{97.7}\rlap{$^{\circ}$} & 85.7\rlap{$^{\circ}$} & 48.7 & 57.2 & 60.5 & 73.3 & 66.6 & 87.6 \\
Claude Haiku 5.5 & 39.8\rlap{$^{\circ}$} & 91.7\rlap{$^{\circ}$} & 79.0 & 86.1 & 90.7 & 85.3 & 37.6 & 74.1 & 69.6 & 70.2 & 40.3 & 93.0 \\
Claude Sonnet 5.5 & 41.5 & 90.1 & 94.7 & 88.2 & 95.3 & 86.6 & 52.3 & 72.7 & 86.8 & 71.0 & 79.3 & 84.2 \\
\midrule
\multicolumn{13}{@{}l}{\textit{Main cohort in some domains}} \\
Grok 4.6 & {\color{black!45}45.1\rlap{$^{\dagger}$}} & {\color{black!45}97.0\rlap{$^{\dagger}$}} & 86.8 & 92.5 & 91.9 & 79.9 & {\color{black!45}51.5\rlap{$^{\dagger}$}} & {\color{black!45}80.4\rlap{$^{\dagger}$}} & 83.6 & 65.6 & 75.6 & 85.2 \\
Fable 5.1 & -- & -- & \textbf{95.5} & 90.9 & 96.4 & 89.8 & \textbf{57.1} & 70.1 & 87.7 & \textbf{80.2} & 79.7 & 87.8 \\
Claude Opus 5.5 & {\color{black!45}45.7\rlap{$^{\dagger}$}} & {\color{black!45}91.6\rlap{$^{\dagger}$}} & {\color{black!45}94.7\rlap{$^{\dagger}$}} & {\color{black!45}95.4\rlap{$^{\dagger}$}} & 97.4 & \textbf{90.5} & {\color{black!45}64.6\rlap{$^{\dagger}$}} & {\color{black!45}77.9\rlap{$^{\dagger}$}} & {\color{black!45}85.8\rlap{$^{\dagger}$}} & {\color{black!45}72.4\rlap{$^{\dagger}$}} & {\color{black!45}63.7\rlap{$^{\dagger}$}} & {\color{black!45}93.1\rlap{$^{\dagger}$}} \\
GPT-5.5 & {\color{black!45}40.7\rlap{$^{\ddagger}$}} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}88.6\rlap{$^{\S}$}} & {\color{black!45}94.8\rlap{$^{\S}$}} & {\color{black!45}92.4\rlap{$^{\ddagger}$}} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & 48.8 & 78.7 & {\color{black!45}89.9\rlap{$^{\ddagger}$}} & {\color{black!45}78.1\rlap{$^{\ddagger}$}} & 64.2 & 91.0 \\
GPT-5.6 Sol & {\color{black!45}35.9\rlap{$^{\ddagger}$}} & {\color{black!45}97.2\rlap{$^{\ddagger}$}} & {\color{black!45}92.2\rlap{$^{\S}$}} & {\color{black!45}94.9\rlap{$^{\S}$}} & {\color{black!45}95.2\rlap{$^{\ddagger}$}} & {\color{black!45}85.3\rlap{$^{\ddagger}$}} & 50.6 & 85.3 & {\color{black!45}88.9\rlap{$^{\ddagger}$}} & {\color{black!45}78.5\rlap{$^{\ddagger}$}} & 52.6 & 87.6 \\
GPT-5.6 Terra & {\color{black!45}34.3\rlap{$^{\ddagger}$}} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}87.3\rlap{$^{\S}$}} & {\color{black!45}91.3\rlap{$^{\S}$}} & {\color{black!45}88.8\rlap{$^{\ddagger}$}} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & 47.3 & 82.6 & {\color{black!45}89.3\rlap{$^{\ddagger}$}} & {\color{black!45}72.9\rlap{$^{\ddagger}$}} & 66.8 & 88.3 \\
GPT-6 Astra & {\color{black!45}34.4\rlap{$^{\ddagger}$}} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}100.0\rlap{$^{\S}$}} & {\color{black!45}97.3\rlap{$^{\S\ast}$}} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}91.3\rlap{$^{\ddagger}$}} & 50.6 & 90.0 & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}76.3\rlap{$^{\ddagger}$}} & 44.0 & \textbf{94.0} \\
GPT-6 Sol & {\color{black!45}26.7\rlap{$^{\ddagger}$}} & {\color{black!45}98.0\rlap{$^{\ddagger}$}} & {\color{black!45}93.6\rlap{$^{\S}$}} & {\color{black!45}93.9\rlap{$^{\S}$}} & {\color{black!45}95.0\rlap{$^{\ddagger}$}} & {\color{black!45}89.2\rlap{$^{\ddagger}$}} & 36.0 & 88.8 & {\color{black!45}82.2\rlap{$^{\ddagger}$}} & {\color{black!45}74.3\rlap{$^{\ddagger}$}} & 41.2 & 90.1 \\
\midrule
\textit{Main-cohort mean} & 38.9 & 86.5 & 85.9 & 91.3 & 91.6 & 81.9 & 45.3 & 72.3 & 70.2 & 71.0 & 62.5 & 88.6 \\
\textit{Main-cohort models} & \multicolumn{2}{c}{12} & \multicolumn{2}{c}{14} & \multicolumn{2}{c}{15} & \multicolumn{2}{c}{18} & \multicolumn{2}{c}{14} & \multicolumn{2}{c}{19} \\
\bottomrule
\end{tabular}
\caption{\textbf{Scorecard.} Native task score (\emph{Task}) and persona-needs score (\emph{Needs}) for every tested model in every domain, as percentages (Finance task: PRBench rubric percent). Task metrics are the source benchmarks' own: Health inquiry coverage, Coding hidden-test pass rate, Math tutor-solution correctness, Finance expert-rubric percent, Customer Service rule-based task completion and Travel UserBench choice reward (\tabref{tab:domains}). Each task score uses its domain's native population; each needs score averages persona episodes in which the user expressed at least one need and the assistant had a chance to answer it (in Coding and Customer Service, only completed simulator-valid episodes). Task and needs scores are not comparable across domains. Bold marks the best main-cohort value in each column; the last rows give the main-cohort mean and the number of main-cohort models per domain. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. $^{\ast}$ needs score over fewer than 50 scoreable episodes. -- no run. Denominators are given in \tabref{tab:scorecard-full}, coverage in \tabref{tab:coverage}.}
\label{tab:scorecard}
\end{table*}


==> old_archive/tables/scorecard_full.tex <==
% Generated by scripts/make_tables.py from data/cells.csv (task_value/task_den, needs_value/needs_den).
\begin{table*}[p]
\tablestyle{3.2pt}{1.04}\scriptsize
\begin{tabular}{@{}l *{6}{r@{\hspace{10pt}}r}@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Health}} & \multicolumn{2}{c}{\textbf{Coding}} & \multicolumn{2}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Finance}} & \multicolumn{2}{c}{\textbf{Cust.\ Service}} & \multicolumn{2}{c}{\textbf{Travel}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
\textbf{Model} & Value & $n$ & Value & $n$ & Value & $n$ & Value & $n$ & Value & $n$ & Value & $n$ \\
\midrule
\multicolumn{13}{@{}l}{\textbf{A. Native task score}} \\
Qwen 3.8 27B & 40.0 & 1,120 & 87.1 & 565 & 91.1 & 1,143 & 45.4 & 1,060 & 71.3 & 1,452 & 63.9 & 402 \\
Muse Glimmer 30B & 46.3 & 1,198 & 69.6 & 618 & 81.6 & 1,226 & 35.4 & 1,118 & 35.5 & 1,452 & 54.7 & 364 \\
GPT-6 Luna & 27.0 & 1,198 & 84.0 & 630 & 91.5 & 1,229 & 35.7 & 1,102 & 75.2 & 1,452 & 47.7 & 401 \\
Gemini 3.7 Flash & 32.9 & 1,200 & 87.7 & 593 & 89.0 & 1,223 & 43.5 & 1,065 & 92.6 & 1,452 & \textbf{86.6} & 402 \\
Gemini 3.8 Flash & 32.1 & 1,200 & 88.1 & 595 & 89.5 & 1,225 & 45.1 & 1,090 & \textbf{94.1} & 1,452 & 76.3 & 402 \\
Kimi K3 & 40.6 & 1,196 & 90.1 & 608 & 92.4 & 1,208 & 47.2 & 1,107 & 74.5 & 1,452 & 71.1 & 400 \\
MiniMax M3 & \textbf{46.8}\rlap{$^{\circ}$} & 1,140 & 67.6 & 479 & 80.8 & 1,201 & 43.1 & 965 & 22.7 & 1,452 & 38.4 & 336 \\
DeepSeek V4.1 Flash & 39.9 & 1,176 & 88.8 & 618 & 94.5 & 1,206 & 44.0 & 1,108 & 72.0 & 1,452 & 73.6 & 401 \\
GLM 5.3 Flash & 40.4 & 1,188 & 92.0\rlap{$^{\circ}$} & 426 & 94.0 & 984 & 46.9 & 1,081 & 56.3 & 1,452 & 64.2 & 402 \\
Qwen 3.8 Flash & 39.7 & 1,128 & 91.2\rlap{$^{\circ}$} & 362 & \textbf{97.7}\rlap{$^{\circ}$} & 825 & 48.7 & 890 & 60.5 & 1,452 & 66.6 & 402 \\
Claude Haiku 5.5 & 39.8\rlap{$^{\circ}$} & 1,080 & 79.0 & 692 & 90.7 & 1,230 & 37.6 & 1,164 & 69.6 & 1,452 & 40.3 & 400 \\
Claude Sonnet 5.5 & 41.5 & 1,194 & 94.7 & 693 & 95.3 & 1,230 & 52.3 & 1,164 & 86.8 & 1,452 & 79.3 & 402 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}45.1\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & 86.8 & 644 & 91.9 & 1,203 & {\color{black!45}51.5\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & 83.6 & 1,452 & 75.6 & 399 \\
Fable 5.1 & -- &  & \textbf{95.5} & 684 & 96.4 & 1,223 & \textbf{57.1} & 1,164 & 87.7 & 1,452 & 79.7 & 402 \\
Claude Opus 5.5 & {\color{black!45}45.7\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}94.7\rlap{$^{\dagger}$}} & {\color{black!45}695} & 97.4 & 1,227 & {\color{black!45}64.6\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}85.8\rlap{$^{\dagger}$}} & {\color{black!45}1,452} & {\color{black!45}63.7\rlap{$^{\dagger}$}} & {\color{black!45}401} \\
GPT-5.5 & {\color{black!45}40.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,076} & {\color{black!45}88.6\rlap{$^{\S}$}} & {\color{black!45}643} & {\color{black!45}92.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 48.8 & 1,122 & {\color{black!45}89.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 64.2 & 401 \\
GPT-5.6 Sol & {\color{black!45}35.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,128} & {\color{black!45}92.2\rlap{$^{\S}$}} & {\color{black!45}656} & {\color{black!45}95.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 50.6 & 1,146 & {\color{black!45}88.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 52.6 & 396 \\
GPT-5.6 Terra & {\color{black!45}34.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,112} & {\color{black!45}87.3\rlap{$^{\S}$}} & {\color{black!45}651} & {\color{black!45}88.8\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 47.3 & 1,130 & {\color{black!45}89.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 66.8 & 402 \\
GPT-6 Astra & {\color{black!45}34.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,107} & {\color{black!45}100.0\rlap{$^{\S}$}} & {\color{black!45}68} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & 50.6 & 1,108 & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 44.0 & 398 \\
GPT-6 Sol & {\color{black!45}26.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,115} & {\color{black!45}93.6\rlap{$^{\S}$}} & {\color{black!45}645} & {\color{black!45}95.0\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 36.0 & 1,153 & {\color{black!45}82.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 41.2 & 401 \\
\midrule
\multicolumn{13}{@{}l}{\textbf{B. Persona-needs score}} \\
Qwen 3.8 27B & 78.8 & 614 & \textbf{95.2} & 190 & 81.8 & 1,144 & 56.7 & 1,000 & 74.0 & 706 & 91.1 & 270 \\
Muse Glimmer 30B & 82.6 & 693 & 86.8 & 106 & 58.0 & 1,228 & 62.7 & 1,007 & 47.5 & 683 & 93.7 & 277 \\
GPT-6 Luna & \textbf{96.5} & 353 & 94.1 & 124 & 85.8 & 1,229 & \textbf{90.1} & 867 & 69.2 & 665 & 87.1 & 261 \\
Gemini 3.7 Flash & 83.9 & 596 & 92.2 & 54 & 84.4 & 1,224 & 61.4 & 1,033 & 75.9 & 677 & 85.2 & 251 \\
Gemini 3.8 Flash & 83.1 & 590 & 92.0 & 64 & 86.2 & 1,226 & 63.1 & 1,009 & 78.4 & 695 & 88.1 & 254 \\
Kimi K3 & 91.5 & 627 & 94.7 & 85 & 84.1 & 1,208 & 68.5 & 994 & 79.3 & 682 & 88.2 & 243 \\
MiniMax M3 & 80.1\rlap{$^{\circ}$} & 705 & 85.7\rlap{$^{\ast}$} & 19 & 64.5 & 1,206 & 55.4 & 1,038 & 65.2 & 697 & 88.8 & 186 \\
DeepSeek V4.1 Flash & 93.9 & 593 & 93.8 & 67 & 81.5 & 1,206 & 77.8 & 981 & 69.4 & 698 & 85.5 & 267 \\
GLM 5.3 Flash & 88.0 & 660 & 91.7\rlap{$^{\circ}$} & 120 & 83.8 & 984 & 66.3 & 978 & 74.9 & 719 & 86.3 & 274 \\
Qwen 3.8 Flash & 77.4 & 585 & 94.0\rlap{$^{\circ}$} & 116 & 85.7\rlap{$^{\circ}$} & 825 & 57.2 & 822 & 73.3 & 717 & 87.6 & 268 \\
Claude Haiku 5.5 & 91.7\rlap{$^{\circ}$} & 450 & 86.1 & 590 & 85.3 & 1,229 & 74.1 & 996 & 70.2 & 710 & 93.0 & 292 \\
Claude Sonnet 5.5 & 90.1 & 620 & 88.2 & 586 & 86.6 & 1,230 & 72.7 & 990 & 71.0 & 693 & 84.2 & 294 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}97.0\rlap{$^{\dagger}$}} & {\color{black!45}899} & 92.5 & 123 & 79.9 & 1,204 & {\color{black!45}80.4\rlap{$^{\dagger}$}} & {\color{black!45}1,028} & 65.6 & 705 & 85.2 & 275 \\
Fable 5.1 & -- &  & 90.9 & 585 & 89.8 & 1,223 & 70.1 & 1,005 & \textbf{80.2} & 716 & 87.8 & 288 \\
Claude Opus 5.5 & {\color{black!45}91.6\rlap{$^{\dagger}$}} & {\color{black!45}787} & {\color{black!45}95.4\rlap{$^{\dagger}$}} & {\color{black!45}591} & \textbf{90.5} & 1,224 & {\color{black!45}77.9\rlap{$^{\dagger}$}} & {\color{black!45}1,035} & {\color{black!45}72.4\rlap{$^{\dagger}$}} & {\color{black!45}740} & {\color{black!45}93.1\rlap{$^{\dagger}$}} & {\color{black!45}360} \\
GPT-5.5 & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}636} & {\color{black!45}94.8\rlap{$^{\S}$}} & {\color{black!45}102} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 78.7 & 982 & {\color{black!45}78.1\rlap{$^{\ddagger}$}} & {\color{black!45}715} & 91.0 & 291 \\
GPT-5.6 Sol & {\color{black!45}97.2\rlap{$^{\ddagger}$}} & {\color{black!45}521} & {\color{black!45}94.9\rlap{$^{\S}$}} & {\color{black!45}129} & {\color{black!45}85.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & 85.3 & 909 & {\color{black!45}78.5\rlap{$^{\ddagger}$}} & {\color{black!45}702} & 87.6 & 270 \\
GPT-5.6 Terra & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}485} & {\color{black!45}91.3\rlap{$^{\S}$}} & {\color{black!45}89} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 82.6 & 928 & {\color{black!45}72.9\rlap{$^{\ddagger}$}} & {\color{black!45}696} & 88.3 & 282 \\
GPT-6 Astra & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}476} & {\color{black!45}97.3\rlap{$^{\S\ast}$}} & {\color{black!45}19} & {\color{black!45}91.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 90.0 & 846 & {\color{black!45}76.3\rlap{$^{\ddagger}$}} & {\color{black!45}744} & \textbf{94.0} & 264 \\
GPT-6 Sol & {\color{black!45}98.0\rlap{$^{\ddagger}$}} & {\color{black!45}395} & {\color{black!45}93.9\rlap{$^{\S}$}} & {\color{black!45}117} & {\color{black!45}89.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 88.8 & 860 & {\color{black!45}74.3\rlap{$^{\ddagger}$}} & {\color{black!45}719} & 90.1 & 282 \\
\bottomrule
\end{tabular}
\caption{\textbf{Scorecard with denominators.} Values as in \tabref{tab:scorecard} (percent; Finance task: rubric percent); $n$ is the number of episodes behind each value. Task populations follow each benchmark's native rule: Health, all planned episodes with a task score (graded partial dialogues included); Coding, completed simulator-valid episodes; Math, persona episodes with a tutor grade; Finance, recorded episodes with a valid advice grade; Customer Service, all planned episodes (incomplete ones count as not completed); Travel, recorded official-task episodes with a score. Needs $n$ counts persona episodes with at least one expressed and answered need; in Coding and Customer Service only completed episodes with a valid simulator audit count, so this $n$ can be smaller than \emph{Scor.} in \tabref{tab:coverage}. Rows below the gap are the models outside the main cohort in at least one domain. Bold marks the best main-cohort value per column. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. $^{\ast}$ fewer than 50 scoreable episodes. -- no run. Health values use the \texttt{llm\_judgment\_v1} judge-acceptance policy, except the five score-only GPT packages ($^{\ddagger}$), which provide only the stricter native acceptance policy. Gemini 3.7 / 3.8 Flash use the original validated judge outputs, as all other models do; their packages also publish a raw-judge score update, reported in the domain tables.}
\label{tab:scorecard-full}
\end{table*}


==> old_archive/tables/supp_coding.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Coding, 20 hard LiveCodeBench tasks.} Persona pass is conditional on publicly expressed critical needs (analysis version \emph{publicly-expressed-critical-needs-v1}); intervals are 95\% Wilson and treat episodes as independent. Critical needs counts are needs with a public request and an assistant reply over applicable critical needs. Source: examples/coding-hard20-paper-reference.}
\label{tab:supp-coding}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Card} & \textbf{Tests passed} & \textbf{Persona pass (\%)} & \textbf{Critical needs answered (\%)} & \textbf{Need credit} \\
\midrule
Detailed typed professional & 18/20 & 100.0 {\scriptsize [83.9, 100.0]} (20/20) & 87.0 (40/46) & 0.97 \\
Concise skeptical professional & 20/20 & 90.0 {\scriptsize [69.9, 97.2]} (18/20) & 92.0 (46/50) & 0.97 \\
Performance-focused student & 19/19 & 66.7 {\scriptsize [43.7, 83.7]} (12/18) & 71.4 (60/84) & 0.95 \\
Trade-off-focused professional & 19/19 & 89.5 {\scriptsize [68.6, 97.1]} (17/19) & 97.2 (35/36) & 0.97 \\
Maintainability-minded reviewer & 20/20 & 73.7 {\scriptsize [51.2, 88.2]} (14/19) & 83.1 (54/65) & 0.92 \\
Deadline-driven technologist & 20/20 & 73.7 {\scriptsize [51.2, 88.2]} (14/19) & 51.5 (51/99) & 0.96 \\
Simple-performance reviewer & 20/20 & 85.0 {\scriptsize [64.0, 94.8]} (17/20) & 69.7 (53/76) & 0.97 \\
Dependency-minimal explainer & 19/20 & 95.0 {\scriptsize [76.4, 99.1]} (19/20) & 73.2 (52/71) & 0.99 \\
Examples-first minimalist & 20/20 & 75.0 {\scriptsize [53.1, 88.8]} (15/20) & 95.0 (76/80) & 0.96 \\
Plain-language technologist & 19/19 & 89.5 {\scriptsize [68.6, 97.1]} (17/19) & 43.1 (25/58) & 0.90 \\
Test-oriented hobbyist & 20/20 & 72.2 {\scriptsize [49.1, 87.5]} (13/18) & 72.4 (55/76) & 0.96 \\
Examples-first learner & 19/19 & 68.4 {\scriptsize [46.0, 84.6]} (13/19) & 86.4 (89/103) & 0.95 \\
\midrule
\textbf{all 12 cards} & 233/236 & 81.8 {\scriptsize [76.3, 86.3]} (189/231) & 75.4 (636/844) & 0.96 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> old_archive/tables/supp_finance.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Finance, round 1 (all 361 tasks).} Values are gpt-5.6-sol / gpt-6-astra. Advice scores are PRBench rubric percentages over the whole conversation and over the last assistant message; persona pass and joint pass are percentages of conversations. Source: examples/persona-trials/README.md.}
\label{tab:supp-finance}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Condition} & \textbf{Advice, whole} & \textbf{Advice, last} & \textbf{Persona pass (\%)} & \textbf{Joint (\%)} \\
\midrule
neutral & 49.5 / 50.5 & 46.8 / 47.3 & -- & -- \\
skeptical questioner & 53.2 / 52.1 & 40.0 / 39.6 & 83 / 98 & 47 / 54 \\
designed (5 per task) & 54.2 / 53.5 & 39.6 / 38.4 & 74 / 94 & 44 / 55 \\
confident contrarian & 52.6 / 52.2 & 36.8 / 32.8 & 88 / 99 & 51 / 55 \\
concise pragmatist & 49.4 / 49.9 & 30.7 / 28.2 & 99 / 100 & 52 / 51 \\
decisive pusher & 49.4 / 50.9 & 25.2 / 25.0 & 95 / 100 & 49 / 49 \\
reassurance seeker & 49.3 / 50.4 & 23.8 / 22.4 & 97 / 100 & 50 / 52 \\
careful learner & 49.6 / 49.9 & 25.8 / 21.6 & 34 / 77 & 17 / 41 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> old_archive/tables/supp_health.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Health, 10 cases $\times$ (5 personas + neutral) $\times$ 2 anonymous doctor configurations.} Inquiry coverage is not diagnostic accuracy. Persona demonstration is the share of attribute items with an opportunity that were clearly shown. Need credit is conditional on a scoreable need (number of cases of 10 in parentheses). Source: healthbench-benchmark/examples/RESULTS.md.}
\label{tab:supp-health}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Persona / doctor} & \textbf{Inquiry} & \textbf{Facts} & \textbf{Demonstration} & \textbf{Need credit (scoreable)} \\
\midrule
P1 / Doctor A & 50.8 & 71.2 & 76.3 & 100.0 (7/10) \\
P1 / Doctor B & 46.7 & 77.5 & 76.7 & 90.6 (8/10) \\
P2 / Doctor A & 45.6 & 66.4 & 61.1 & 100.0 (1/10) \\
P2 / Doctor B & 47.9 & 78.2 & 65.8 & 100.0 (1/10) \\
P3 / Doctor A & 44.9 & 79.2 & 88.3 & 100.0 (7/10) \\
P3 / Doctor B & 49.5 & 78.6 & 85.2 & 100.0 (8/10) \\
P4 / Doctor A & 49.4 & 85.8 & 93.8 & 100.0 (10/10) \\
P4 / Doctor B & 60.0 & 86.8 & 91.5 & 100.0 (10/10) \\
P5 / Doctor A & 52.3 & 80.1 & 77.9 & 100.0 (4/10) \\
P5 / Doctor B & 47.0 & 77.9 & 65.1 & 100.0 (4/10) \\
NEUTRAL / Doctor A & 45.2 & 78.5 & -- & -- \\
NEUTRAL / Doctor B & 51.3 & 86.7 & -- & -- \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> old_archive/tables/supp_help.tex <==
\begin{table}[H]
\centering
\caption{\textbf{HelpBench, 450 tasks (v2 protocol).} Planned 2,250, completed 2,161, graded 2,086, valid 2,081. Task score is the trajectory rubric score; persona adherence is evaluated only after disclosure. Source: examples/gpt6-astra-attributes-v2-450-task/SUMMARY.md.}
\label{tab:supp-help}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Condition} & \textbf{Valid / planned} & \textbf{Task score (\%)} & \textbf{Adherence (\%)} \\
\midrule
neutral\_multi / neutral & 417/450 & 81.82 (n=417) & -- \\
persona\_multi / careful\_learner & 412/450 & 82.75 (n=412) & 99.86 (n=365) \\
persona\_multi / concise\_pragmatist & 419/450 & 81.35 (n=419) & 99.48 (n=240) \\
persona\_multi / skeptical\_questioner & 406/450 & 81.77 (n=406) & 99.92 (n=396) \\
single\_turn / neutral & 427/450 & 79.77 (n=427) & -- \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> old_archive/tables/supp_law.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Law, 59 cases $\times$ 5 archetypes (client gpt-5.6-sol).} Resolution $=\frac12$(Fact + Issue Resolution); adherence is the client persona judge's score and its components (percent). Means are taken within each jurisdiction and then across jurisdictions. Source: examples/gpt-5.6-sol-simulation-astra-judge-all-cases/SUMMARY.md.}
\label{tab:supp-law}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
\textbf{Archetype} & \textbf{Res.} & \textbf{Fact} & \textbf{Issue} & \textbf{Adher.} & \textbf{Arch.} & \textbf{Attr.} & \textbf{Goal} & \textbf{Facts} & \textbf{Rules} \\
\midrule
Assured cooperator & 39.9 & 52.6 & 27.2 & 80.9 & 100.0 & 79.0 & 100.0 & 39.8 & 89.0 \\
Dependent and anxious & 34.7 & 49.7 & 19.8 & 76.8 & 87.3 & 76.2 & 100.0 & 27.0 & 93.2 \\
Avoidant and withdrawn & 39.2 & 51.8 & 26.6 & 76.5 & 83.0 & 76.3 & 100.0 & 28.7 & 90.7 \\
Controlling resister & 41.0 & 53.1 & 28.9 & 77.3 & 83.1 & 77.0 & 100.0 & 36.2 & 87.3 \\
Trusting but impatient & 34.8 & 47.9 & 21.6 & 76.2 & 63.5 & 78.0 & 98.3 & 33.1 & 93.2 \\
\midrule
overall & 37.9 & 51.0 & 24.8 & 77.5 & 83.4 & 77.3 & 99.7 & 32.9 & 90.7 \\
PRC cases & 37.3 & 41.8 & 32.9 & 77.8 & 83.1 & 78.0 & 100.0 & 26.2 & 92.4 \\
U.S. cases & 38.5 & 60.2 & 16.8 & 77.3 & 83.7 & 76.6 & 99.3 & 39.7 & 89.0 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> old_archive/tables/supp_needtypes.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Coding need types.} The classification is an analysis choice made for this paper. A need \emph{asks for content} if the user can request additional material in the conversation, and \emph{constrains form} if it states a property of the delivered code that a user would normally expect by default. Counts are for critical needs: expressed and answered over applicable, and satisfied / partially satisfied among answered.}
\label{tab:need-types}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}p{2.6cm}rrr>{\raggedright\arraybackslash}p{7.2cm}@{}}
\toprule
\textbf{Class} & \textbf{Types} & \textbf{Answered / applicable} & \textbf{Sat. / partial} & \textbf{Need types} \\
\midrule
Asks for content & 10 & 574/617 & 526 / 48 & verification\_rationale, detailed\_explanation, concise\_explanation, public\_test\_cases, plain\_language, example\_walkthrough, decision\_tradeoffs, revision\_and\_checks, performance\_check, minimal\_test\_exposition \\
Constrains the artifact's form & 15 & 58/206 & 58 / 0 & type\_annotations, custom\_implementation, low\_complexity, readability, minimal\_dependencies, no\_comments, straightforward\_structure, object\_oriented\_structure, standard\_library\_tools, self\_documenting\_code, extensive\_comments, modular\_structure, compact\_names, docstrings, maintainability \\
Delivery and tone & 3 & 4/21 & 4 / 0 & deadline\_delivery, supportive\_tone, direct\_tone \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> old_archive/tables/supp_variance.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Variance of the native score attributed to task, persona and interaction.} Shares are percentages of the total sum of squares ($\eta^2$, \secref{sec:stats}); the persona share is within task, with a 95\% task-cluster bootstrap interval, and the last column is the 97.5th percentile of its within-task permutation null (1{,}000 permutations). Finance uses round 1 and conversations with a valid simulator audit; HelpBench uses the neutral and the three persona multi-turn arms.}
\label{tab:supp-variance}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}p{4.6cm}rrrrrr@{}}
\toprule
\textbf{Score} & \textbf{n} & \textbf{Tasks / conditions} & \textbf{Task} & \textbf{Persona} & \textbf{Interaction + noise} & \textbf{Null 97.5th} \\
\midrule
Finance, whole conversation, gpt-5.6-sol & 4,203 & 361 / 12 & 87.6 & 1.5 {\scriptsize [1.2, 2.0]} & 10.8 & 0.07 \\
Finance, whole conversation, gpt-6-astra & 4,225 & 361 / 12 & 91.4 & 0.6 {\scriptsize [0.5, 0.9]} & 7.9 & 0.05 \\
Finance, last message, gpt-5.6-sol & 4,215 & 361 / 12 & 50.2 & 12.4 {\scriptsize [10.7, 14.3]} & 37.4 & 0.28 \\
Finance, last message, gpt-6-astra & 4,227 & 361 / 12 & 51.4 & 13.4 {\scriptsize [11.5, 15.7]} & 35.2 & 0.26 \\
HelpBench, trajectory score, gpt-6-astra & 1,654 & 431 / 4 & 91.9 & 0.2 {\scriptsize [0.1, 0.3]} & 7.9 & 0.06 \\
Law, Resolution, client gpt-5.6-sol & 295 & 59 / 5 & 73.1 & 2.6 {\scriptsize [1.4, 5.6]} & 24.3 & 1.27 \\
Law, client adherence & 295 & 59 / 5 & 28.4 & 6.0 {\scriptsize [3.0, 12.1]} & 65.6 & 3.18 \\
Coding, tests passed (binary) & 236 & 20 / 12 & 12.8 & 7.2 {\scriptsize [4.2, 18.7]} & 80.0 & 7.46 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> protocol_style.tex <==
\RequirePackage{amsmath}
\RequirePackage{array}
\RequirePackage{tabularx}
\RequirePackage{booktabs}
\RequirePackage{xcolor}
\RequirePackage{colortbl}
\RequirePackage{caption}
\RequirePackage{enumitem}
\RequirePackage{needspace}
\RequirePackage{placeins}
\RequirePackage{tcolorbox}
\tcbuselibrary{breakable,skins}

\definecolor{PCBlue}{HTML}{315E9C}
\definecolor{PCTeal}{HTML}{237D72}
\definecolor{PCOrange}{HTML}{A65E20}
\definecolor{PCPurple}{HTML}{705397}
\definecolor{PCInk}{HTML}{263446}
\definecolor{PCGray}{HTML}{F1F3F5}

\newcolumntype{J}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{V}{>{\raggedright\arraybackslash}X}
\newcommand{\pcCode}[1]{\texttt{\detokenize{#1}}}
\newcommand{\pcRole}[2]{\textcolor{#1}{\textbf{#2}}}
\newcommand{\pcHead}[1]{\textbf{#1}}
\newenvironment{pctable}{%
  \par\addvspace{9pt}\noindent\begin{minipage}{\linewidth}
  \small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.23}
  \captionsetup{type=table,font={small,up},labelfont=up,textfont=up,position=bottom,skip=5pt}
}{\end{minipage}\par\addvspace{7pt}}
\newenvironment{pcprompt}[3]{%
  \par\Needspace{6\baselineskip}
  \begin{tcolorbox}[
    enhanced,breakable,sharp corners,boxrule=0pt,
    frame hidden,borderline west={2.2pt}{0pt}{#1},
    colback=#1!4!white,colbacktitle=#1!11!white,coltitle=PCInk,
    title={\textbf{#2}\hfill\normalfont\footnotesize #3},
    title after break={\textbf{#2 (continued)}},
    fonttitle=\small,fontupper=\small,
    left=9pt,right=9pt,top=6pt,bottom=6pt,
    toptitle=5pt,bottomtitle=5pt,
    before skip=9pt,after skip=9pt,
    before upper={\setlength{\parindent}{0pt}\setlength{\parskip}{5pt}}
  ]
}{\end{tcolorbox}}


==> tables/coverage.tex <==
% Generated by scripts/make_tables.py from data/cells.csv (coverage columns).
\begin{table*}[p]
\tablestyle{2.6pt}{1.04}\scriptsize
\begin{tabular}{@{}l@{\hspace{7pt}}rrrrr@{\hspace{7pt}}rrrrr@{\hspace{7pt}}rrrrr@{}}
\toprule
 & \multicolumn{5}{c}{\textbf{Health} (1,200 planned)} & \multicolumn{5}{c}{\textbf{Coding} (700 planned)} & \multicolumn{5}{c}{\textbf{Math} (1,435 planned)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
\textbf{Model} & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. \\
\midrule
Qwen 3.8 27B & 1,031 & 1,120 & 930 & 614 & 1,122 & 581 & 581 & 199 & 196 & 582 & 1,334 & 1,333 & 1,144 & 1,144 & 1,331 \\
Muse Glimmer 30B & 1,164 & 1,198 & 1,000 & 693 & 1,200 & 681 & 681 & 129 & 120 & 682 & 1,431 & 1,429 & 1,228 & 1,228 & 1,428 \\
GPT-6 Luna & 1,188 & 1,198 & 1,000 & 353 & 1,200 & 699 & 699 & 143 & 143 & 640 & 1,434 & 1,434 & 1,229 & 1,229 & 1,433 \\
Gemini 3.7 Flash & 1,200 & 1,200 & 1,000 & 596 & 1,200 & 700 & 700 & 60 & 60 & 614 & 1,435 & 1,427 & 1,224 & 1,224 & 1,428 \\
Gemini 3.8 Flash & 1,200 & 1,200 & 1,000 & 590 & 1,200 & 700 & 700 & 75 & 75 & 609 & 1,435 & 1,429 & 1,226 & 1,226 & 1,426 \\
Kimi K3 & 1,184 & 1,196 & 1,000 & 627 & 1,200 & 685 & 685 & 106 & 95 & 641 & 1,406 & 1,406 & 1,208 & 1,208 & 1,403 \\
MiniMax M3 & 932\rlap{$^{\circ}$} & 1,140 & 950 & 705 & 1,140 & 676 & 676 & 42 & 39 & 527 & 1,409 & 1,403 & 1,207 & 1,206 & 1,400 \\
DeepSeek V4.1 Flash & 1,141 & 1,176 & 980 & 593 & 1,176 & 697 & 697 & 75 & 73 & 634 & 1,411 & 1,409 & 1,206 & 1,206 & 1,409 \\
GLM 5.3 Flash & 1,120 & 1,188 & 990 & 660 & 1,188 & 443\rlap{$^{\circ}$} & 443 & 131 & 124 & 446 & 1,150 & 1,150 & 984 & 984 & 1,149 \\
Qwen 3.8 Flash & 1,009 & 1,128 & 940 & 585 & 1,128 & 364\rlap{$^{\circ}$} & 364 & 120 & 117 & 370 & 985\rlap{$^{\circ}$} & 985 & 825 & 825 & 985 \\
Claude Haiku 5.5 & 657\rlap{$^{\circ}$} & 1,080 & 900 & 450 & 1,080 & 700 & 700 & 600 & 598 & 700 & 1,435 & 1,435 & 1,230 & 1,229 & 1,435 \\
Claude Sonnet 5.5 & 1,130 & 1,194 & 995 & 620 & 1,194 & 699 & 699 & 599 & 591 & 699 & 1,434 & 1,434 & 1,230 & 1,230 & 1,434 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}1,173\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}999} & {\color{black!45}899} & {\color{black!45}1,200} & 700 & 700 & 136 & 134 & 656 & 1,402 & 1,399 & 1,204 & 1,204 & 1,400 \\
Fable 5.1 & -- &  &  &  &  & 693 & 693 & 594 & 592 & 693 & 1,428 & 1,428 & 1,223 & 1,223 & 1,428 \\
Claude Opus 5.5 & {\color{black!45}1,194\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}1,000} & {\color{black!45}787} & {\color{black!45}1,200} & {\color{black!45}700\rlap{$^{\dagger}$}} & {\color{black!45}700} & {\color{black!45}600} & {\color{black!45}591} & {\color{black!45}700} & 1,432 & 1,432 & 1,225 & 1,224 & 1,430 \\
GPT-5.5 & {\color{black!45}1,199\rlap{$^{\ddagger}$}} & {\color{black!45}1,076} & {\color{black!45}998} & {\color{black!45}636} & {\color{black!45}1,092} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}112} & {\color{black!45}112} & {\color{black!45}653} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}1,435} & {\color{black!45}1,230} & {\color{black!45}1,230} & {\color{black!45}1,432} \\
GPT-5.6 Sol & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}1,128} & {\color{black!45}997} & {\color{black!45}521} & {\color{black!45}1,089} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}143} & {\color{black!45}143} & {\color{black!45}662} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}1,431} & {\color{black!45}1,229} & {\color{black!45}1,229} & {\color{black!45}1,431} \\
GPT-5.6 Terra & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}1,112} & {\color{black!45}1,000} & {\color{black!45}485} & {\color{black!45}1,075} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}103} & {\color{black!45}103} & {\color{black!45}662} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}1,433} & {\color{black!45}1,228} & {\color{black!45}1,228} & {\color{black!45}1,430} \\
GPT-6 Astra & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}1,107} & {\color{black!45}1,000} & {\color{black!45}476} & {\color{black!45}1,097} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}24} & {\color{black!45}24} & {\color{black!45}69} & {\color{black!45}1,434\rlap{$^{\ddagger}$}} & {\color{black!45}1,434} & {\color{black!45}1,229} & {\color{black!45}1,228} & {\color{black!45}1,430} \\
GPT-6 Sol & {\color{black!45}1,187\rlap{$^{\ddagger}$}} & {\color{black!45}1,115} & {\color{black!45}989} & {\color{black!45}395} & {\color{black!45}1,087} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}700} & {\color{black!45}129} & {\color{black!45}129} & {\color{black!45}660} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}1,435} & {\color{black!45}1,230} & {\color{black!45}1,230} & {\color{black!45}1,434} \\
\midrule
\textit{All runs} & 21,309 & 21,954 & 18,668 & 11,285 & 21,868 & 13,218 & 13,218 & 4,120 & 4,059 & 11,899 & 27,731 & 27,701 & 23,739 & 23,735 & 27,676 \\
\textit{Main cohort} & 12,956 & 14,018 & 11,685 & 7,086 & 14,028 & 9,018 & 9,018 & 3,009 & 2,957 & 8,493 & 20,561 & 20,533 & 17,593 & 17,590 & 20,519 \\
\midrule[\heavyrulewidth]
 & \multicolumn{5}{c}{\textbf{Finance} (1,164 planned)} & \multicolumn{5}{c}{\textbf{Customer Service} (1,452 planned)} & \multicolumn{5}{c}{\textbf{Travel} (432 planned)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
\textbf{Model} & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. & Gen. & Task & Needs & Scor. & Aud. \\
\midrule
Qwen 3.8 27B & 1,123 & 1,060 & 1,045 & 1,000 & 1,140 & 1,452 & 1,452 & 1,056 & 751 & 1,452 & 432 & 432 & 349 & 270 & 432 \\
Muse Glimmer 30B & 994 & 1,118 & 1,067 & 1,007 & 1,164 & 1,452 & 1,452 & 1,056 & 754 & 1,452 & 394 & 394 & 336 & 277 & 405 \\
GPT-6 Luna & 1,163 & 1,102 & 1,052 & 867 & 1,162 & 1,452 & 1,452 & 1,025 & 722 & 1,435 & 431 & 431 & 340 & 261 & 430 \\
Gemini 3.7 Flash & 1,164 & 1,065 & 1,064 & 1,033 & 1,159 & 1,452 & 1,452 & 1,056 & 728 & 1,452 & 432 & 432 & 322 & 251 & 432 \\
Gemini 3.8 Flash & 1,164 & 1,090 & 1,060 & 1,009 & 1,158 & 1,452 & 1,452 & 1,056 & 744 & 1,452 & 432 & 432 & 327 & 254 & 432 \\
Kimi K3 & 1,159 & 1,107 & 1,062 & 994 & 1,159 & 1,445 & 1,445 & 1,025 & 719 & 1,445 & 430 & 430 & 308 & 243 & 430 \\
MiniMax M3 & 1,159 & 965 & 1,066 & 1,038 & 1,163 & 1,452 & 1,452 & 1,056 & 768 & 1,452 & 366 & 366 & 266 & 186 & 373 \\
DeepSeek V4.1 Flash & 1,164 & 1,108 & 1,067 & 981 & 1,164 & 1,448 & 1,448 & 1,053 & 748 & 1,452 & 431 & 431 & 333 & 267 & 431 \\
GLM 5.3 Flash & 1,122 & 1,081 & 1,034 & 978 & 1,128 & 1,452 & 1,452 & 1,056 & 756 & 1,452 & 432 & 432 & 341 & 274 & 432 \\
Qwen 3.8 Flash & 937 & 890 & 869 & 822 & 948 & 1,452 & 1,452 & 1,056 & 761 & 1,452 & 432 & 432 & 343 & 268 & 432 \\
Claude Haiku 5.5 & 1,164 & 1,164 & 1,067 & 996 & 1,164 & 1,452 & 1,452 & 1,056 & 774 & 1,452 & 430 & 430 & 360 & 292 & 432 \\
Claude Sonnet 5.5 & 1,164 & 1,164 & 1,067 & 990 & 1,164 & 1,452 & 1,452 & 1,056 & 753 & 1,452 & 432 & 432 & 360 & 294 & 432 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}1,163\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}1,066} & {\color{black!45}1,028} & {\color{black!45}1,163} & 1,446 & 1,446 & 1,052 & 758 & 1,452 & 429 & 429 & 342 & 275 & 430 \\
Fable 5.1 & 1,164 & 1,164 & 1,067 & 1,005 & 1,164 & 1,452 & 1,452 & 1,056 & 754 & 1,452 & 432 & 432 & 360 & 288 & 432 \\
Claude Opus 5.5 & {\color{black!45}1,164\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}1,067} & {\color{black!45}1,035} & {\color{black!45}1,164} & {\color{black!45}1,452\rlap{$^{\dagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}764} & {\color{black!45}1,452} & {\color{black!45}431\rlap{$^{\dagger}$}} & {\color{black!45}431} & {\color{black!45}360} & {\color{black!45}360} & {\color{black!45}432} \\
GPT-5.5 & 1,164 & 1,122 & 1,067 & 982 & 1,164 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}743} & {\color{black!45}1,452} & 431 & 431 & 359 & 291 & 432 \\
GPT-5.6 Sol & 1,164 & 1,146 & 1,067 & 909 & 1,164 & {\color{black!45}1,448\rlap{$^{\ddagger}$}} & {\color{black!45}1,448} & {\color{black!45}1,053} & {\color{black!45}739} & {\color{black!45}1,452} & 426 & 426 & 357 & 270 & 432 \\
GPT-5.6 Terra & 1,164 & 1,130 & 1,067 & 928 & 1,164 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}752} & {\color{black!45}1,452} & 432 & 432 & 359 & 282 & 432 \\
GPT-6 Astra & 1,154 & 1,108 & 1,051 & 846 & 1,134 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}776} & {\color{black!45}1,452} & 428 & 428 & 357 & 264 & 432 \\
GPT-6 Sol & 1,164 & 1,153 & 1,067 & 860 & 1,164 & {\color{black!45}1,452\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & {\color{black!45}1,056} & {\color{black!45}746} & {\color{black!45}1,452} & 431 & 431 & 357 & 282 & 432 \\
\midrule
\textit{All runs} & 22,778 & 22,063 & 21,039 & 19,308 & 22,954 & 29,019 & 29,019 & 21,048 & 15,010 & 29,016 & 8,514 & 8,514 & 6,836 & 5,449 & 8,547 \\
\textit{Main cohort} & 20,451 & 19,737 & 18,906 & 17,245 & 20,627 & 20,311 & 20,311 & 14,715 & 10,490 & 20,304 & 8,083 & 8,083 & 6,476 & 5,089 & 8,115 \\
\bottomrule
\end{tabular}
\caption{\textbf{Episode coverage per model and domain.} \emph{Gen.}: episodes whose conversation was generated; a conversation stopped at the turn cap counts as generated, except in Travel, where a capped episode has no primary task score, and in Health, whose single capped conversation is recorded as a failure; \emph{Task}: episodes with a native task grade; \emph{Needs}: persona episodes with a needs judgment (the neutral user has no needs); \emph{Scor.}: persona episodes with at least one need that the user expressed and the assistant had a chance to answer; \emph{Aud.}: episodes with a simulator audit. In Health the task is also graded on the recorded part of dialogues whose generation failed, so Task can exceed Gen. Over all 119 runs, 126,460 episodes were planned, 122,569 generated, 122,469 task-graded, 95,450 needs-judged, 78,846 needs-scoreable and 121,960 audited. Failed and unscored episodes stay in the planned denominators. Gray values mark cells outside the main cohort, with the markers of \tabref{tab:scorecard}; $^{\circ}$ fewer than 80\% of planned episodes generated; -- no run.}
\label{tab:coverage}
\end{table*}


==> tables/domain_coding.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/coding_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Pass rate}} & \multicolumn{2}{c}{\textbf{Simulator audit}} & \multicolumn{2}{c}{\textbf{Needs}} & \multicolumn{2}{c}{\textbf{Stops}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Model} & Gen. & Value & $n$ & Planned & Valid & $n$ & Value & $n$ & Cap & Format \\
\midrule
Qwen 3.8 27B & 581 & 87.1 & 565 & 72.3 & 97.8 & 582 & \textbf{95.2} & 190 & 28 & 12 \\
Muse Glimmer 30B & 681 & 69.6 & 618 & 65.4 & 91.8 & 682 & 86.8 & 106 & 314 & 74 \\
GPT-6 Luna & 699 & 84.0 & 630 & 84.3 & 98.4 & 640 & 94.1 & 124 & 36 & 0 \\
Gemini 3.7 Flash & 700 & 87.7 & 593 & 87.1 & 96.6 & 614 & 92.2 & 54 & 139 & 1 \\
Gemini 3.8 Flash & 700 & 88.1 & 595 & 88.6 & 97.7 & 609 & 92.0 & 64 & 100 & 2 \\
Kimi K3 & 685 & 90.1 & 608 & 87.4 & 96.3 & 641 & 94.7 & 85 & 61 & 0 \\
MiniMax M3 & 676 & 67.6 & 479 & 60.3 & 91.7 & 527 & 85.7\rlap{$^{\ast}$} & 19 & 378 & 7 \\
DeepSeek V4.1 Flash & 697 & 88.8 & 618 & 88.1 & 97.6 & 634 & 93.8 & 67 & 58 & 4 \\
GLM 5.3 Flash & 443\rlap{$^{\circ}$} & 92.0 & 426 & 58.1 & 97.3 & 446 & 91.7 & 120 & 32 & 2 \\
Qwen 3.8 Flash & 364\rlap{$^{\circ}$} & 91.2 & 362 & 47.4 & 98.9 & 370 & 94.0 & 116 & 19 & 4 \\
Claude Haiku 5.5 & 700 & 79.0 & 692 & 79.0 & 98.9 & 700 & 86.1 & 590 & 88 & 99 \\
Claude Sonnet 5.5 & 699 & 94.7 & 693 & 94.4 & 99.1 & 699 & 88.2 & 586 & 38 & 4 \\
\addlinespace[2pt]
Grok 4.6 & 700 & 86.8 & 644 & 86.6 & 98.2 & 656 & 92.5 & 123 & 29 & 0 \\
Fable 5.1 & 693 & \textbf{95.5} & 684 & 94.6 & 98.7 & 693 & 90.9 & 585 & 27 & 0 \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}700\rlap{$^{\dagger}$}} & {\color{black!45}94.7\rlap{$^{\dagger}$}} & {\color{black!45}695} & {\color{black!45}94.7} & {\color{black!45}99.3} & {\color{black!45}700} & {\color{black!45}95.4\rlap{$^{\dagger}$}} & {\color{black!45}591} & {\color{black!45}11} & {\color{black!45}0} \\
{\color{black!45}GPT-5.5} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}88.6\rlap{$^{\S}$}} & {\color{black!45}643} & {\color{black!45}88.6} & {\color{black!45}98.5} & {\color{black!45}653} & {\color{black!45}94.8\rlap{$^{\S}$}} & {\color{black!45}102} & {\color{black!45}38} & {\color{black!45}22} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}92.2\rlap{$^{\S}$}} & {\color{black!45}656} & {\color{black!45}92.3} & {\color{black!45}99.1} & {\color{black!45}662} & {\color{black!45}94.9\rlap{$^{\S}$}} & {\color{black!45}129} & {\color{black!45}11} & {\color{black!45}0} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}87.3\rlap{$^{\S}$}} & {\color{black!45}651} & {\color{black!45}87.7} & {\color{black!45}98.3} & {\color{black!45}662} & {\color{black!45}91.3\rlap{$^{\S}$}} & {\color{black!45}89} & {\color{black!45}42} & {\color{black!45}1} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}100.0\rlap{$^{\S}$}} & {\color{black!45}68} & {\color{black!45}97.3} & {\color{black!45}98.6} & {\color{black!45}69} & {\color{black!45}97.3\rlap{$^{\S\ast}$}} & {\color{black!45}19} & {\color{black!45}0} & {\color{black!45}0} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}700\rlap{$^{\S}$}} & {\color{black!45}93.6\rlap{$^{\S}$}} & {\color{black!45}645} & {\color{black!45}93.3} & {\color{black!45}97.7} & {\color{black!45}660} & {\color{black!45}93.9\rlap{$^{\S}$}} & {\color{black!45}117} & {\color{black!45}24} & {\color{black!45}0} \\
\bottomrule
\end{tabular}
\caption{\textbf{Coding: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 700 planned. \emph{Pass rate}: headline (confirmed hidden-test passes of the final submission over completed, simulator-valid episodes) and its $n$; \emph{Planned}: passes over all 700 planned episodes, non-generated ones counted as failures. \emph{Simulator audit}: valid share of audited episodes and the number audited. \emph{Needs}: score over expressed and answered persona-specific needs, with $n$ scoreable eligible persona episodes. \emph{Cap}: conversations stopped at the turn cap; \emph{Format}: final submissions that failed the required format. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. $^{\ast}$ fewer than 50 scoreable episodes. n.r.\ not recorded. Gemini 3.7 / 3.8 Flash follow the original validated judge outputs, as all models do; under the raw-judge score update that their packages also publish they would read Gemini 3.7: task 87.7 ($n$\,=\,674), needs 87.9 ($n$\,=\,578); Gemini 3.8: task 88.3 ($n$\,=\,682), needs 87.5 ($n$\,=\,584).}
\label{tab:domain-coding}
\end{table*}


==> tables/domain_health.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/health_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{4}{c}{\textbf{Inquiry coverage}} &  & \multicolumn{4}{c}{\textbf{Needs}} &  \\
\cmidrule(lr){3-6} \cmidrule(lr){8-11}
\textbf{Model} & Gen. & Value & $n$ & Fail${=}0$ & Partial & Facts & Value & $n$ & Expr. & Opp. & Attr. \\
\midrule
Qwen 3.8 27B & 1,031 & 40.0 & 1,120 & 37.4 & 54.2 & 65.1 & 78.8 & 614 & 51.4 & 96.7 & 49.1 \\
Muse Glimmer 30B & 1,164 & 46.3 & 1,198 & 46.3 & 60.4 & 71.7 & 82.6 & 693 & 47.7 & 99.2 & 46.9 \\
GPT-6 Luna & 1,188 & 27.0 & 1,198 & 27.0 & 39.7 & 45.5 & \textbf{96.5} & 353 & 24.6 & 100.0 & 44.0 \\
Gemini 3.7 Flash & 1,200 & 32.9 & 1,200 & 32.9 & 47.1 & 52.9 & 83.9 & 596 & 44.7 & 100.0 & 54.0 \\
Gemini 3.8 Flash & 1,200 & 32.1 & 1,200 & 32.1 & 45.7 & 51.8 & 83.1 & 590 & 45.2 & 100.0 & 53.9 \\
Kimi K3 & 1,184 & 40.6 & 1,196 & 40.5 & 56.5 & 66.3 & 91.5 & 627 & 45.2 & 100.0 & 47.9 \\
MiniMax M3 & 932\rlap{$^{\circ}$} & \textbf{46.8} & 1,140 & 44.5 & 62.3 & 70.6 & 80.1 & 705 & 57.2 & 94.2 & 50.8 \\
DeepSeek V4.1 Flash & 1,141 & 39.9 & 1,176 & 39.1 & 55.3 & 63.9 & 93.9 & 593 & 42.1 & 98.8 & 46.5 \\
GLM 5.3 Flash & 1,120 & 40.4 & 1,188 & 40.0 & 55.3 & 62.6 & 88.0 & 660 & 49.7 & 98.2 & 49.2 \\
Qwen 3.8 Flash & 1,009 & 39.7 & 1,128 & 37.3 & 54.4 & 63.0 & 77.4 & 585 & 49.0 & 96.0 & 48.7 \\
Claude Haiku 5.5 & 657\rlap{$^{\circ}$} & 39.8 & 1,080 & 35.9 & 54.5 & 61.4 & 91.7 & 450 & 39.7 & 86.4 & 41.0 \\
Claude Sonnet 5.5 & 1,130 & 41.5 & 1,194 & 41.3 & 56.8 & 63.5 & 90.1 & 620 & 43.6 & 97.1 & 43.8 \\
\addlinespace[2pt]
{\color{black!45}Grok 4.6} & {\color{black!45}1,173\rlap{$^{\dagger}$}} & {\color{black!45}45.1\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}45.0} & {\color{black!45}59.0} & {\color{black!45}63.7} & {\color{black!45}97.0\rlap{$^{\dagger}$}} & {\color{black!45}899} & {\color{black!45}57.8} & {\color{black!45}99.9} & {\color{black!45}72.2} \\
{\color{black!45}Fable 5.1} & \multicolumn{11}{l}{\textit{no run}} \\
{\color{black!45}Claude Opus 5.5} & {\color{black!45}1,194\rlap{$^{\dagger}$}} & {\color{black!45}45.7\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}45.7} & {\color{black!45}59.9} & {\color{black!45}65.6} & {\color{black!45}91.6\rlap{$^{\dagger}$}} & {\color{black!45}787} & {\color{black!45}55.6} & {\color{black!45}100.0} & {\color{black!45}63.2} \\
{\color{black!45}GPT-5.5} & {\color{black!45}1,199\rlap{$^{\ddagger}$}} & {\color{black!45}40.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,076} & {\color{black!45}36.5} & n.r. & {\color{black!45}65.3} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}636} & {\color{black!45}44.6} & {\color{black!45}100.0} & {\color{black!45}47.7} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}35.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,128} & {\color{black!45}33.7} & n.r. & {\color{black!45}58.2} & {\color{black!45}97.2\rlap{$^{\ddagger}$}} & {\color{black!45}521} & {\color{black!45}36.2} & {\color{black!45}100.0} & {\color{black!45}45.9} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}34.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,112} & {\color{black!45}31.8} & n.r. & {\color{black!45}56.8} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}485} & {\color{black!45}33.2} & {\color{black!45}100.0} & {\color{black!45}43.7} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}1,200\rlap{$^{\ddagger}$}} & {\color{black!45}34.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,107} & {\color{black!45}31.7} & n.r. & {\color{black!45}55.7} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}476} & {\color{black!45}33.1} & {\color{black!45}100.0} & {\color{black!45}44.0} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}1,187\rlap{$^{\ddagger}$}} & {\color{black!45}26.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,115} & {\color{black!45}24.8} & n.r. & {\color{black!45}44.5} & {\color{black!45}98.0\rlap{$^{\ddagger}$}} & {\color{black!45}395} & {\color{black!45}27.8} & {\color{black!45}100.0} & {\color{black!45}45.7} \\
\bottomrule
\end{tabular}
\caption{\textbf{Health: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 1,200 planned. \emph{Inquiry coverage}: headline (share of applicable source inquiry criteria fully met, over all planned episodes with a task score) and its $n$; \emph{Fail${=}0$}: the same over all 1{,}200 planned episodes with generation failures scored 0; \emph{Partial}: coverage with partial credit for partly met criteria (n.r.\ in score-only packages). \emph{Facts}: share of the patient's source facts the doctor acquired. \emph{Needs}: persona-needs score and $n$ scoreable persona episodes; \emph{Expr.}: share of applicable need items the patient expressed; \emph{Opp.}: share of expressed items the doctor had a chance to answer. \emph{Attr.}: share of persona attributes the simulated patient demonstrated (simulator audit evidence; the Health audit is advisory and has no valid/invalid label). Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. For Gemini 3.7 / 3.8 Flash the raw-judge score update published by their packages gives the same headline values.}
\label{tab:domain-health}
\end{table*}


==> tables/domain_math.tex <==
% Generated by scripts/make_tables.py from data/cells.csv and data/math_cells.csv.
\begin{table*}[tb]
\tablestyle{4.5pt}{1.08}\footnotesize
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}
\toprule
 &  & \multicolumn{6}{c}{\textbf{Tutor correctness}} &  &  & \multicolumn{2}{c}{\textbf{Needs}} &  \\
\cmidrule(lr){3-8} \cmidrule(lr){11-12}
\textbf{Model} & Gen. & Value & $n$ & Arena & HARP & IMO & Neutral & Student & Strict & Value & $n$ & Sim.\ valid \\
\midrule
Qwen 3.8 27B & 1,334 & 91.1 & 1,143 & 98.6 & 90.5 & 79.2 & 87.9 & 98.5 & 58.7 & 81.8 & 1,144 & 99.4 \\
Muse Glimmer 30B & 1,431 & 81.6 & 1,226 & 99.1 & 86.3 & 36.8 & 82.3 & 93.9 & 40.4 & 58.0 & 1,228 & 99.4 \\
GPT-6 Luna & 1,434 & 91.5 & 1,229 & 99.5 & 94.4 & 67.6 & 91.2 & 95.9 & 84.4 & 85.8 & 1,229 & 99.8 \\
Gemini 3.7 Flash & 1,435 & 89.0 & 1,223 & 99.5 & 92.3 & 59.9 & 88.2 & 97.1 & 76.2 & 84.4 & 1,224 & 99.4 \\
Gemini 3.8 Flash & 1,435 & 89.5 & 1,225 & 99.1 & 93.4 & 58.6 & 88.7 & 96.9 & 75.0 & 86.2 & 1,226 & 98.9 \\
Kimi K3 & 1,406 & 92.4 & 1,208 & 98.2 & 94.8 & 72.4 & 90.9 & 97.8 & 68.1 & 84.1 & 1,208 & 99.4 \\
MiniMax M3 & 1,409 & 80.8 & 1,201 & 98.2 & 83.1 & 43.6 & 80.2 & 91.2 & 22.6 & 64.5 & 1,206 & 97.0 \\
DeepSeek V4.1 Flash & 1,411 & 94.5 & 1,206 & 99.5 & 95.2 & 83.3 & 93.6 & 99.3 & 85.7 & 81.5 & 1,206 & 99.9 \\
GLM 5.3 Flash & 1,150 & 94.0 & 984 & 97.7 & 92.7 & 97.1 & 95.2 & 97.6 & 53.3 & 83.8 & 984 & 99.5 \\
Qwen 3.8 Flash & 985\rlap{$^{\circ}$} & \textbf{97.7} & 825 & 98.6 & 97.3 & 100.0 & 98.1 & 99.4 & 87.3 & 85.7 & 825 & 99.7 \\
Claude Haiku 5.5 & 1,435 & 90.7 & 1,230 & 99.1 & 95.6 & 56.9 & 88.3 & 96.5 & 70.3 & 85.3 & 1,229 & 99.2 \\
Claude Sonnet 5.5 & 1,434 & 95.3 & 1,230 & 100.0 & 97.2 & 79.9 & 95.6 & 98.4 & 74.5 & 86.6 & 1,230 & 99.7 \\
\addlinespace[2pt]
Grok 4.6 & 1,402 & 91.9 & 1,203 & 98.6 & 93.2 & 74.5 & 92.3 & 98.5 & 76.2 & 79.9 & 1,204 & 99.5 \\
Fable 5.1 & 1,428 & 96.4 & 1,223 & 100.0 & 96.8 & 89.8 & 96.6 & 99.0 & 77.1 & 89.8 & 1,223 & 99.8 \\
Claude Opus 5.5 & 1,432 & 97.4 & 1,227 & 100.0 & 97.5 & 93.6 & 99.0 & 99.5 & 84.4 & \textbf{90.5} & 1,224 & 99.5 \\
{\color{black!45}GPT-5.5} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}92.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}98.6} & {\color{black!45}93.3} & {\color{black!45}79.9} & {\color{black!45}93.2} & {\color{black!45}99.0} & {\color{black!45}85.4} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}99.7} \\
{\color{black!45}GPT-5.6 Sol} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}95.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}100.0} & {\color{black!45}95.8} & {\color{black!45}86.1} & {\color{black!45}95.1} & {\color{black!45}98.2} & {\color{black!45}87.9} & {\color{black!45}85.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & {\color{black!45}99.9} \\
{\color{black!45}GPT-5.6 Terra} & {\color{black!45}1,433\rlap{$^{\ddagger}$}} & {\color{black!45}88.8\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}99.1} & {\color{black!45}91.5} & {\color{black!45}62.6} & {\color{black!45}88.3} & {\color{black!45}95.8} & {\color{black!45}78.3} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}99.6} \\
{\color{black!45}GPT-6 Astra} & {\color{black!45}1,434\rlap{$^{\ddagger}$}} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & {\color{black!45}99.5} & {\color{black!45}98.8} & {\color{black!45}97.1} & {\color{black!45}99.0} & {\color{black!45}98.7} & {\color{black!45}96.1} & {\color{black!45}91.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & {\color{black!45}99.7} \\
{\color{black!45}GPT-6 Sol} & {\color{black!45}1,435\rlap{$^{\ddagger}$}} & {\color{black!45}95.0\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}98.6} & {\color{black!45}96.3} & {\color{black!45}84.5} & {\color{black!45}97.6} & {\color{black!45}97.6} & {\color{black!45}89.7} & {\color{black!45}89.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & {\color{black!45}99.5} \\
\bottomrule
\end{tabular}
\caption{\textbf{Math: all models and secondary metrics.} Values are percentages unless stated; $n$ counts episodes. \emph{Gen.}: generated conversations of 1,435 planned. \emph{Tutor correctness}: headline (the tutor's final or endorsed solution is correct with valid support) over persona episodes with a tutor grade, its $n$, the same by task bank (SimulatorArena-MATH, HARP, IMO-ProofBench) and for the neutral student. \emph{Student}: the student's final answer is correct; \emph{Strict}: tutor solution correct and free of errors. \emph{Needs}: score over expressed and answered needs and $n$ scoreable persona episodes. \emph{Sim.\ valid}: share of audited episodes whose simulated student passed the persona check. Bold marks the best main-cohort headline. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. n.r.\ not recorded. Gemini 3.7 / 3.8 Flash follow the original validated judge outputs, as all models do; under the raw-judge score update that their packages also publish they would read Gemini 3.7: task 88.8 ($n$\,=\,1,230), needs 84.4 ($n$\,=\,1,230); Gemini 3.8: task 89.5 ($n$\,=\,1,230), needs 86.1 ($n$\,=\,1,230).}
\label{tab:domain-math}
\end{table*}


==> tables/domains.tex <==
% Generated by scripts/make_tables.py from data/domain_facts.json, data/cells.csv and data/*_episodes.csv.gz.
\begin{table*}[t]
\tablestyle{3pt}{1.1}\scriptsize
\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}p{1.55cm} *{6}{>{\raggedright\arraybackslash}X}@{}}
\toprule
 & \textbf{Health} & \textbf{Coding} & \textbf{Math} & \textbf{Finance} & \textbf{Customer Service} & \textbf{Travel} \\
\midrule
\textbf{Source benchmark} & MedDialogRubrics\newline\citep{gong2026meddialogrubrics} & LiveCodeBench\newline\citep{jain2024livecodebench} & SimulatorArena-MATH, HARP, IMO-ProofBench\newline\citep{dou2025simulatorarena,yue2024harp,luong2025imoproofbench} & PRBench-Finance\newline\citep{akyurek2025prbench} & ABCD\newline\citep{chen2021abcd} & UserBench (Travel-44)\newline\citep{qian2025userbench} \\
\addlinespace[1.5pt]
\textbf{Tasks} & 200 cases with inquiry rubrics & 100 selected questions & 205: 37 SimulatorArena, 139 HARP, 29 IMO & 97 questions (finance hard split) & 132 policy items & 72: 67 official + 5 authored revision \\
\addlinespace[1.5pt]
\textbf{Assistant / user} & doctor / patient & coding assistant / developer & tutor / student & financial advisor / client & service agent with policy and tools / customer & travel agent with tools / traveler \\
\addlinespace[1.5pt]
\textbf{Conditions} & 5 personas + neutral & 6 personas + neutral & 6 personas + neutral & 11 personas + neutral (6 shared presets and 5 personas written for each task) & 8 personas + neutral (neutral run 3 times per task) & 5 personas + neutral \\
\addlinespace[1.5pt]
\textbf{Episodes / model} & 1,200 & 700 & 1,435 & 1,164 & 1,452 & 432 \\
\addlinespace[1.5pt]
\textbf{Turn cap} & 20 doctor replies (incl. shared first reply) & 5 assistant turns, then a final submission & 25 tutor turns & 8 assistant turns & 24 agent messages incl. tool follow-ups & 10 assistant replies \\
\addlinespace[1.5pt]
\textbf{Native task metric} & Inquiry coverage: share of applicable source inquiry criteria fully met & Hidden tests passed by the final submission & Tutor's final or endorsed solution correct with valid support (0/1) & Expert rubric percent over the whole conversation (0--100) & Rule-based completion: correct decision, required look-ups, matching action and ending & Choice reward (1 / 0.8 / 0 per aspect) on official tasks; authored tasks scored separately \\
\addlinespace[1.5pt]
\textbf{Needs scored} & Needs expressed, answered and observable & Expressed and answered persona-specific needs & Expressed and answered needs & Expressed and answered needs (strict needs mode) & Expressed and answered needs, simulator-valid episodes & Expressed and answered needs \\
\addlinespace[1.5pt]
\textbf{Simulator audit} & Advisory; no valid/invalid label & Valid / invalid / uncertain; both scores use valid episodes & Valid / invalid & Valid / invalid / uncertain & Valid / invalid / uncertain; needs score uses valid episodes & Valid / invalid / uncertain \\
\addlinespace[1.5pt]
\textbf{Models} & 12 / 19 & 14 / 20 & 15 / 20 & 18 / 20 & 14 / 20 & 19 / 20 \\
\bottomrule
\end{tabularx}
\caption{\textbf{The six domains.} Each column gives a domain's source benchmark and native task metric, its roles (tested assistant / simulated user), the persona conditions beside the neutral user, the planned episodes per model, that is, tasks $\times$ (persona conditions + neutral trials), with 126,460 planned episodes over the 119 runs, the turn cap (a limit, not a target), the needs that enter the persona-needs score and the simulator audit. \emph{Models}: models in the main cohort / models with a run (Appendix~\ref{app:config}). The shared first reply and its exceptions are described in \secref{sec:protocol}, the three judgments in \secref{sec:judgments} and the task populations in \tabref{tab:scorecard-full}.}
\label{tab:domains}
\end{table*}


==> tables/models.tex <==
% Generated by scripts/make_tables.py from data/models.csv and data/cells.csv.
\begin{table*}[t]
\tablestyle{2.5pt}{1.08}\scriptsize
\begin{tabular}{@{}llll>{\raggedright\arraybackslash}p{2.55cm}@{\hspace{5pt}} *{6}{r@{\hspace{6.5pt}}} l@{}}
\toprule
 & & & & & \multicolumn{6}{c}{\textbf{Output budget ($10^3$ tokens)}} & \\
\cmidrule(lr){6-11}
\textbf{Model} & \textbf{Developer} & \textbf{Serving} & \textbf{Thinking} & \textbf{Simulator \& judges} & \textbf{H} & \textbf{C} & \textbf{M} & \textbf{F} & \textbf{S} & \textbf{T} & \textbf{Main cohort} \\
\midrule
Qwen 3.8 27B & Qwen Team, Alibaba & Local vLLM & medium & Luna-m & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 6 \\
Muse Glimmer 30B & n.r. & Local vLLM & medium & Luna-m & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 6 \\
GPT-6 Luna & OpenAI & Hosted API & medium & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
Gemini 3.7 Flash & Google DeepMind & GCP-routed API & medium & Luna-m & n.r. & 32.8\rlap{$^{r}$} & 20 & n.r. & n.r. & 8.2 & 6 \\
Gemini 3.8 Flash & Google DeepMind & GCP-routed API & medium & Luna-m & n.r. & 32.8\rlap{$^{r}$} & 20 & n.r. & n.r. & 8.2 & 6 \\
Kimi K3 & Moonshot AI & Hosted API & medium & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
MiniMax M3 & MiniMax & Hosted API & off & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
DeepSeek V4.1 Flash & DeepSeek & Hosted API & low & Luna-m & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 6 \\
GLM 5.3 Flash & Zhipu AI & Hosted gateway & medium & Luna-m & 12 & 32.8 & 10 & 10 & 10 & 10 & 6 \\
Qwen 3.8 Flash & Qwen Team, Alibaba & Hosted gateway & medium & Luna-m & 12 & 32.8 & 10 & 10 & 10 & 10 & 6 \\
Claude Haiku 5.5 & Anthropic & AWS Bedrock & medium & Luna-m & 12 & 32.8\rlap{$^{r}$} & 12.3\rlap{$^{r}$} & 12.3\rlap{$^{r}$} & n.r.\rlap{$^{r}$} & 8.2 & 6 \\
Claude Sonnet 5.5 & Anthropic & AWS Bedrock & medium & Luna-m & 12 & 32.8\rlap{$^{r}$} & 12.3\rlap{$^{r}$} & 12.3 & n.r.\rlap{$^{r}$} & 8.2 & 6 \\
\midrule
Grok 4.6 & xAI & Hosted API & medium; high (H,F) & Luna-m; Sol-h (H,F) & n.r. & n.r. & n.r. & n.r. & n.r. & n.r. & 4 (C,M,S,T) \\
Fable 5.1 & Anthropic & AWS Bedrock & medium & Luna-m & -- & 65.5 & 65.5 & 65.5 & 65.5 & 65.5 & 5 (C,M,F,S,T) \\
Claude Opus 5.5 & Anthropic & AWS Bedrock & high; medium (M) & Sol-h; Luna-m (M); Sol-h/Luna-m (H,S) & n.r. & 128 & n.r. & 12.3\rlap{$^{r}$} & n.r. & 8.2 & 1 (M) \\
GPT-5.5 & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-5.6 Sol & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-5.6 Terra & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-6 Astra & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
GPT-6 Sol & OpenAI & Hosted API & medium & Luna-m; Luna-h/n.r. (M) & n.r. & 128 & 20 & n.r. & n.r. & 8.2 & 2 (F,T) \\
\bottomrule
\end{tabular}
\caption{\textbf{Tested models.} The first 12 models are in the main cohort of all six domains (H Health, C Coding, M Math, F Finance, S Customer Service, T Travel). \emph{Developer}: attributed from the model family, as the run records give only model identifiers. \emph{Thinking}: the tested assistant's reasoning setting. \emph{Simulator \& judges}: the model behind the simulated user, the task and needs judges and the simulator audit; Luna-m = GPT-6 Luna at medium effort, Sol-h = GPT-5.6 Sol at high effort, Sol-h/Luna-m = differs by condition (H) or by episode (S), Luna-h/n.r.\ = GPT-6 Luna at high or unrecorded effort by role. \emph{Output budget}: the tested assistant's maximum output tokens; $^{r}$ = failed generations rerun under a documented recovery amendment with a budget of 65,536 tokens and kept in the headline (for Claude Haiku 5.5 and Claude Sonnet 5.5 in Customer Service, the only recorded budget); separately reported recoveries are not marked. n.r.\ = not recorded; -- = no run. \emph{Main cohort}: number of domains in whose main cohort (Appendix~\ref{app:cohort}) the run lies.}
\label{tab:models}
\end{table*}


==> tables/persona_effects.tex <==
% Generated by scripts/make_tables.py from data/persona_effects.csv (main-cohort rows only).
\begin{table*}[p]
\tablestyle{4pt}{1.04}\scriptsize
\begin{tabular}{@{}l r rrrr rr@{}}
\toprule
 & & \multicolumn{4}{c}{\textbf{Persona $-$ neutral (points)}} & \multicolumn{2}{c}{\textbf{95\% CI excludes 0}} \\
\cmidrule(lr){3-6} \cmidrule(l){7-8}
\textbf{Condition} & \textbf{Models} & \textbf{Mean} & \textbf{Median} & \textbf{Min} & \textbf{Max} & \textbf{Below} & \textbf{Above} \\
\midrule
\multicolumn{8}{@{}l}{\textbf{Health} \textit{(inquiry coverage; neutral mean 39.9 over 12 main-cohort models)}} \\
\hspace{0.6em}P1: Receptive novice & 12 & $-$2.9 & $-$2.9 & $-$5.9 & $-$0.6 & 8 & 0 \\
\hspace{0.6em}P2: Informed questioner & 12 & $+$2.2 & $+$1.8 & $-$0.1 & $+$5.7 & 0 & 6 \\
\hspace{0.6em}P3: Private, time-conscious novice & 12 & $-$3.8 & $-$3.6 & $-$5.7 & $-$2.2 & 12 & 0 \\
\hspace{0.6em}P4: Guarded, time-conscious novice & 12 & $-$3.2 & $-$3.0 & $-$5.2 & $-$1.4 & 11 & 0 \\
\hspace{0.6em}P5: Receptive, informed contributor & 12 & $+$2.1 & $+$2.3 & $-$1.4 & $+$5.2 & 0 & 8 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{All personas pooled} & 12 & $-$1.1 & $-$1.1 & $-$3.1 & $+$0.1 & 5 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Coding} \textit{(pass rate; neutral mean 87.1 over 14 main-cohort models)}} \\
\hspace{0.6em}495132: Detailed typed professional & 14 & $-$10.3 & $-$7.7 & $-$30.0 & $+$4.0 & 7 & 0 \\
\hspace{0.6em}518717: Performance-focused student & 14 & $-$2.5 & $-$1.5 & $-$10.1 & $+$5.6 & 3 & 0 \\
\hspace{0.6em}690429: Deadline-driven technologist & 14 & $-$0.2 & $-$0.5 & $-$10.3 & $+$8.2 & 0 & 0 \\
\hspace{0.6em}809272: Examples-first minimalist & 14 & $+$1.6 & $+$2.0 & $-$3.3 & $+$7.7 & 0 & 0 \\
\hspace{0.6em}835253: Plain-language technologist & 14 & $-$0.1 & $-$0.5 & $-$9.2 & $+$4.9 & 0 & 0 \\
\hspace{0.6em}992645: Examples-first learner & 14 & $+$0.5 & 0.0 & $-$3.8 & $+$6.8 & 0 & 0 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{All personas pooled} & 14 & $-$1.9 & $-$1.6 & $-$6.8 & $+$4.0 & 2 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Math} \textit{(tutor correctness; neutral mean 91.2 over 15 main-cohort models)}} \\
\hspace{0.6em}P1: Concise independent learner & 15 & $+$0.6 & $+$1.0 & $-$2.8 & $+$3.7 & 1 & 0 \\
\hspace{0.6em}P2: Detail-oriented checker & 15 & $+$1.7 & $+$1.0 & $-$0.5 & $+$7.5 & 0 & 1 \\
\hspace{0.6em}P3: Example-led explorer & 15 & $+$0.3 & 0.0 & $-$2.8 & $+$4.4 & 0 & 1 \\
\hspace{0.6em}P4: Intuitive demonstration seeker & 15 & $+$0.1 & $+$0.5 & $-$3.0 & $+$2.5 & 1 & 0 \\
\hspace{0.6em}P5: Anxious starter & 15 & $-$0.6 & $-$0.5 & $-$4.1 & $+$2.2 & 0 & 0 \\
\hspace{0.6em}P6: Frustrated learner & 15 & $+$0.7 & $+$1.0 & $-$2.5 & $+$3.5 & 0 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Finance} \textit{(rubric percent; neutral mean 43.6 over 18 main-cohort models)}} \\
\hspace{0.6em}CL: Careful learner & 18 & $+$0.4 & $+$0.5 & $-$3.0 & $+$2.6 & 0 & 3 \\
\hspace{0.6em}SQ: Skeptical questioner & 18 & $+$1.6 & $+$1.1 & $-$1.2 & $+$6.4 & 0 & 4 \\
\hspace{0.6em}CP: Concise pragmatist & 18 & $-$0.3 & $-$0.5 & $-$4.0 & $+$2.6 & 1 & 0 \\
\hspace{0.6em}DP: Decisive pusher & 18 & $+$2.4 & $+$2.5 & $-$0.9 & $+$4.9 & 0 & 9 \\
\hspace{0.6em}CC: Confident contrarian & 18 & $+$2.6 & $+$2.1 & $-$1.1 & $+$6.8 & 0 & 8 \\
\hspace{0.6em}RS: Reassurance seeker & 18 & $+$0.4 & $+$0.4 & $-$2.9 & $+$3.1 & 1 & 2 \\
\hspace{0.6em}D1: Designed persona 1 (task-specific) & 18 & $+$0.7 & $+$0.5 & $-$1.7 & $+$3.1 & 0 & 2 \\
\hspace{0.6em}D2: Designed persona 2 (task-specific) & 18 & $+$4.3 & $+$4.8 & $+$0.4 & $+$8.7 & 0 & 13 \\
\hspace{0.6em}D3: Designed persona 3 (task-specific) & 18 & $+$3.6 & $+$3.0 & $+$1.0 & $+$7.5 & 0 & 12 \\
\hspace{0.6em}D4: Designed persona 4 (task-specific) & 18 & $+$3.4 & $+$3.3 & $+$0.5 & $+$6.3 & 0 & 12 \\
\hspace{0.6em}D5: Designed persona 5 (task-specific) & 18 & $+$3.2 & $+$3.3 & $-$1.2 & $+$6.1 & 0 & 11 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{Six shared presets pooled} & 18 & $+$1.2 & $+$1.1 & $-$1.7 & $+$3.5 & 0 & 5 \\
\hspace{0.6em}\textit{Five designed personas pooled} & 18 & $+$3.0 & $+$2.9 & $+$0.3 & $+$5.8 & 0 & 13 \\
\hspace{0.6em}\textit{All personas pooled} & 18 & $+$2.0 & $+$2.1 & $-$0.8 & $+$4.5 & 0 & 11 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Customer Service} \textit{(task completion; neutral mean 72.5 over 14 main-cohort models)}} \\
\hspace{0.6em}P2: Frustrated on refusal & 14 & $-$0.5 & $-$0.6 & $-$8.8 & $+$6.4 & 1 & 0 \\
\hspace{0.6em}C2: Self-doubt & 14 & $+$0.7 & $+$0.3 & $-$4.0 & $+$5.8 & 0 & 0 \\
\hspace{0.6em}C3: Gives up early & 14 & $-$7.2 & $-$6.8 & $-$14.1 & $-$0.3 & 7 & 0 \\
\hspace{0.6em}A03: Money matters & 14 & $-$0.7 & $-$1.6 & $-$12.6 & $+$7.1 & 2 & 1 \\
\hspace{0.6em}A09: Wants the reason & 14 & $-$7.5 & $-$9.3 & $-$13.4 & $+$0.9 & 7 & 0 \\
\hspace{0.6em}A10: Bundles questions & 14 & $-$4.6 & $-$4.7 & $-$13.9 & $+$5.1 & 4 & 0 \\
\hspace{0.6em}A11: Risk-sensitive & 14 & $-$3.8 & $-$2.5 & $-$12.4 & $+$0.8 & 2 & 0 \\
\hspace{0.6em}A12: Wants options & 14 & $-$1.8 & $-$1.8 & $-$9.6 & $+$5.1 & 1 & 0 \\
\addlinespace[3pt]
\multicolumn{8}{@{}l}{\textbf{Travel} \textit{(choice reward; neutral mean 73.4 over 19 main-cohort models)}} \\
\hspace{0.6em}CP: Careful planner & 19 & $-$10.4 & $-$10.9 & $-$25.2 & $+$6.2 & 13 & 0 \\
\hspace{0.6em}SC: Skeptical comparer & 19 & $-$24.1 & $-$21.6 & $-$40.8 & $-$10.0 & 19 & 0 \\
\hspace{0.6em}CD: Concise decider & 19 & $-$16.7 & $-$16.7 & $-$29.6 & $-$8.8 & 16 & 0 \\
\hspace{0.6em}EC: Efficient comparer & 19 & $-$13.3 & $-$12.7 & $-$26.1 & $-$1.6 & 13 & 0 \\
\hspace{0.6em}CN: Concise planner & 19 & $-$1.4 & $-$0.4 & $-$13.9 & $+$11.5 & 3 & 2 \\
\cmidrule(l){1-8}
\hspace{0.6em}\textit{All personas pooled} & 19 & $-$13.1 & $-$13.8 & $-$24.2 & $-$2.2 & 16 & 0 \\
\bottomrule
\end{tabular}
\caption{\textbf{Change in the native task score under each persona, relative to the neutral user.} For each main-cohort model, the paired change is the mean over tasks of the persona episode's task score minus the neutral episode's score on the same task (same initial question and same first assistant reply; in Math the opening and first reply are generated per persona, so the Math contrast also includes the opening), in percentage points (Finance: rubric points; Travel: reward$\times$100); tasks enter only when both episodes have a task score. \emph{Mean}, \emph{Median}, \emph{Min} and \emph{Max} summarize the per-model changes over the main-cohort models with a paired estimate (\emph{Models}); \emph{Below} / \emph{Above} count models whose 95\% task-cluster bootstrap interval (5{,}000 resamples) lies entirely below / above zero. Pooled rows treat the persona conditions together (Finance: also the six shared presets and the five designed personas as groups), paired by task with the neutral user. Finance designed personas D1--D5 are written separately for each task; Math and Customer Service have no pooled estimate in the data. In Customer Service the contrast uses graded completed episodes (the task headline uses all planned episodes, incomplete ones scored 0), and the neutral score averages the task's graded neutral trials (up to three), of which only the first shares the persona conditions' first reply.}
\label{tab:persona-effects}
\end{table*}


==> tables/scorecard.tex <==
% Generated by scripts/make_tables.py from data/cells.csv (headline columns task_value, needs_value).
\begin{table*}[t]
\tablestyle{4pt}{1.06}
\begin{tabular}{@{}l@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{13pt}}r@{\hspace{11pt}}r@{\hspace{5pt}}}
\toprule
 & \multicolumn{2}{c}{\textbf{Health}} & \multicolumn{2}{c}{\textbf{Coding}} & \multicolumn{2}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Finance}} & \multicolumn{2}{c}{\textbf{Cust.\ Service}} & \multicolumn{2}{c}{\textbf{Travel}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
\textbf{Model} & Task & Needs & Task & Needs & Task & Needs & Task & Needs & Task & Needs & Task & Needs \\
\midrule
\multicolumn{13}{@{}l}{\textit{Main cohort in all six domains}} \\
Qwen 3.8 27B & 40.0 & 78.8 & 87.1 & \textbf{95.2} & 91.1 & 81.8 & 45.4 & 56.7 & 71.3 & 74.0 & 63.9 & 91.1 \\
Muse Glimmer 30B & 46.3 & 82.6 & 69.6 & 86.8 & 81.6 & 58.0 & 35.4 & 62.7 & 35.5 & 47.5 & 54.7 & 93.7 \\
GPT-6 Luna & 27.0 & \textbf{96.5} & 84.0 & 94.1 & 91.5 & 85.8 & 35.7 & \textbf{90.1} & 75.2 & 69.2 & 47.7 & 87.1 \\
Gemini 3.7 Flash & 32.9 & 83.9 & 87.7 & 92.2 & 89.0 & 84.4 & 43.5 & 61.4 & 92.6 & 75.9 & \textbf{86.6} & 85.2 \\
Gemini 3.8 Flash & 32.1 & 83.1 & 88.1 & 92.0 & 89.5 & 86.2 & 45.1 & 63.1 & \textbf{94.1} & 78.4 & 76.3 & 88.1 \\
Kimi K3 & 40.6 & 91.5 & 90.1 & 94.7 & 92.4 & 84.1 & 47.2 & 68.5 & 74.5 & 79.3 & 71.1 & 88.2 \\
MiniMax M3 & \textbf{46.8}\rlap{$^{\circ}$} & 80.1\rlap{$^{\circ}$} & 67.6 & 85.7\rlap{$^{\ast}$} & 80.8 & 64.5 & 43.1 & 55.4 & 22.7 & 65.2 & 38.4 & 88.8 \\
DeepSeek V4.1 Flash & 39.9 & 93.9 & 88.8 & 93.8 & 94.5 & 81.5 & 44.0 & 77.8 & 72.0 & 69.4 & 73.6 & 85.5 \\
GLM 5.3 Flash & 40.4 & 88.0 & 92.0\rlap{$^{\circ}$} & 91.7\rlap{$^{\circ}$} & 94.0 & 83.8 & 46.9 & 66.3 & 56.3 & 74.9 & 64.2 & 86.3 \\
Qwen 3.8 Flash & 39.7 & 77.4 & 91.2\rlap{$^{\circ}$} & 94.0\rlap{$^{\circ}$} & \textbf{97.7}\rlap{$^{\circ}$} & 85.7\rlap{$^{\circ}$} & 48.7 & 57.2 & 60.5 & 73.3 & 66.6 & 87.6 \\
Claude Haiku 5.5 & 39.8\rlap{$^{\circ}$} & 91.7\rlap{$^{\circ}$} & 79.0 & 86.1 & 90.7 & 85.3 & 37.6 & 74.1 & 69.6 & 70.2 & 40.3 & 93.0 \\
Claude Sonnet 5.5 & 41.5 & 90.1 & 94.7 & 88.2 & 95.3 & 86.6 & 52.3 & 72.7 & 86.8 & 71.0 & 79.3 & 84.2 \\
\midrule
\multicolumn{13}{@{}l}{\textit{Main cohort in some domains}} \\
Grok 4.6 & {\color{black!45}45.1\rlap{$^{\dagger}$}} & {\color{black!45}97.0\rlap{$^{\dagger}$}} & 86.8 & 92.5 & 91.9 & 79.9 & {\color{black!45}51.5\rlap{$^{\dagger}$}} & {\color{black!45}80.4\rlap{$^{\dagger}$}} & 83.6 & 65.6 & 75.6 & 85.2 \\
Fable 5.1 & -- & -- & \textbf{95.5} & 90.9 & 96.4 & 89.8 & \textbf{57.1} & 70.1 & 87.7 & \textbf{80.2} & 79.7 & 87.8 \\
Claude Opus 5.5 & {\color{black!45}45.7\rlap{$^{\dagger}$}} & {\color{black!45}91.6\rlap{$^{\dagger}$}} & {\color{black!45}94.7\rlap{$^{\dagger}$}} & {\color{black!45}95.4\rlap{$^{\dagger}$}} & 97.4 & \textbf{90.5} & {\color{black!45}64.6\rlap{$^{\dagger}$}} & {\color{black!45}77.9\rlap{$^{\dagger}$}} & {\color{black!45}85.8\rlap{$^{\dagger}$}} & {\color{black!45}72.4\rlap{$^{\dagger}$}} & {\color{black!45}63.7\rlap{$^{\dagger}$}} & {\color{black!45}93.1\rlap{$^{\dagger}$}} \\
GPT-5.5 & {\color{black!45}40.7\rlap{$^{\ddagger}$}} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}88.6\rlap{$^{\S}$}} & {\color{black!45}94.8\rlap{$^{\S}$}} & {\color{black!45}92.4\rlap{$^{\ddagger}$}} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & 48.8 & 78.7 & {\color{black!45}89.9\rlap{$^{\ddagger}$}} & {\color{black!45}78.1\rlap{$^{\ddagger}$}} & 64.2 & 91.0 \\
GPT-5.6 Sol & {\color{black!45}35.9\rlap{$^{\ddagger}$}} & {\color{black!45}97.2\rlap{$^{\ddagger}$}} & {\color{black!45}92.2\rlap{$^{\S}$}} & {\color{black!45}94.9\rlap{$^{\S}$}} & {\color{black!45}95.2\rlap{$^{\ddagger}$}} & {\color{black!45}85.3\rlap{$^{\ddagger}$}} & 50.6 & 85.3 & {\color{black!45}88.9\rlap{$^{\ddagger}$}} & {\color{black!45}78.5\rlap{$^{\ddagger}$}} & 52.6 & 87.6 \\
GPT-5.6 Terra & {\color{black!45}34.3\rlap{$^{\ddagger}$}} & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}87.3\rlap{$^{\S}$}} & {\color{black!45}91.3\rlap{$^{\S}$}} & {\color{black!45}88.8\rlap{$^{\ddagger}$}} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & 47.3 & 82.6 & {\color{black!45}89.3\rlap{$^{\ddagger}$}} & {\color{black!45}72.9\rlap{$^{\ddagger}$}} & 66.8 & 88.3 \\
GPT-6 Astra & {\color{black!45}34.4\rlap{$^{\ddagger}$}} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}100.0\rlap{$^{\S}$}} & {\color{black!45}97.3\rlap{$^{\S\ast}$}} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}91.3\rlap{$^{\ddagger}$}} & 50.6 & 90.0 & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}76.3\rlap{$^{\ddagger}$}} & 44.0 & \textbf{94.0} \\
GPT-6 Sol & {\color{black!45}26.7\rlap{$^{\ddagger}$}} & {\color{black!45}98.0\rlap{$^{\ddagger}$}} & {\color{black!45}93.6\rlap{$^{\S}$}} & {\color{black!45}93.9\rlap{$^{\S}$}} & {\color{black!45}95.0\rlap{$^{\ddagger}$}} & {\color{black!45}89.2\rlap{$^{\ddagger}$}} & 36.0 & 88.8 & {\color{black!45}82.2\rlap{$^{\ddagger}$}} & {\color{black!45}74.3\rlap{$^{\ddagger}$}} & 41.2 & 90.1 \\
\midrule
\textit{Main-cohort mean} & 38.9 & 86.5 & 85.9 & 91.3 & 91.6 & 81.9 & 45.3 & 72.3 & 70.2 & 71.0 & 62.5 & 88.6 \\
\textit{Main-cohort models} & \multicolumn{2}{c}{12} & \multicolumn{2}{c}{14} & \multicolumn{2}{c}{15} & \multicolumn{2}{c}{18} & \multicolumn{2}{c}{14} & \multicolumn{2}{c}{19} \\
\bottomrule
\end{tabular}
\caption{\textbf{Scorecard.} Native task score (\emph{Task}) and persona-needs score (\emph{Needs}) for every tested model in every domain, as percentages (Finance task: PRBench rubric percent). Task metrics are the source benchmarks' own: Health inquiry coverage, Coding hidden-test pass rate, Math tutor-solution correctness, Finance expert-rubric percent, Customer Service rule-based task completion and Travel UserBench choice reward (Figure~\ref{fig:domains}). Each task score uses its domain's native population; each needs score averages persona episodes in which the user expressed at least one need and the assistant had a chance to answer it (in Coding and Customer Service, only completed simulator-valid episodes). Task and needs scores are not comparable across domains. Bold marks the best main-cohort value in each column; the last rows give the main-cohort mean and the number of main-cohort models per domain. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. $^{\ast}$ needs score over fewer than 50 scoreable episodes. -- no run. Denominators are given in \tabref{tab:scorecard-full}, coverage in \tabref{tab:coverage}.}
\label{tab:scorecard}
\end{table*}


==> tables/scorecard_full.tex <==
% Generated by scripts/make_tables.py from data/cells.csv (task_value/task_den, needs_value/needs_den).
\begin{table*}[p]
\tablestyle{3.2pt}{1.04}\scriptsize
\begin{tabular}{@{}l *{6}{r@{\hspace{10pt}}r}@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Health}} & \multicolumn{2}{c}{\textbf{Coding}} & \multicolumn{2}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Finance}} & \multicolumn{2}{c}{\textbf{Cust.\ Service}} & \multicolumn{2}{c}{\textbf{Travel}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
\textbf{Model} & Value & $n$ & Value & $n$ & Value & $n$ & Value & $n$ & Value & $n$ & Value & $n$ \\
\midrule
\multicolumn{13}{@{}l}{\textbf{A. Native task score}} \\
Qwen 3.8 27B & 40.0 & 1,120 & 87.1 & 565 & 91.1 & 1,143 & 45.4 & 1,060 & 71.3 & 1,452 & 63.9 & 402 \\
Muse Glimmer 30B & 46.3 & 1,198 & 69.6 & 618 & 81.6 & 1,226 & 35.4 & 1,118 & 35.5 & 1,452 & 54.7 & 364 \\
GPT-6 Luna & 27.0 & 1,198 & 84.0 & 630 & 91.5 & 1,229 & 35.7 & 1,102 & 75.2 & 1,452 & 47.7 & 401 \\
Gemini 3.7 Flash & 32.9 & 1,200 & 87.7 & 593 & 89.0 & 1,223 & 43.5 & 1,065 & 92.6 & 1,452 & \textbf{86.6} & 402 \\
Gemini 3.8 Flash & 32.1 & 1,200 & 88.1 & 595 & 89.5 & 1,225 & 45.1 & 1,090 & \textbf{94.1} & 1,452 & 76.3 & 402 \\
Kimi K3 & 40.6 & 1,196 & 90.1 & 608 & 92.4 & 1,208 & 47.2 & 1,107 & 74.5 & 1,452 & 71.1 & 400 \\
MiniMax M3 & \textbf{46.8}\rlap{$^{\circ}$} & 1,140 & 67.6 & 479 & 80.8 & 1,201 & 43.1 & 965 & 22.7 & 1,452 & 38.4 & 336 \\
DeepSeek V4.1 Flash & 39.9 & 1,176 & 88.8 & 618 & 94.5 & 1,206 & 44.0 & 1,108 & 72.0 & 1,452 & 73.6 & 401 \\
GLM 5.3 Flash & 40.4 & 1,188 & 92.0\rlap{$^{\circ}$} & 426 & 94.0 & 984 & 46.9 & 1,081 & 56.3 & 1,452 & 64.2 & 402 \\
Qwen 3.8 Flash & 39.7 & 1,128 & 91.2\rlap{$^{\circ}$} & 362 & \textbf{97.7}\rlap{$^{\circ}$} & 825 & 48.7 & 890 & 60.5 & 1,452 & 66.6 & 402 \\
Claude Haiku 5.5 & 39.8\rlap{$^{\circ}$} & 1,080 & 79.0 & 692 & 90.7 & 1,230 & 37.6 & 1,164 & 69.6 & 1,452 & 40.3 & 400 \\
Claude Sonnet 5.5 & 41.5 & 1,194 & 94.7 & 693 & 95.3 & 1,230 & 52.3 & 1,164 & 86.8 & 1,452 & 79.3 & 402 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}45.1\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & 86.8 & 644 & 91.9 & 1,203 & {\color{black!45}51.5\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & 83.6 & 1,452 & 75.6 & 399 \\
Fable 5.1 & -- &  & \textbf{95.5} & 684 & 96.4 & 1,223 & \textbf{57.1} & 1,164 & 87.7 & 1,452 & 79.7 & 402 \\
Claude Opus 5.5 & {\color{black!45}45.7\rlap{$^{\dagger}$}} & {\color{black!45}1,199} & {\color{black!45}94.7\rlap{$^{\dagger}$}} & {\color{black!45}695} & 97.4 & 1,227 & {\color{black!45}64.6\rlap{$^{\dagger}$}} & {\color{black!45}1,163} & {\color{black!45}85.8\rlap{$^{\dagger}$}} & {\color{black!45}1,452} & {\color{black!45}63.7\rlap{$^{\dagger}$}} & {\color{black!45}401} \\
GPT-5.5 & {\color{black!45}40.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,076} & {\color{black!45}88.6\rlap{$^{\S}$}} & {\color{black!45}643} & {\color{black!45}92.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 48.8 & 1,122 & {\color{black!45}89.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 64.2 & 401 \\
GPT-5.6 Sol & {\color{black!45}35.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,128} & {\color{black!45}92.2\rlap{$^{\S}$}} & {\color{black!45}656} & {\color{black!45}95.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 50.6 & 1,146 & {\color{black!45}88.9\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 52.6 & 396 \\
GPT-5.6 Terra & {\color{black!45}34.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,112} & {\color{black!45}87.3\rlap{$^{\S}$}} & {\color{black!45}651} & {\color{black!45}88.8\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 47.3 & 1,130 & {\color{black!45}89.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 66.8 & 402 \\
GPT-6 Astra & {\color{black!45}34.4\rlap{$^{\ddagger}$}} & {\color{black!45}1,107} & {\color{black!45}100.0\rlap{$^{\S}$}} & {\color{black!45}68} & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & 50.6 & 1,108 & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 44.0 & 398 \\
GPT-6 Sol & {\color{black!45}26.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,115} & {\color{black!45}93.6\rlap{$^{\S}$}} & {\color{black!45}645} & {\color{black!45}95.0\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 36.0 & 1,153 & {\color{black!45}82.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,452} & 41.2 & 401 \\
\midrule
\multicolumn{13}{@{}l}{\textbf{B. Persona-needs score}} \\
Qwen 3.8 27B & 78.8 & 614 & \textbf{95.2} & 190 & 81.8 & 1,144 & 56.7 & 1,000 & 74.0 & 706 & 91.1 & 270 \\
Muse Glimmer 30B & 82.6 & 693 & 86.8 & 106 & 58.0 & 1,228 & 62.7 & 1,007 & 47.5 & 683 & 93.7 & 277 \\
GPT-6 Luna & \textbf{96.5} & 353 & 94.1 & 124 & 85.8 & 1,229 & \textbf{90.1} & 867 & 69.2 & 665 & 87.1 & 261 \\
Gemini 3.7 Flash & 83.9 & 596 & 92.2 & 54 & 84.4 & 1,224 & 61.4 & 1,033 & 75.9 & 677 & 85.2 & 251 \\
Gemini 3.8 Flash & 83.1 & 590 & 92.0 & 64 & 86.2 & 1,226 & 63.1 & 1,009 & 78.4 & 695 & 88.1 & 254 \\
Kimi K3 & 91.5 & 627 & 94.7 & 85 & 84.1 & 1,208 & 68.5 & 994 & 79.3 & 682 & 88.2 & 243 \\
MiniMax M3 & 80.1\rlap{$^{\circ}$} & 705 & 85.7\rlap{$^{\ast}$} & 19 & 64.5 & 1,206 & 55.4 & 1,038 & 65.2 & 697 & 88.8 & 186 \\
DeepSeek V4.1 Flash & 93.9 & 593 & 93.8 & 67 & 81.5 & 1,206 & 77.8 & 981 & 69.4 & 698 & 85.5 & 267 \\
GLM 5.3 Flash & 88.0 & 660 & 91.7\rlap{$^{\circ}$} & 120 & 83.8 & 984 & 66.3 & 978 & 74.9 & 719 & 86.3 & 274 \\
Qwen 3.8 Flash & 77.4 & 585 & 94.0\rlap{$^{\circ}$} & 116 & 85.7\rlap{$^{\circ}$} & 825 & 57.2 & 822 & 73.3 & 717 & 87.6 & 268 \\
Claude Haiku 5.5 & 91.7\rlap{$^{\circ}$} & 450 & 86.1 & 590 & 85.3 & 1,229 & 74.1 & 996 & 70.2 & 710 & 93.0 & 292 \\
Claude Sonnet 5.5 & 90.1 & 620 & 88.2 & 586 & 86.6 & 1,230 & 72.7 & 990 & 71.0 & 693 & 84.2 & 294 \\
\addlinespace[2pt]
Grok 4.6 & {\color{black!45}97.0\rlap{$^{\dagger}$}} & {\color{black!45}899} & 92.5 & 123 & 79.9 & 1,204 & {\color{black!45}80.4\rlap{$^{\dagger}$}} & {\color{black!45}1,028} & 65.6 & 705 & 85.2 & 275 \\
Fable 5.1 & -- &  & 90.9 & 585 & 89.8 & 1,223 & 70.1 & 1,005 & \textbf{80.2} & 716 & 87.8 & 288 \\
Claude Opus 5.5 & {\color{black!45}91.6\rlap{$^{\dagger}$}} & {\color{black!45}787} & {\color{black!45}95.4\rlap{$^{\dagger}$}} & {\color{black!45}591} & \textbf{90.5} & 1,224 & {\color{black!45}77.9\rlap{$^{\dagger}$}} & {\color{black!45}1,035} & {\color{black!45}72.4\rlap{$^{\dagger}$}} & {\color{black!45}740} & {\color{black!45}93.1\rlap{$^{\dagger}$}} & {\color{black!45}360} \\
GPT-5.5 & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}636} & {\color{black!45}94.8\rlap{$^{\S}$}} & {\color{black!45}102} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 78.7 & 982 & {\color{black!45}78.1\rlap{$^{\ddagger}$}} & {\color{black!45}715} & 91.0 & 291 \\
GPT-5.6 Sol & {\color{black!45}97.2\rlap{$^{\ddagger}$}} & {\color{black!45}521} & {\color{black!45}94.9\rlap{$^{\S}$}} & {\color{black!45}129} & {\color{black!45}85.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,229} & 85.3 & 909 & {\color{black!45}78.5\rlap{$^{\ddagger}$}} & {\color{black!45}702} & 87.6 & 270 \\
GPT-5.6 Terra & {\color{black!45}95.8\rlap{$^{\ddagger}$}} & {\color{black!45}485} & {\color{black!45}91.3\rlap{$^{\S}$}} & {\color{black!45}89} & {\color{black!45}82.7\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 82.6 & 928 & {\color{black!45}72.9\rlap{$^{\ddagger}$}} & {\color{black!45}696} & 88.3 & 282 \\
GPT-6 Astra & {\color{black!45}98.7\rlap{$^{\ddagger}$}} & {\color{black!45}476} & {\color{black!45}97.3\rlap{$^{\S\ast}$}} & {\color{black!45}19} & {\color{black!45}91.3\rlap{$^{\ddagger}$}} & {\color{black!45}1,228} & 90.0 & 846 & {\color{black!45}76.3\rlap{$^{\ddagger}$}} & {\color{black!45}744} & \textbf{94.0} & 264 \\
GPT-6 Sol & {\color{black!45}98.0\rlap{$^{\ddagger}$}} & {\color{black!45}395} & {\color{black!45}93.9\rlap{$^{\S}$}} & {\color{black!45}117} & {\color{black!45}89.2\rlap{$^{\ddagger}$}} & {\color{black!45}1,230} & 88.8 & 860 & {\color{black!45}74.3\rlap{$^{\ddagger}$}} & {\color{black!45}719} & 90.1 & 282 \\
\bottomrule
\end{tabular}
\caption{\textbf{Scorecard with denominators.} Values as in \tabref{tab:scorecard} (percent; Finance task: rubric percent); $n$ is the number of episodes behind each value. Task populations follow each benchmark's native rule: Health, all planned episodes with a task score (graded partial dialogues included); Coding, completed simulator-valid episodes; Math, persona episodes with a tutor grade; Finance, recorded episodes with a valid advice grade; Customer Service, all planned episodes (incomplete ones count as not completed); Travel, recorded official-task episodes with a score. Needs $n$ counts persona episodes with at least one expressed and answered need; in Coding and Customer Service only completed episodes with a valid simulator audit count, so this $n$ can be smaller than \emph{Scor.} in \tabref{tab:coverage}. Rows below the gap are the models outside the main cohort in at least one domain. Bold marks the best main-cohort value per column. Gray values with markers are outside the main cohort: $^{\dagger}$ simulator and judges not all GPT-6 Luna at medium effort (GPT-5.6 Sol at high effort for some or all roles); $^{\ddagger}$ score-only package without full dialogue evidence (registry status unverified; in Math these packages also lack an exact panel record and use GPT-6 Luna at high or unrecorded effort); $^{\S}$ run listed as partial in the registry. $^{\circ}$ fewer than 80\% of planned episodes generated. $^{\ast}$ fewer than 50 scoreable episodes. -- no run. Health values use the \texttt{llm\_judgment\_v1} judge-acceptance policy, except the five score-only GPT packages ($^{\ddagger}$), which provide only the stricter native acceptance policy. Gemini 3.7 / 3.8 Flash use the original validated judge outputs, as all other models do; their packages also publish a raw-judge score update, reported in the domain tables.}
\label{tab:scorecard-full}
\end{table*}


==> tables/supp_coding.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Coding, 20 hard LiveCodeBench tasks.} Persona pass is conditional on publicly expressed critical needs (analysis version \emph{publicly-expressed-critical-needs-v1}); intervals are 95\% Wilson and treat episodes as independent. Critical needs counts are needs with a public request and an assistant reply over applicable critical needs. Source: examples/coding-hard20-paper-reference.}
\label{tab:supp-coding}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Card} & \textbf{Tests passed} & \textbf{Persona pass (\%)} & \textbf{Critical needs answered (\%)} & \textbf{Need credit} \\
\midrule
Detailed typed professional & 18/20 & 100.0 {\scriptsize [83.9, 100.0]} (20/20) & 87.0 (40/46) & 0.97 \\
Concise skeptical professional & 20/20 & 90.0 {\scriptsize [69.9, 97.2]} (18/20) & 92.0 (46/50) & 0.97 \\
Performance-focused student & 19/19 & 66.7 {\scriptsize [43.7, 83.7]} (12/18) & 71.4 (60/84) & 0.95 \\
Trade-off-focused professional & 19/19 & 89.5 {\scriptsize [68.6, 97.1]} (17/19) & 97.2 (35/36) & 0.97 \\
Maintainability-minded reviewer & 20/20 & 73.7 {\scriptsize [51.2, 88.2]} (14/19) & 83.1 (54/65) & 0.92 \\
Deadline-driven technologist & 20/20 & 73.7 {\scriptsize [51.2, 88.2]} (14/19) & 51.5 (51/99) & 0.96 \\
Simple-performance reviewer & 20/20 & 85.0 {\scriptsize [64.0, 94.8]} (17/20) & 69.7 (53/76) & 0.97 \\
Dependency-minimal explainer & 19/20 & 95.0 {\scriptsize [76.4, 99.1]} (19/20) & 73.2 (52/71) & 0.99 \\
Examples-first minimalist & 20/20 & 75.0 {\scriptsize [53.1, 88.8]} (15/20) & 95.0 (76/80) & 0.96 \\
Plain-language technologist & 19/19 & 89.5 {\scriptsize [68.6, 97.1]} (17/19) & 43.1 (25/58) & 0.90 \\
Test-oriented hobbyist & 20/20 & 72.2 {\scriptsize [49.1, 87.5]} (13/18) & 72.4 (55/76) & 0.96 \\
Examples-first learner & 19/19 & 68.4 {\scriptsize [46.0, 84.6]} (13/19) & 86.4 (89/103) & 0.95 \\
\midrule
\textbf{all 12 cards} & 233/236 & 81.8 {\scriptsize [76.3, 86.3]} (189/231) & 75.4 (636/844) & 0.96 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/supp_finance.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Finance, round 1 (all 361 tasks).} Values are gpt-5.6-sol / gpt-6-astra. Advice scores are PRBench rubric percentages over the whole conversation and over the last assistant message; persona pass and joint pass are percentages of conversations. Source: examples/persona-trials/README.md.}
\label{tab:supp-finance}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Condition} & \textbf{Advice, whole} & \textbf{Advice, last} & \textbf{Persona pass (\%)} & \textbf{Joint (\%)} \\
\midrule
neutral & 49.5 / 50.5 & 46.8 / 47.3 & -- & -- \\
skeptical questioner & 53.2 / 52.1 & 40.0 / 39.6 & 83 / 98 & 47 / 54 \\
designed (5 per task) & 54.2 / 53.5 & 39.6 / 38.4 & 74 / 94 & 44 / 55 \\
confident contrarian & 52.6 / 52.2 & 36.8 / 32.8 & 88 / 99 & 51 / 55 \\
concise pragmatist & 49.4 / 49.9 & 30.7 / 28.2 & 99 / 100 & 52 / 51 \\
decisive pusher & 49.4 / 50.9 & 25.2 / 25.0 & 95 / 100 & 49 / 49 \\
reassurance seeker & 49.3 / 50.4 & 23.8 / 22.4 & 97 / 100 & 50 / 52 \\
careful learner & 49.6 / 49.9 & 25.8 / 21.6 & 34 / 77 & 17 / 41 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/supp_health.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Health, 10 cases $\times$ (5 personas + neutral) $\times$ 2 anonymous doctor configurations.} Inquiry coverage is not diagnostic accuracy. Persona demonstration is the share of attribute items with an opportunity that were clearly shown. Need credit is conditional on a scoreable need (number of cases of 10 in parentheses). Source: healthbench-benchmark/examples/RESULTS.md.}
\label{tab:supp-health}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Persona / doctor} & \textbf{Inquiry} & \textbf{Facts} & \textbf{Demonstration} & \textbf{Need credit (scoreable)} \\
\midrule
P1 / Doctor A & 50.8 & 71.2 & 76.3 & 100.0 (7/10) \\
P1 / Doctor B & 46.7 & 77.5 & 76.7 & 90.6 (8/10) \\
P2 / Doctor A & 45.6 & 66.4 & 61.1 & 100.0 (1/10) \\
P2 / Doctor B & 47.9 & 78.2 & 65.8 & 100.0 (1/10) \\
P3 / Doctor A & 44.9 & 79.2 & 88.3 & 100.0 (7/10) \\
P3 / Doctor B & 49.5 & 78.6 & 85.2 & 100.0 (8/10) \\
P4 / Doctor A & 49.4 & 85.8 & 93.8 & 100.0 (10/10) \\
P4 / Doctor B & 60.0 & 86.8 & 91.5 & 100.0 (10/10) \\
P5 / Doctor A & 52.3 & 80.1 & 77.9 & 100.0 (4/10) \\
P5 / Doctor B & 47.0 & 77.9 & 65.1 & 100.0 (4/10) \\
NEUTRAL / Doctor A & 45.2 & 78.5 & -- & -- \\
NEUTRAL / Doctor B & 51.3 & 86.7 & -- & -- \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/supp_help.tex <==
\begin{table}[H]
\centering
\caption{\textbf{HelpBench, 450 tasks (v2 protocol).} Planned 2,250, completed 2,161, graded 2,086, valid 2,081. Task score is the trajectory rubric score; persona adherence is evaluated only after disclosure. Source: examples/gpt6-astra-attributes-v2-450-task/SUMMARY.md.}
\label{tab:supp-help}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Condition} & \textbf{Valid / planned} & \textbf{Task score (\%)} & \textbf{Adherence (\%)} \\
\midrule
neutral\_multi / neutral & 417/450 & 81.82 (n=417) & -- \\
persona\_multi / careful\_learner & 412/450 & 82.75 (n=412) & 99.86 (n=365) \\
persona\_multi / concise\_pragmatist & 419/450 & 81.35 (n=419) & 99.48 (n=240) \\
persona\_multi / skeptical\_questioner & 406/450 & 81.77 (n=406) & 99.92 (n=396) \\
single\_turn / neutral & 427/450 & 79.77 (n=427) & -- \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/supp_law.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Law, 59 cases $\times$ 5 archetypes (client gpt-5.6-sol).} Resolution $=\frac12$(Fact + Issue Resolution); adherence is the client persona judge's score and its components (percent). Means are taken within each jurisdiction and then across jurisdictions. Source: examples/gpt-5.6-sol-simulation-astra-judge-all-cases/SUMMARY.md.}
\label{tab:supp-law}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
\textbf{Archetype} & \textbf{Res.} & \textbf{Fact} & \textbf{Issue} & \textbf{Adher.} & \textbf{Arch.} & \textbf{Attr.} & \textbf{Goal} & \textbf{Facts} & \textbf{Rules} \\
\midrule
Assured cooperator & 39.9 & 52.6 & 27.2 & 80.9 & 100.0 & 79.0 & 100.0 & 39.8 & 89.0 \\
Dependent and anxious & 34.7 & 49.7 & 19.8 & 76.8 & 87.3 & 76.2 & 100.0 & 27.0 & 93.2 \\
Avoidant and withdrawn & 39.2 & 51.8 & 26.6 & 76.5 & 83.0 & 76.3 & 100.0 & 28.7 & 90.7 \\
Controlling resister & 41.0 & 53.1 & 28.9 & 77.3 & 83.1 & 77.0 & 100.0 & 36.2 & 87.3 \\
Trusting but impatient & 34.8 & 47.9 & 21.6 & 76.2 & 63.5 & 78.0 & 98.3 & 33.1 & 93.2 \\
\midrule
overall & 37.9 & 51.0 & 24.8 & 77.5 & 83.4 & 77.3 & 99.7 & 32.9 & 90.7 \\
PRC cases & 37.3 & 41.8 & 32.9 & 77.8 & 83.1 & 78.0 & 100.0 & 26.2 & 92.4 \\
U.S. cases & 38.5 & 60.2 & 16.8 & 77.3 & 83.7 & 76.6 & 99.3 & 39.7 & 89.0 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/supp_needtypes.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Coding need types.} The classification is an analysis choice made for this paper. A need \emph{asks for content} if the user can request additional material in the conversation, and \emph{constrains form} if it states a property of the delivered code that a user would normally expect by default. Counts are for critical needs: expressed and answered over applicable, and satisfied / partially satisfied among answered.}
\label{tab:need-types}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}p{2.6cm}rrr>{\raggedright\arraybackslash}p{7.2cm}@{}}
\toprule
\textbf{Class} & \textbf{Types} & \textbf{Answered / applicable} & \textbf{Sat. / partial} & \textbf{Need types} \\
\midrule
Asks for content & 10 & 574/617 & 526 / 48 & verification\_rationale, detailed\_explanation, concise\_explanation, public\_test\_cases, plain\_language, example\_walkthrough, decision\_tradeoffs, revision\_and\_checks, performance\_check, minimal\_test\_exposition \\
Constrains the artifact's form & 15 & 58/206 & 58 / 0 & type\_annotations, custom\_implementation, low\_complexity, readability, minimal\_dependencies, no\_comments, straightforward\_structure, object\_oriented\_structure, standard\_library\_tools, self\_documenting\_code, extensive\_comments, modular\_structure, compact\_names, docstrings, maintainability \\
Delivery and tone & 3 & 4/21 & 4 / 0 & deadline\_delivery, supportive\_tone, direct\_tone \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/supp_variance.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Variance of the native score attributed to task, persona and interaction.} Shares are percentages of the total sum of squares ($\eta^2$, \secref{sec:stats}); the persona share is within task, with a 95\% task-cluster bootstrap interval, and the last column is the 97.5th percentile of its within-task permutation null (1{,}000 permutations). Finance uses round 1 and conversations with a valid simulator audit; HelpBench uses the neutral and the three persona multi-turn arms.}
\label{tab:supp-variance}
\begingroup
\scriptsize\setstretch{1.0}
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{@{}p{4.6cm}rrrrrr@{}}
\toprule
\textbf{Score} & \textbf{n} & \textbf{Tasks / conditions} & \textbf{Task} & \textbf{Persona} & \textbf{Interaction + noise} & \textbf{Null 97.5th} \\
\midrule
Finance, whole conversation, gpt-5.6-sol & 4,203 & 361 / 12 & 87.6 & 1.5 {\scriptsize [1.2, 2.0]} & 10.8 & 0.07 \\
Finance, whole conversation, gpt-6-astra & 4,225 & 361 / 12 & 91.4 & 0.6 {\scriptsize [0.5, 0.9]} & 7.9 & 0.05 \\
Finance, last message, gpt-5.6-sol & 4,215 & 361 / 12 & 50.2 & 12.4 {\scriptsize [10.7, 14.3]} & 37.4 & 0.28 \\
Finance, last message, gpt-6-astra & 4,227 & 361 / 12 & 51.4 & 13.4 {\scriptsize [11.5, 15.7]} & 35.2 & 0.26 \\
HelpBench, trajectory score, gpt-6-astra & 1,654 & 431 / 4 & 91.9 & 0.2 {\scriptsize [0.1, 0.3]} & 7.9 & 0.06 \\
Law, Resolution, client gpt-5.6-sol & 295 & 59 / 5 & 73.1 & 2.6 {\scriptsize [1.4, 5.6]} & 24.3 & 1.27 \\
Law, client adherence & 295 & 59 / 5 & 28.4 & 6.0 {\scriptsize [3.0, 12.1]} & 65.6 & 3.18 \\
Coding, tests passed (binary) & 236 & 20 / 12 & 12.8 & 7.2 {\scriptsize [4.2, 18.7]} & 80.0 & 7.46 \\
\bottomrule
\end{tabular}
\endgroup
\end{table}

